A note on a bijection for Schr\"oder permutations

There is a bijection from Schroder paths to {4132, 4231}-avoiding permutations due to Bandlow, Egge, and Killpatrick that sends "area" to "inversion number". Here we give a concise description of this bijection.

==> texmf/tex/latex/pstricks/multido.tex <==
%% BEGIN multido.tex
%%
\def\fileversion{1.4}
\def\filedate{93/01/14}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   multido.tex/multido.sty contains a loop macro, \multido, that supports
%%   fixed-point addition and has a nice interface. Among other things, it
%%   is useful for pictures and putting numbers on axes. multido.tex
%%   is compatible with most TeX macro packages, including Plain TeX, LaTeX,
%%   AmSTeX, and Ams-LaTeX.
%%
%% INSTALLATION:
%%   Put this file where your TeX looks for inputs, under the name multido.tex.
%%   Use the file multido.sty with LaTeX.
%%
%% DOCUMENTATION:
%%   See multido.doc.
%%
%% COPYING:
%%   Copying of part or all of this file is allowed under the following
%%   conditions only:
%%   (1) You may freely distribute unchanged copies of the file. Please
%%       include the documentation when you do so.
%%   (2) You may modify a renamed copy of the file, but only for personal
%%       use or use within an organization.
%%   (3) You may copy fragments from the file, for personal use or for
%%       distribution, as long as credit is given where credit is due.
%%
%%   You are NOT ALLOWED to take money for the distribution or use of
%%   this file or modified versions or fragments thereof, except for
%%   a nominal charge for copying etc.
%%
%% CODE:
% These macros use TeX primitives, plus the Plain TeX commands:
%   \dimen@, \dimen@i, \count@, \newcount, \newtoks, \@ne, \tw@, \@z@.
%
% Check if file is loaded, announce file on terminal, and take care of @:
%


\message{ v\fileversion, \filedate\space <tvz>}

\csname MultidoLoaded\endcsname
\let\MultidoLoaded\endinput

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

% These are some useful hacks. "\multido@dimtonum" strips the value of "#1",
% a dimension register, of the "pt", and assigns the result to "#2",
% a command sequence.

\def\@empty{}
\def\@nnil{\@nil}
\def\multido@dimtonum#1#2{\edef#2{\multido@@dimtonum#1}}
\def\multido@@dimtonum#1{\expandafter\multido@@@dimtonum\the#1}
\edef\next{%
  \noexpand\def\noexpand\multido@@@dimtonum##1\string p\string t{##1}}
\next

% "\multido@count" stores the number of repetitions. "\multidocount" keeps
% track of the iteration. These are also used locally as scratch counters
% by "\FPadd@". "\multido@stuff" is used to store the <stuff> that is
% to be repeated.

\newcount\multido@count
\newcount\multidocount
\newtoks\multido@stuff

\def\multido{\multido@{}{\begingroup}{\endgroup}}
\def\mmultido{\multido@{\multido@stepvar}{\begingroup}{\endgroup}}
\def\Multido{\multido@{}{}{}}
\def\MMultido{\multido@{\multido@stepvar}{}{}}

% "\multido@initvar" processes the variable declarations, initializing
% the value of the variables and defining "\multido@stepvar" to increment
% the variables with each repetition. "\multido@count" is set to the number
% of repetitions.

\long\def\multido@#1#2#3#4#5#6{%
  #2%
    \multido@count=#5\relax
    \ifnum\multido@count=\z@\else\multido@@{#1}{#4}{#6}\fi
  #3%
  \ignorespaces}
\def\multido@@#1#2#3{%
  \def\multido@stepvar{}%
  \def\do{\noexpand\do\noexpand}%
  \multido@initvar#2,\@nil,%
  \let\do\noexpand
  \edef\multido@stepvar{\multido@stepvar}%
  \ifnum\multido@count<\z@\multido@count=-\multido@count\fi
  \multidocount=1\relax
  #1%
  \multido@stuff{#3}%
  \multido@loop}
\def\multido@loop{%
  \the\multido@stuff
  \ifnum\multidocount<\multido@count
    \advance\multidocount\@ne
    \multido@stepvar
    \expandafter\multido@loop
  \fi}
\def\multidostop{\multidocount=\multido@count}
\def\multido@badvar{%
  \multido@count=0
  \errhelp{\multido command will be skipped.}%
  \errmessage{Bad \string\multido\space variable declaration}}
\def\multido@initvar#1,{%
  \def\multido@temp{#1}%
  \ifx\multido@temp\@nnil\else
    \ifx\multido@temp\@empty\else
      \multido@@initvar#1\@nil=+\@nil\relax
    \fi
    \expandafter\multido@initvar
  \fi}
\def\multido@@initvar#1=#2+#3\@nil#4\relax{%
  \ifx\@empty#4\@empty
    \multido@badvar
  \else
    \multido@vartype#1\@empty
    \ifx\multido@temp\relax
      \multido@badvar
    \else
      \multido@temp{#2}{#3}#1%
    \fi
  \fi}
\def\multido@vartype#1{%
  \ifcat\noexpand\@nil\noexpand#1%
     \expandafter\multido@@vartype\string#1\@nil
  \else
    \let\multido@temp\relax
  \fi}
\def\multido@@vartype#1#2#3\@nil{%
  \expandafter\let\expandafter\multido@temp
    \csname multido@init@#2\endcsname}
\def\MultidoCheckNames{%
  \let\multido@@@vartype\multido@vartype
  \def\multido@vartype##1{%
    \ifx\undefined##1%
      \multido@@@vartype{##1}%
    \else
      \errhelp{\multido command will be skipped.}%
      \errmessage{Multido variable \string##1 already defined}%
      \let\multido@temp\relax
    \fi}}

% For each variable type, we must now define \multido@init<vartype>.
% The syntax of these macros is:
%
%   \multido@init@<vartype>{initial value}{increment}{variable}
%
% and the outcome should be:
%
% 1. Set <variable> to the initial value.
% 2. Invoke \multido@addtostep{step stuff}, where <step stuff> is
% whatever should be done to increment the variable. <step stuff> is
% expanded first, with expansion suppressed by "\do".

\def\multido@addtostep#1{\edef\multido@stepvar{\multido@stepvar#1}}

% Variable type for dimensions ("d", "D"):

\def\multido@init@d#1#2#3{%
  \expandafter\ifx\csname pssetlength\endcsname\relax
    \dimen@=#1\relax\dimen@i=#2\relax
  \else
    \pssetlength\dimen@{#1}\pssetlength\dimen@i{#2}%
  \fi
  \edef#3{\number\dimen@ sp}%
  \ifnum\multido@count<\z@\dimen@i=-\dimen@i\fi
  \multido@addtostep{\do\multido@step@d{\do#3}{\number\dimen@i sp}}}
\def\multido@step@d#1#2{%
  \dimen@=#1\advance\dimen@#2
  \edef#1{\number\dimen@ sp}}%
\def\multido@init@D{\multido@init@d}

% Variable type for integers ("i", "I"):

\def\multido@init@i#1#2#3{%
  \count@=#1\relax
  \edef#3{\the\count@}%
  \count@=#2\relax
  \ifnum\multido@count<\z@\count@=-\count@\fi
  \multido@addtostep{\do\multido@step@i{\do#3}{\the\count@}}}
\def\multido@step@i#1#2{%
  \count@=#1\advance\count@ by #2
  \edef#1{\the\count@}}
\def\multido@init@I{\multido@init@i}

% Variable type for reals ("r", "R").

\def\multido@init@r#1#2#3{%
  \dimen@=#1pt
  \multido@dimtonum\dimen@#3%
  \dimen@=#2pt
  \ifnum\multido@count<\z@\dimen@=-\dimen@\fi
  \multido@addtostep{\do\multido@step@r{\do#3}{\number\dimen@ sp}}}
\def\multido@step@r#1#2{%
  \dimen@=#1pt\advance\dimen@#2
  \multido@dimtonum\dimen@#1}
\def\multido@init@R{\multido@init@r}

% Variable type for numbers ("n", "N").

\def\multido@init@n#1#2#3{%
  \edef#3{#1}%
  \ifnum\multido@count<\z@\expandafter\FPsub\else\expandafter\FPadd\fi
  {0}{#2}\multido@temp
  \multido@addtostep{\do\FPadd{\do#3}{\multido@temp}{\do#3}}}
\def\multido@init@N{\multido@init@n}

% Simple fixed-point addition couldn't be harder.
% "\dimen@" and "\dimen@i" are used as scratch {\em counters} (to avoid
% creating a new counter). "\count@", "\multido@count" and "\multidocount"
% are also used as scratch counters.

% This is probably pretty close to optimal, given the requirements that
% leading and trailing spaces be OK in the arguments, and that there need
% not be any numbers to the left of the decimal.

\def\FPadd#1#2#3{%
  \edef\multido@temp{#1..\noexpand\@nil#2}%
  \expandafter\FPadd@\multido@temp..\@nil
  \let#3\multido@temp}
\def\FPsub#1#2{%
  \edef\multido@temp{\noexpand\FPsub@#2\noexpand\@empty}%
  \FPadd{#1}{\multido@temp}}
\def\FPsub@#1{\ifx-#1\else-#1\fi}
\def\FPadd@#1.#2.#3\@nil#4.#5.#6\@nil{%
  \begingroup
    \def\multido@temp{\let\next\relax}%
    \let\next\z@
    \afterassignment\multido@temp\count@=#1\next
    \dimen@i=0#2sp\relax
    \let\next\z@
    \afterassignment\multido@temp\multido@count=#4\next
    \multidocount=0#5\relax
    \dimen@=\number\count@ sp
    \count@=\@ne
    \FPadd@@@#500000000\@nil
    \ifnum#11<\z@
      \count@=-\tw@
      \dimen@=-\dimen@
    \fi
    \ifnum#41<\z@
      \count@=-\count@
      \multido@count=-\multido@count
    \fi
    \ifnum\count@>\z@
      \advance\multido@count\dimen@
      \advance\multidocount\dimen@i
      \ifnum\multidocount<\multido@temp\relax
        \advance\multidocount\multido@temp\relax
      \else
        \advance\multido@count\@ne
      \fi
      \advance\count@-3
    \else
      \advance\multido@count-\dimen@
      \advance\multidocount-\dimen@i
      \ifnum\multido@count<\z@
        \multido@count=-\multido@count
        \multidocount=-\multidocount
        \advance\count@\@ne
      \else
        \ifnum\multido@count=\z@
          \ifnum\multidocount<\z@
            \multidocount=-\multidocount
            \advance\count@\@ne
          \fi
        \fi
      \fi
      \ifnum\multidocount<\z@
        \advance\multidocount\multido@temp
        \advance\multido@count-\@ne
      \fi
      \advance\multidocount\multido@temp\relax
    \fi
    \expandafter\FPadd@@\the\multidocount\@empty\@nil
  \endgroup}
\def\FPadd@@#1#2#3\@nil{\xdef\multido@temp{%
  \ifnum\count@=-1-\fi
  \the\multido@count\ifx#2\@empty\else.#2#3\fi}}
\def\FPadd@@@#1#2#3#4#5#6#7#8#9\@nil{\def\multido@temp{1#9}}

\catcode`\@=\TheAtCode\relax

\endinput
%%
%% END multido.tex


==> texmf/tex/latex/pstricks/pst-3d.tex <==
%% BEGIN pst-3d.tex
%%
%% Tilting and other pseudo-3D tricks with PSTricks 97.
%% There is not any documentation.
%%
\def\fileversion{97}
\def\filedate{1997/03/25}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\message{ v\fileversion, \filedate}

\csname PSTthreeDLoaded\endcsname
\let\PSTthreeDLoaded\endinput

\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex}
  \expandafter\next
\fi

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

% \begin{macro}{\tx@SetMatrixThreeD,\tx@ProjThreeD,\tx@SetMatrixEmbed}
% Viewpoint for 3D coordinates is given by three angles: $\alpha$, $\beta$ and
% $\gamma$. $\alpha$ and $\beta$ determine the direction from which one is
% looking. $\gamma$ then determines the orientation of the observing.
%
% When $\alpha$, $\beta$ and $\gamma$ are all zero, the observer is looking
% from the negative part of the $y$-axis, and sees the $xz$-plane the way in
% 2D one sees the $xy$ plan. Hence, to convert the 3D coordinates to their 2D
% project, $\la x, y, z\ra$ map to $\la x, z\ra$.
%
% When the orientation is different, we rotate the coordinates, and then
% perform the same projection.
%
% We move up to latitude $\beta$, over to longitude $\alpha$, and then rotate
% by $\gamma$. This means that we first rotate around $y$-axis by $\gamma$,
% then around $x$-axis by $\beta$, and the around $z$-axis by $\alpha$.
%
% Here are the matrices:
% \begin{eqnarray*}
%   R_z(\alpha) & = & \left[
%     \begin{array}{ccc}
%       \cos \alpha & -\sin \alpha & 0 \\
%       \sin \alpha & cos \alpha   & 0 \\
%       0           & 0            & 1
%     \end{array} \right] \\
%   R_x(\beta) & = & \left[
%     \begin{array}{ccc}
%       1           & 0            & 0 \\
%       0           & \cos \beta   & \sin \beta \\
%       0           & -\sin \beta  & \cos \beta
%     \end{array} \right] \\
%   R_y(\gamma) & = & \left[
%     \begin{array}{ccc}
%       \cos \gamma & 0            & -\sin \gamma \\
%       0           & 1            & 0 \\
%       \sin \gamma & 0            & \cos \gamma
%     \end{array} \right]
% \end{eqnarray*}
%
% The rotation of a coordinate is then performed by the matrix $R_z(\alpha)
% R_x(\beta) R_y(\gamma)$. The first and third columns of the matrix are the
% basis vectors of the plan upon which the 3D coordinates are project (the old
% basis vectors were $\la 1, 0, 0\ra$ and $\la 0, 0, 1$\ra; rotating these
% gives the first and third columns of the matrix).
%
% These new basis vectors are:
% \begin{eqnarray*}
%   \tilde{x} & = & \left[
%     \begin{array}{c}
%       \cos\alpha \cos\gamma - \sin\beta \sin\alpha \sin\gamma \\
%       \sin\alpha \cos\gamma + \sin\beta \cos\alpha \sin\gamma \\
%       \cos\beta \sin\gamma
%     \end{array} \right] \\
%   \tilde{z} & = & \left[
%     \begin{array}{c}
%       -\cos\alpha \sin\gamma - \sin\beta \sin\alpha \cos\gamma \\
%       -\sin\alpha \sin\gamma + \sin\beta \cos\alpha \cos\gamma \\
%       \cos\beta \cos\gamma
%     \end{array} \right]
% \end{eqnarray*}
%
% Rather than specifying the angles $\alpha$ and $\beta$, the user gives a
% vector indicating where the viewpoint is. This new viewpoint is the rotation
% o the old viewpoint. The old viewpoint is $\la 0, -1, 0\ra$, and so the new
% viewpoint is
% \[
%  R_z(\alpha) R_x(\beta) \left[ \begin{array}{c} 0\\-1\\0 \end{array} \right]
%  \, = \,
%  \left[ \begin{array}{c}
%    \cos\beta \sin\alpha \\
%    -\cos\beta \cos\alpha \\
%    \sin\beta
%  \end{array} \right]
%  \, = \,
%  \left[ \begin{array}{c} v_1 \\ v_2 \\ v_3 \end{array} \right]
% \]
% Therefore,
% \begin{eqnarray*}
%   \alpha & = & \arc\tan (v_1 / -v_2) \\
%   \beta & = & \arc\tan (v_3 \sin\alpha / v_1)
% \end{eqnarray*}
% Unless $p_1=p_2=0$, in which case $\alpha=0$ and $\beta=\sign(p_3)90$, or
% $p_1=p_3=0$, in which case $\beta=0$.
%
% The syntax of "SetMatrixThreeD" is
% \begin{Ex}
%   $v_1$ $v_2$ $v_3$ $\gamma$ "SetMatrixThreeD"
% \end{Ex}
% "SetMatrixThreeD" first computes
% \[
%   \begin{array}{ll}
%     a=\sin\alpha & b=\cos\alpha\\
%     c=\sin\beta  & d=\cos\beta\\
%     e=\sin\gamma & f=\cos\gamma
%   \end{array}
% \]
% and then sets "Matrix3D" to "["$\tilde{x}$ $\tilde{z}$"]".
%
%    \begin{macrocode}
\pst@def{SetMatrixThreeD}<%
  dup sin /e ED cos /f ED
  /p3 ED /p2 ED /p1 ED
  p1 0 eq
  { /a 0 def /b p2 0 le { 1 } { -1 } ifelse def
    p3 p2 abs
  }
  { p2 0 eq
    { /a p1 0 lt { -1 } { 1 } ifelse def /b 0 def
      p3 p1 abs
    }
    { p1 dup mul p2 dup mul add sqrt dup
      p1 exch div /a ED
      p2 exch div neg /b ED
      p3 p1 a div
    }
    ifelse
  }
  ifelse
  atan dup sin /c ED cos /d ED
  /Matrix3D
  [
    b f mul c a mul e mul sub
    a f mul c b mul e mul add
    d e mul
    b e mul neg c a mul f mul sub
    a e mul neg c b mul f mul add
    d f mul
  ] def>
%    \end{macrocode}
%
% The syntax of "ProjThreeD" is
% \begin{Ex}
%   $x$ $y$ $z$ ProjThreeD $x'$ $y'$
% \end{Ex}
% where $x'=\la x, y, z\ra \cdot \tilde{x}$ and $y'=\la x, y, z\ra \cdot
% \tilde{z}$.
%
%    \begin{macrocode}
\pst@def{ProjThreeD}<%
  /z ED /y ED /x ED
  Matrix3D aload pop
  z mul exch y mul add exch x mul add
  4 1 roll
  z mul exch y mul add exch x mul add
  exch>
%    \end{macrocode}
%
% To embed 2D $\la x, y\ra$ coordinates in 3D, the user specifies the normal
% vector and an angle. If we decompose this normal vector into an angle, as
% when converting 3D coordinates to 2D coordinates, and let $\hat\alpha$,
% $\hat\beta$ and $\hat\gamma$ be the three angles, then when these angles are
% all zero the coordinate $\la x, y\ra$ gets mapped to $\la x, 0, y\ra$, and
% otherwise $\la x, y\ra$ gets mapped to
% \[
%   R_z(\hat\alpha) R_x(\hat\beta) R_y(\hat\gamma)
%   \left[ \begin{array}{c} x \\ 0 \\ y \end{array} \right]
%  \, = \,
%   \left[ \begin{array}{c}
%    \hat{x}_1 x + \hat{z}_1 y\\
%    \hat{x}_2 x + \hat{z}_2 y\\
%    \hat{x}_3 x + \hat{z}_3 y
%   \end{array} \right]
% \]
% where $\hat{x}$ and $\hat{z}$ are the first and third columns of
% $R_z(\hat\alpha) R_x(\hat\beta) R_y(\hat\gamma)$.
%
% Now add on a 3D-origin:
% \[
%   \left[ \begin{array}{c}
%    \hat{x}_1 x + \hat{z}_1 y + x_0\\
%    \hat{x}_2 x + \hat{z}_2 y + y_0\\
%    \hat{x}_3 x + \hat{z}_3 y + z_0
%   \end{array} \right]
% \]
%
% Now when we project back onto 2D coordinates, we get
% \begin{eqnarray*}
%   x' & = & \tilde{x}_1(\hat{x}_1 x + \hat{z}_1 y + x_0) +
%            \tilde{x}_2(\hat{x}_2 x + \hat{z}_2 y + y_0) +
%            \tilde{x}_3(\hat{x}_3 x + \hat{z}_3 y + z_0)\\
%   & = &
%   (\tilde{x}_1\hat{x}_1 + \tilde{x}_2\hat{x}_2 + \tilde{x}_3\hat{x}_3) x\\
%   + (\tilde{x}_1\hat{z}_1 + \tilde{x}_2\hat{z}_2 + \tilde{x}_3\hat{z}_3) y\\
%   + \tilde{x}_1 x_0 + \tilde{x}_2 y_0 + \tilde{z}_3 z_0
%   y' & = & \tilde{z}_1(\hat{x}_1 x + \hat{z}_1 y + x_0) +
%            \tilde{z}_2(\hat{x}_2 x + \hat{z}_2 y + y_0) +
%            \tilde{z}_3(\hat{x}_3 x + \hat{z}_3 y + z_0)\\
%   & = &
%   (\tilde{z}_1\hat{x}_1 + \tilde{z}_2\hat{x}_2 + \tilde{z}_3\hat{x}_3) x\\
%   + (\tilde{z}_1\hat{z}_1 + \tilde{z}_2\hat{z}_2 + \tilde{z}_3\hat{z}_3) y\\
%   + \tilde{z}_1 x_0 + \tilde{z}_2 y_0 + \tilde{z}_3 z_0
% \end{eqnarray*}
% Hence, the transformation matrix is:
% \[
%   \left[ \begin{array}{c}
%   \tilde{x}_1\hat{x}_1 + \tilde{x}_2\hat{x}_2 + \tilde{x}_3\hat{x}_3) \\
%   \tilde{z}_1\hat{x}_1 + \tilde{z}_2\hat{x}_2 + \tilde{z}_3\hat{x}_3) \\
%   \tilde{x}_1\hat{z}_1 + \tilde{x}_2\hat{z}_2 + \tilde{x}_3\hat{z}_3) \\
%   \tilde{z}_1\hat{z}_1 + \tilde{z}_2\hat{z}_2 + \tilde{z}_3\hat{z}_3) \\
%   \tilde{x}_1 x_0 + \tilde{x}_2 y_0 + \tilde{z}_3 z_0 \\
%   \tilde{z}_1 x_0 + \tilde{z}_2 y_0 + \tilde{z}_3 z_0
%   \end{array} \right]
% \]
%
% The syntax of "SetMatrixEmbed" is
% \begin{Ex}
%   $x_0$ $y_0$ $z_0$ $\hat{v_1}$ $\hat{v_2}$ $\hat{v_3} $\hat{\gamma}$
%   $v_1$ $v_2$ $v_3$ $\gamma$ "SetMatrixEmbed"
% \end{Ex}
% "SetMatrixEmbed" first sets "<x1 x2 x3 y1 y2 y3>" to the basis vectors for
% the viewpoint projection (the tilde stuff above). Then it sets "Matrix3D" to
% the basis vectors for the embedded plane. Finally, it sets the
% transformation matrix to the matrix given above.
%
%    \begin{macrocode}
\pst@def{SetMatrixEmbed}<%
  \tx@SetMatrixThreeD
  Matrix3D aload pop
  /z3 ED /z2 ED /z1 ED /x3 ED /x2 ED /x1 ED
  \tx@SetMatrixThreeD
  [
  Matrix3D aload pop
  z3 mul exch z2 mul add exch z1 mul add 4 1 roll
  z3 mul exch z2 mul add exch z1 mul add
  Matrix3D aload pop
  x3 mul exch x2 mul add exch x1 mul add 4 1 roll
  x3 mul exch x2 mul add exch x1 mul add
  3 -1 roll 3 -1 roll 4 -1 roll 8 -3 roll 3 copy
  x3 mul exch x2 mul add exch x1 mul add 4 1 roll
  z3 mul exch z2 mul add exch z1 mul add
  ]
  concat>
%   \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psset@viewpoint,\psk@viewpoint}
%    \begin{macrocode}
\let\pssetzlength\pssetylength
\def\psset@viewpoint#1{%
  \pst@expandafter\psset@@viewpoint#1 {} {} {} \@nil
  \let\psk@viewpoint\pst@tempg}
\def\psset@@viewpoint#1 #2 #3 #4\@nil{%
  \begingroup
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetzlength\pst@dimc{#3}%
    \xdef\pst@tempg{%
      \pst@number\pst@dima \pst@number\pst@dimb \pst@number\pst@dimc}%
  \endgroup}
\psset@viewpoint{1 -1 1}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psset@viewangle,\psk@viewangle}
%    \begin{macrocode}
\def\psset@viewangle#1{\pst@getangle{#1}\psk@viewangle}
\psset@viewangle{0}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psset@normal,\psk@normal}
%    \begin{macrocode}
\def\psset@normal#1{%
  \pst@expandafter\psset@@viewpoint#1 {} {} {} \@nil
  \let\psk@normal\pst@tempg}
\psset@normal{0 0 1}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psset@embedangle,\psk@embedangle}
%    \begin{macrocode}
\def\psset@embedangle#1{\pst@getangle{#1}\psk@embedangle}
\psset@embedangle{0}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\tx@TMSave,\tx@TMRestore}
% \begin{LVerbatim}
%   {<Proc for modifying tm>} TMChange
%    \begin{macrocode}
\pst@def{TMSave}<%
  tx@Dict /TMatrix known not { /TMatrix { } def /RAngle { 0 } def } if
  /TMatrix [ TMatrix CM ] cvx def>
\pst@def{TMRestore}<%
  CP /TMatrix [ TMatrix setmatrix ] cvx def moveto>
\pst@def{TMChange}<%
  \tx@TMSave
  /cp [ currentpoint ] cvx def % ??? Check this later.
  CM
% Set "standard" coor. system , with "pt" units and origin at currentpoint.
% This let's us rotate, or whatever, around \TeX's current point, without
% having to worry about strange coordinate systems that the dvi-to-ps
% driver might be using.
  CP T \tx@STV
% Let M = old matrix (on stack), and M' equal current matrix. Then
% go from M' to M by applying  M Inv(M').
  CM matrix invertmatrix    % Inv(M')
  matrix concatmatrix       % M Inv(M')
% Now modify transformation matrix:
  exch exec
% Now apply M Inv(M')
  concat cp moveto>
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\ThreeDput}
%    \begin{macrocode}
\def\ThreeDput{\def\pst@par{}\pst@object{ThreeDput}}
\def\ThreeDput@i{\@ifnextchar({\ThreeDput@ii}{\ThreeDput@ii(\z@,\z@,\z@)}}
\def\ThreeDput@ii(#1,#2,#3){%
  \pst@killglue\pst@makebox{\ThreeDput@iii(#1,#2,#3)}}
\def\ThreeDput@iii(#1,#2,#3){%
  \begingroup
    \use@par
    \if@star\pst@starbox\fi
    \pst@makesmall\pst@hbox
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetzlength\pst@dimc{#3}%
    \leavevmode
    \hbox{%
      \pst@Verb{%
        { \pst@number\pst@dima
          \pst@number\pst@dimb
          \pst@number\pst@dimc
          \psk@normal
          \psk@embedangle
          \psk@viewpoint
          \psk@viewangle
          \tx@SetMatrixEmbed
        } \tx@TMChange}%
    \box\pst@hbox
    \pst@Verb{\tx@TMRestore}}%
  \endgroup
  \ignorespaces}
%    \end{macrocode}
% \end{macro}
%
%
% \section{Arithmetic\label{Arithmetic}}
%
%
% \begin{macro}{\pst@divide}
% This is adapted from Donald Arseneau's "shapepar.sty".
% Syntax:
% \begin{LVerbatim}
%   \pst@divide{<numerator>}{<denominator>}{<command>}
%   \pst@@divide{<numerator>}{<denominator>}
% \end{LVerbatim}
% <numerator> and <denominator> should be dimensions. "\pst@divide" sets
% <command> to <num>/<den> (in points). "\pst@@divide" sets "\pst@dimg" to
% <num>/<den>.
%    \begin{macrocode}
\def\pst@divide#1#2#3{%
  \pst@@divide{#1}{#2}%
  \pst@dimtonum\pst@dimg{#3}}
\def\pst@@divide#1#2{%
  \pst@dimg=#1\relax
  \pst@dimh=#2\relax
  \pst@cntg=\pst@dimh
  \pst@cnth=67108863
  \pst@@@divide\pst@@@divide\pst@@@divide\pst@@@divide
  \divide\pst@dimg\pst@cntg}
%    \end{macrocode}
% The number 16 is the level of uncertainty. Use a lower power of 2 for more
% accuracy (2 is most precise). But if you change it, you must change the
% repetions of "\pst@@@divide" in "\pst@@divide" above:
% \[
%   \mbox{precision}^\mbox{repetitions} = 65536
% \]
% (E.g., $16^4 = 65536$).
%    \begin{macrocode}
\def\pst@@@divide{%
  \ifnum
    \ifnum\pst@dimg<\z@-\fi\pst@dimg<\pst@cnth
    \multiply\pst@dimg\sixt@@n
  \else
    \divide\pst@cntg\sixt@@n
  \fi}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\pst@pyth}
% Syntax:
% \begin{LVerbatim}
%   \pst@pyth{<dim1>}{<dim2>}{<dimen register>}
% \end{LVerbatim}
% <dimen register> is set to $((dim1)^2+(dim2)^2)^{1/2}$.
%
% The algorithm is copied from \PiCTeX, by Michael Wichura (with permission).
% Here is his description:
% \begin{quote}
% Suppose $x>0$, $y>0$. Put $s = x+y$. Let $z = (x^2+y^2)^{1/2}$. Then $z =
% s\times f$, where
% \[
%   f = (t^2 + (1-t)^2)^{1/2} = ((1+\tau^2)/2)^{1/2}
% \]
% and $t = x/s$  and  $\tau = 2(t-1/2)$.
% \end{quote}
%    \begin{macrocode}
\def\pst@pyth#1#2#3{%
  \begingroup
    \pst@dima=#1\relax
    \ifnum\pst@dima<\z@\pst@dima=-\pst@dima\fi  % dima=abs(x)
    \pst@dimb=#2\relax
    \ifnum\pst@dimb<\z@\pst@dimb=-\pst@dimb\fi  % dimb=abs(y)
    \advance\pst@dimb\pst@dima         % dimb=s=abs(x)+abs(y)
    \ifnum\pst@dimb=\z@
      \global\pst@dimg=\z@             % dimg=z=sqrt(x^2+y^2)
    \else
      \multiply\pst@dima 8\relax              % dima= 8abs(x)
      \pst@@divide\pst@dima\pst@dimb     % dimg =8t=8abs(x)/s
      \advance\pst@dimg -4pt            % dimg = 4tau = (8t-4)
      \multiply\pst@dimg 2
      \pst@dimtonum\pst@dimg\pst@tempa
      \pst@dima=\pst@tempa\pst@dimg           % dima=(8tau)^2
      \advance\pst@dima 64pt         % dima=u=[64+(8tau)^2]/2
      \divide\pst@dima 2\relax                      % =(8f)^2
      \pst@dimd=7pt                % initial guess at sqrt(u)
      \pst@@pyth\pst@@pyth\pst@@pyth            % dimd=sqrt(u)
      \pst@dimtonum\pst@dimd\pst@tempa
      \pst@dimg=\pst@tempa\pst@dimb
      \global\divide\pst@dimg 8             % dimg=z=(8f)*s/8
    \fi
  \endgroup
  #3=\pst@dimg}
\def\pst@@pyth{%                      dimd = g <-- (g + u/g)/2
  \pst@@divide\pst@dima\pst@dimd
  \advance\pst@dimd\pst@dimg
  \divide\pst@dimd 2\relax}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\pst@sinandcos}
% Syntax:
% \begin{LVerbatim}
%   \pst@sinandcos{<dim>}{<int>}
% \end{LVerbatim}
% <dim>, in "sp" units, should equal 100,000 times the angle, in degrees
% between 0 and 90. <int> should equal the angle's quadrant (0, 1, 2 or 3).
% "\pst@dimg" is set to $\sin(\theta)$ and "\pst@dimh" is set to
% $\cos(\theta)$ (in pt's).
%
% The algorithms uses the usual McLaurin expansion.
%    \begin{macrocode}
\def\pst@sinandcos#1{%
  \begingroup
    \pst@dima=#1\relax
    \pst@dima=.366022\pst@dima     %Now 1pt=1/32rad
    \pst@dimb=\pst@dima   % dimb->32sin(angle) in pts
    \pst@dimc=32\p@       % dimc->32cos(angle) in pts
    \pst@dimtonum\pst@dima\pst@tempa
    \pst@cntb=\tw@
    \pst@cntc=-\@ne
    \pst@cntg=32
    \loop
    \ifnum\pst@dima>\@cclvi % 256
      \pst@dima=\pst@tempa\pst@dima
      \divide\pst@dima\pst@cntg
      \divide\pst@dima\pst@cntb
      \ifodd\pst@cntb
        \advance\pst@dimb \pst@cntc\pst@dima
        \pst@cntc=-\pst@cntc
      \else
        \advance\pst@dimc by \pst@cntc\pst@dima
      \fi
      \advance\pst@cntb\@ne
    \repeat
    \divide\pst@dimb\pst@cntg
    \divide\pst@dimc\pst@cntg
    \global\pst@dimg\pst@dimb
    \global\pst@dimh\pst@dimc
  \endgroup}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\pst@getsinandcos}
% "\pst@getsinandcos" normalizes the angle to be in the first quadrant, sets
% "\pst@quadrant" to 0 for the first quadrant, 1 for the second, 2 for the
% third, and 3 for the fourth, invokes "\pst@sinandcos", and sets "\pst@sin"
% to the sine and "\pst@cos" to the cosine.
%    \begin{macrocode}
\def\pst@getsinandcos#1{%
  \pst@dimg=100000sp
  \pst@dimg=#1\pst@dimg
  \pst@dimh=36000000sp
  \pst@cntg=0
  \loop
  \ifnum\pst@dimg<\z@
    \advance\pst@dimg\pst@dimh
  \repeat
  \loop
  \ifnum\pst@dimg>\pst@dimh
    \advance\pst@dimg-\pst@dimh
  \repeat
  \pst@dimh=9000000sp
  \def\pst@tempg{%
    \ifnum\pst@dimg<\pst@dimh\else
      \advance\pst@dimg-\pst@dimh
      \advance\pst@cntg\@ne
      \ifnum\pst@cntg>\thr@@ \advance\pst@cntg-4 \fi
      \expandafter\pst@tempg
    \fi}%
  \pst@tempg
  \chardef\pst@quadrant\pst@cntg
  \ifdim\pst@dimg=\z@
    \def\pst@sin{0}%
    \def\pst@cos{1}%
  \else
    \pst@sinandcos\pst@dimg
    \pst@dimtonum\pst@dimg\pst@sin
    \pst@dimtonum\pst@dimh\pst@cos
  \fi}
%    \end{macrocode}
% \end{macro}
%
% \section{Tilting}
%
% \begin{macro}{\pstilt}
%    \begin{macrocode}
\def\pstilt#1{\pst@makebox{\pstilt@{#1}}}
\def\pstilt@#1{%
  \begingroup
    \leavevmode
    \pst@getsinandcos{#1}%
    \hbox{%
      \ifcase\pst@quadrant
        \kern\pst@cos\dp\pst@hbox
        \pst@dima=\pst@cos\ht\pst@hbox
        \ht\pst@hbox=\pst@sin\ht\pst@hbox
        \dp\pst@hbox=\pst@sin\dp\pst@hbox
      \or
        \kern\pst@sin\ht\pst@hbox
        \pst@dima=\pst@sin\dp\pst@hbox
        \ht\pst@hbox=\pst@cos\ht\pst@hbox
        \dp\pst@hbox=\pst@cos\dp\pst@hbox
      \or
        \kern\pst@cos\ht\pst@hbox
        \pst@dima=\pst@sin\dp\pst@hbox
        \pst@dimg=\pst@sin\ht\pst@hbox
        \ht\pst@hbox=\pst@sin\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \or
        \kern\pst@sin\dp\pst@hbox
        \pst@dima=\pst@sin\ht\pst@hbox
        \pst@dimg=\pst@cos\ht\pst@hbox
        \ht\pst@hbox=\pst@cos\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \fi
      \pst@Verb{%
        { [ 1 0
            \pst@cos\space \ifnum\pst@quadrant>\@ne neg \fi
            \pst@sin\space
            \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
            \ifodd\pst@quadrant exch \fi
            0 0
          ] concat
        } \tx@TMChange}%
      \box\pst@hbox
      \pst@Verb{\tx@TMRestore}%
      \kern\pst@dima}%
  \endgroup}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psTilt}
%    \begin{macrocode}
\def\psTilt#1{\pst@makebox{\psTilt@{#1}}}
\def\psTilt@#1{%
  \begingroup
    \leavevmode
    \pst@getsinandcos{#1}%
    \hbox{%
      \ifodd\pst@quadrant
        \pst@@divide{\dp\pst@hbox}{\pst@cos\p@}%
        \ifnum\pst@quadrant=\thr@@\kern\else\pst@dima=\fi\pst@sin\pst@dimg
        \pst@@divide{\ht\pst@hbox}{\pst@cos\p@}%
        \ifnum\pst@quadrant=\@ne\kern\else\pst@dima=\fi\pst@sin\pst@dimg
      \else
        \ifdim\pst@sin\p@=\z@
          \@pstrickserr{\string\psTilt\space angle cannot be 0 or 180}\@ehpa
          \def\pst@sin{.7071}%
          \def\pst@cos{.7071}%
        \fi
        \pst@@divide{\dp\pst@hbox}{\pst@sin\p@}%
        \ifnum\pst@quadrant=\z@\kern\else\pst@dima=\fi\pst@cos\pst@dimg
        \pst@@divide{\ht\pst@hbox}{\pst@sin\p@}%
        \ifnum\pst@quadrant=\tw@\kern\else\pst@dima=\fi\pst@cos\pst@dimg
      \fi
      \ifnum\pst@quadrant>\@ne
        \pst@dimg=\ht\pst@hbox
        \ht\pst@hbox=\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \fi
      \pst@Verb{%
        { [ 1 0
            \pst@cos\space \pst@sin\space
            \ifodd\pst@quadrant exch \fi
            \tx@Div
            \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
            \ifnum\pst@quadrant>\@ne -1 \else 1 \fi
            0 0
          ] concat
        } \tx@TMChange}%
      \box\pst@hbox
      \pst@Verb{\tx@TMRestore}%
      \kern\pst@dima}%
  \endgroup}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psset@Tshadowsize,\psTshadowsize}
%    \begin{macrocode}
\def\psset@Tshadowsize#1{\pst@checknum{#1}\psTshadowsize}
\psset@Tshadowsize{1}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psset@Tshadowangle,\psk@Tshadowangle}
%    \begin{macrocode}
\def\psset@Tshadowangle#1{\pst@getangle{#1}\psk@Tshadowangle}
\psset@Tshadowangle{60}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psset@Tshadowcolor,\psTshadowcolor}
%    \begin{macrocode}
\def\psset@Tshadowcolor#1{\pst@getcolor{#1}\psTshadowcolor}
\psset@Tshadowcolor{lightgray}
%    \end{macrocode}
% \end{macro}
%
% \begin{macro}{\psshadow}
%    \begin{macrocode}
\def\psshadow{\def\pst@par{}\pst@object{psshadow}}
\def\psshadow@i{\pst@makebox{\psshadow@ii}}
\def\psshadow@ii{%
  \begingroup
    \use@par
    \leavevmode
    \pst@getsinandcos{\psk@Tshadowangle}%
    \hbox{%
      \lower\dp\pst@hbox\hbox{%
        \pst@Verb{%
          { [ 1 0
              \pst@cos\space \psTshadowsize mul
              \ifnum\pst@quadrant>\@ne neg \fi
              \pst@sin\space \psTshadowsize mul
              \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
              \ifodd\pst@quadrant exch \fi
              0 0
            ] concat
          } \tx@TMChange}}%
      \hbox to\z@{{\@nameuse{\psTshadowcolor}\copy\pst@hbox\hss}}%
      \pst@Verb{\tx@TMRestore}%
      \box\pst@hbox}%
  \endgroup}
%    \end{macrocode}
% \end{macro}

\catcode`\@=\TheAtCode\relax

\endinput
%%
%% END pst-3d.tex


==> texmf/tex/latex/pstricks/pst-blur.tex <==
%%
%% This is file `pst-blur.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-blur.dtx  (with options: `texfile')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-blur.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-blur.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\def\pstblurfileversion{1.0}
\def\pstblurfiledate{98/09/15}
\message{ v\pstblurfileversion, \pstblurfiledate}
\csname PstBlurLoaded\endcsname
\let\PstBlurLoaded\endinput
\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }\expandafter\next
\fi
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
\pstheader{pst-blur.pro}
\newif\ifpsblur
\def\psset@blur#1{\@nameuse{psblur#1}\pst@setrepeatarrowsflag}
\psset@blur{false}

\def\psset@blurradius#1{\pst@getlength{#1}\psx@blurradius}
\psset@blurradius{1.5pt}

\def\psset@blursteps#1{\pst@getint{#1}\psx@blursteps}
\psset@blursteps{20}

\def\psset@blurbg#1{\pst@getcolor{#1}\psx@blurbg}
\psset@blurbg{white}
\def\pst@closedshadow{%
\ifpsblur\pst@blurclosedshadow\else\pst@sharpclosedshadow\fi
}
\def\pst@sharpclosedshadow{%
\addto@pscode{%
gsave
\psk@shadowsize \psk@shadowangle \tx@PtoC
\tx@Shadow
\pst@usecolor\psshadowcolor
gsave fill grestore
stroke
grestore
gsave
\pst@usecolor\psfillcolor
gsave fill grestore
stroke
grestore}}
\def\pst@blurclosedshadow{%
\addto@pscode{%
gsave
gsave \pst@usecolor\psshadowcolor currentrgbcolor grestore
gsave \pst@usecolor\psx@blurbg currentrgbcolor grestore
\psx@blurradius\space
\psx@blursteps\space
\psk@shadowsize \psk@shadowangle \tx@PtoC
tx@PstBlurDict begin BlurShadow end
grestore
gsave
\pst@usecolor\psfillcolor
gsave fill grestore
stroke
grestore
}}
\def\psblurbox{%
\def\pst@par{}\pst@object{psblurbox}}
\def\psblurbox@i{\pst@makebox\psblurbox@ii}
\def\psblurbox@ii{%
\begingroup
\pst@useboxpar
\psblurtrue
\psshadowtrue
\psboxseptrue
\setbox\pst@hbox=\hbox{\psframebox@ii}%
\pst@dimh=\psk@shadowsize\p@
\pst@dimh=.7071\pst@dimh
\advance\pst@dimh\psx@blurradius\p@
\pst@dimg=\dp\pst@hbox
\advance\pst@dimg\pst@dimh
\dp\pst@hbox=\pst@dimg
\pst@dimg=\wd\pst@hbox
\advance\pst@dimg\pst@dimh
\wd\pst@hbox=\pst@dimg
\leavevmode
\box\pst@hbox
\endgroup}

\catcode`\@=\TheAtCode\relax
\endinput
%%
%% End of file `pst-blur.tex'.


==> texmf/tex/latex/pstricks/pst-char.tex <==
%% BEGIN pst-char.tex
%%
%% Stroking and filling characters with line and fill styles with PSTricks 97.
%% See the PSTricks User's Guide for description.
%% See chartest.tex for sample input.
%%
\def\fileversion{97 patch 3}
\def\filedate{1999/03/11}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\message{ v\fileversion, \filedate}

\csname PSTcharpathLoaded\endcsname
\let\PSTcharpathLoaded\endinput

\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex}
  \expandafter\next
\fi

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

\def\tx@CharPathShow{%
  /tx@CharPathSavedShow /show load def
  /show {
    % These 3 lines check whether charpath yields anything interesting.
    dup gsave newpath 0 0 moveto
    true charpath pathbbox grestore
    3 -1 roll eq 3 1 roll eq and
    % If not, just use show.
    { tx@CharPathSavedShow }
    % Otherwise, use charpath.
    { true charpath }
    ifelse }
  def }

\def\pscharpath{\def\pst@par{}\pst@object{pscharpath}}
\def\pscharpath@i{\pst@makebox\pscharpath@ii}
\def\pscharpath@ii{%
  \leavevmode\hbox{%
    \pstVerb{\tx@CharPathShow}%
    \box\pst@hbox
    \pstVerb{/show /tx@CharPathSavedShow load def}%
% DG/SR modification begin - Nov. 26, 1998 - Patch 2
% \if@star is true but \solid@star must not be executed in \begin@ClosedObj !
%    \begin@ClosedObj
    \let\solid@starOLD\solid@star
    \let\solid@star\relax
    \begin@ClosedObj
    \let\solid@star\solid@starOLD
% DG/SR modification end
      \def\pst@linetype{1}%
      \psdashadjustfalse
      \showpointsfalse
      \let\pst@newpath\@empty
      \def\use@pscode{%
        \pst@Verb{%
          gsave
            \tx@STV
            \pst@code
          grestore
% DG/SR modification begin - Jul.  3, 1998 / Mar. 11, 1999 - Patches 1 and 3
%          \if@star\else CP newpath moveto \fi}}%
          \if@star\else CP newpath moveto \fi}%
        \gdef\pst@code{}}%
% DG/SR modification end
    \end@ClosedObj}}

\def\pscharclip{\def\pst@par{}\pst@object{pscharclip}}
\def\pscharclip@i{\pst@makebox\pscharclip@ii}
\def\pscharclip@ii{%
  \leavevmode
  \begingroup
    \begin@psclip
    {\@startrue\pscharpath@ii}%
    \pstVerb{clip \if@star\else currentpoint newpath moveto\fi}%
    \def\endpscharclip{\end@psclip\endgroup}%
    \ignorespaces}
\def\endpscharclip{\pst@misplaced\endpscharclip}

\catcode`\@=\TheAtCode\relax

\endinput
%%
%% END pst-char.tex


==> texmf/tex/latex/pstricks/pst-coil.tex <==
%% BEGIN pst-coil.tex
%%
%% Coils and zigzags with PSTricks 97.
%% See the PSTricks User's Guide for documentation.
%% For use with the PostScript header file `pst-coil.pro'.
%%
\def\fileversion{97 patch 2}
\def\filedate{1998/03/19}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\message{ v\fileversion, \filedate}
\csname PSTcoilsLoaded\endcsname
\let\PSTcoilsLoaded\endinput
\ifx\PSTricksLoaded\endinput\else
\def\next{\input pstricks.tex}\expandafter\next
\fi
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
\pstheader{pst-coil.pro}
\edef\pst@theheaders{\pst@theheaders,pst-coil.pro}
\def\pst@coildict{tx@CoilDict begin }
\def\psset@coilwidth#1{\pst@getlength{#1}\psk@coilwidth}
\psset@coilwidth{1cm}
\def\psset@coilheight#1{\pst@checknum{#1}\pscoilheight}
\psset@coilheight{1}
\def\psset@coilarmA#1{\pst@getlength{#1}\psk@coilarmA}
\def\psset@coilarmB#1{\pst@getlength{#1}\psk@coilarmB}
\def\psset@coilarm#1{%
\pst@getlength{#1}\psk@coilarmA
\let\psk@coilarmB\psk@coilarmA}
\psset@coilarm{.5cm}
\def\psset@coilaspect#1{\pst@getangle{#1}\psk@coilaspect}
\psset@coilaspect{45}
\def\psset@coilinc#1{\pst@getangle{#1}\psk@coilinc}
\psset@coilinc{10}
\def\pscoil{\def\pst@par{}\pst@object{pscoil}}
\def\pscoil@i{\pst@getarrows\pscoil@ii}
\def\pscoil@ii(#1){%
\@ifnextchar(%
{\pscoil@iii{1}(#1)}%
{\pscoil@iii{\z@}(0,0)(#1)}}
\def\pscoil@iii#1(#2)(#3){%
\begin@OpenObj
\pst@getcoor{#2}\pst@tempa
\pst@getcoor{#3}\pst@tempb
\pst@optcp{#1}\pst@tempa
\addto@pscode{%
\pst@tempa \pst@tempb
\psk@coilwidth \pscoilheight
\psk@coilarmA \psk@coilarmB
\psk@coilaspect \psk@coilinc
\pst@coildict \tx@Coil end}%
\showpointsfalse
\end@OpenObj}
\def\tx@CoilLoop{CoilLoop }
\def\tx@Coil{Coil }
\def\psCoil{\def\pst@par{}\pst@object{psCoil}}
\def\psCoil@i#1#2{%
\begin@AltOpenObj
\showpointsfalse
\pst@getangle{#1}\pst@tempa
\pst@getangle{#2}\pst@tempb
\addto@pscode{%
\pst@tempa
\pst@tempb
\psk@coilwidth
\pscoilheight
\psk@coilaspect
\psk@coilinc
\pst@coildict \tx@AltCoil end
\@nameuse{psls@\pslinestyle}}%
\end@OpenObj}
\def\tx@AltCoil{AltCoil }
\def\pszigzag{\def\pst@par{}\pst@object{pszigzag}}
\def\pszigzag@i{\pst@getarrows\pszigzag@ii}
\def\pszigzag@ii(#1){%
\@ifnextchar({\pszigzag@iii{1}(#1)}{\pszigzag@iii{\z@}(0,0)(#1)}}
\def\pszigzag@iii#1(#2)(#3){%
\begin@OpenObj
\pst@getcoor{#2}\pst@tempa
\pst@getcoor{#3}\pst@tempb
\pst@optcp{#1}\pst@tempa
\addto@pscode{%
\pst@tempa
\pst@tempb
\pscoilheight
\psk@coilwidth
\psk@coilarmA
\psk@coilarmB
\pst@coildict \tx@ZigZag end
\psline@iii
\tx@Line}%
\end@OpenObj}
\def\tx@ZigZag{ZigZag }
\def\nccoil{\pst@object{nccoil}}
\def\nccoil@i{\check@arrow{\nccoil@ii}}
\def\nccoil@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
\tx@NCCoor
tx@Dict begin
% DG/SR modification begin - Mar. 19, 1998 - Patch 2
4 2 roll
% DG/SR modification end
\psk@coilwidth \pscoilheight
\psk@coilarmA \psk@coilarmB
\psk@coilaspect \psk@coilinc
\pst@coildict \tx@Coil end
end}}
\def\pccoil{\def\pst@par{}\pst@object{pccoil}}
\def\pccoil@i{\pc@object\nccoil@ii}
\def\nczigzag{\pst@object{nczigzag}}
\def\nczigzag@i{\check@arrow{\nczigzag@ii}}
\def\nczigzag@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
\tx@NCCoor
tx@Dict begin
% DG/SR modification begin - Mar. 19, 1998 - Patch 2
4 2 roll
% DG/SR modification end
\pscoilheight
\psk@coilwidth
\psk@coilarmA
\psk@coilarmB
\pst@coildict \tx@ZigZag end
\psline@iii
\tx@Line
end}}
\def\pczigzag{\def\pst@par{}\pst@object{pczigzag}}
\def\pczigzag@i{\pc@object\nczigzag@ii}
\catcode`\@=\TheAtCode\relax
\endinput
%%
%% END pst-coil.tex


==> texmf/tex/latex/pstricks/pst-fill.tex <==
%% BEGIN pst-fill.tex
%%
%% Filling and tiling with PSTricks 97.
%%
\def\fileversion{97 patch 2}
\def\filedate{1997/12/12}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%%
%% Note (D.G. - April 8, 97 and November / December 97):
%% * With a \PstTiling macro defined (or "tiling" optional parameter
%%   on \usepackage[tiling]{pst-fill}), this file run exactly as
%%   the original boxfill.tex file from Timothy, version 0.94,
%%   except a correction in \pst@ManualFillCycle to avoid a division by 0.
%%   It's the default.
%% * With a \PstTiling macro defined (or "tiling" optional parameter
%%   on \usepackage[tiling]{pst-fill}) there are several add-ons
%%   and changes to do `tiling' rather than `filling' in "automatic" mode :
%%     - we fix the position of the beginning of tiling,
%%     - we allow normally the framing of the area as expected, using
%%       the line.... parameters
%%     - we define move parameters fillmovex, fillmovey and fillmove,
%%     - we define fillcyclex as previous fillcycle parameter, and add the
%%       fillcycley and fillcycle (both fillcyclex and fillcycley) ones
%%     - we can extend the tiling area using fillloopaddx, fillloopaddy and
%%       fillloopadd parameters,
%%     - we can debug and see the whole tiling area without clipping using
%%       PstDebug parameter,
%%     - for names consistancy, we can use fillangle in place of boxfillangle
%%       and fillsize in place of boxfillsize,
%%     - default value for fillsep is 0 and for fillsize is auto.

% Preliminaries:

\message{ v\fileversion, \filedate}

\csname PSTboxfillLoaded\endcsname
\let\PSTboxfillLoaded\endinput

\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex}
  \expandafter\next
\fi

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

% The box:

\newbox\pst@fillbox
\def\psboxfill{\pst@killglue\pst@makebox\psboxfill@i}
\def\psboxfill@i{\setbox\pst@fillbox\box\pst@hbox\ignorespaces}

% Parameters:

\def\psset@boxfillsize#1{%
  \def\pst@tempg{#1}\def\pst@temph{auto}%
  \ifx\pst@tempg\pst@temph
    \let\psk@boxfillsize\relax
  \else
    \psset@@boxfillsize#1(\z@,\z@)\@empty(\z@,\z@)(\@nil
  \fi}
\def\psset@@boxfillsize#1(#2,#3)#4(#5,#6)#7(#8\@nil{%
  \begingroup
    \ifx\@empty#7\relax
      \pst@dima\z@
      \pst@dimb\z@
      \pssetxlength\pst@dimc{#2}%
      \pssetylength\pst@dimd{#3}%
    \else
      \pssetxlength\pst@dima{#2}%
      \pssetylength\pst@dimb{#3}%
      \pssetxlength\pst@dimc{#5}%
      \pssetylength\pst@dimd{#6}%
    \fi
    \xdef\pst@tempg{%
      \pst@dima=\number\pst@dima sp
      \pst@dimb=\number\pst@dimb sp
      \pst@dimc=\number\pst@dimc sp
      \pst@dimd=\number\pst@dimd sp }%
  \endgroup
  \let\psk@boxfillsize\pst@tempg}

\psset{boxfillsize={(-15cm,-15cm)(15cm,15cm)}}

\def\psset@boxfillcolor#1{\pst@getcolor{#1}\psboxfillcolor}
\psset@boxfillcolor{black}

\def\psset@boxfillangle#1{\pst@getangle{#1}\psk@boxfillangle}
\psset@boxfillangle{0}

\def\psset@fillsepx#1{\pst@getlength{#1}\psk@fillsepx}
\def\psset@fillsepy#1{\pst@getlength{#1}\psk@fillsepy}
\def\psset@fillsep#1{\psset@fillsepx{#1}\let\psk@fillsepy\psk@fillsepx}
\psset@fillsep{2pt}

% DG addition begin - Apr. 8, 1997 and Nov. 1997 - Patch 2
\ifx\PstTiling\@undefined
\def\psset@fillcycle#1{\pst@getint{#1}\psk@fillcycle}
\psset@fillcycle{0}
\else
% For consistancy, use "fill" as prefix for angle and size
\def\psset@fillangle#1{\psset@boxfillangle{#1}}
\def\psset@fillsize#1{\psset{boxfillsize={#1}}}
% Change some default values with better ones for tilings
\psset@fillsep{0}
\psset{fillsize=auto}
% Define fillcyclex (previously fillcycle), fillcycley and fillcycle for both
\def\psset@fillcyclex#1{\pst@getint{#1}\psk@fillcyclex}
\def\psset@fillcycley#1{\pst@getint{#1}\psk@fillcycley}
\def\psset@fillcycle#1{%
\psset@fillcyclex{#1}\let\psk@fillcycley\psk@fillcyclex}
\psset@fillcycle{0}
% Define fillmove, fillmovex and fillmovey parameters
\def\psset@fillmovex#1{\pst@getlength{#1}\psk@fillmovex}
\def\psset@fillmovey#1{\pst@getlength{#1}\psk@fillmovey}
\def\psset@fillmove#1{\psset@fillmovex{#1}\psset@fillmovey{#1}}
\psset@fillmove{0pt}
% Define fillloopaddx, fillloopaddy and fillloopadd parameters
% if tiling is not complete
\def\psset@fillloopaddx#1{\pst@getint{#1}\psk@fillloopaddx}
\def\psset@fillloopaddy#1{\pst@getint{#1}\psk@fillloopaddy}
\def\psset@fillloopadd#1{%
\psset@fillloopaddx{#1}\let\psk@fillloopaddy\psk@fillloopaddx}
\psset@fillloopadd{0}
% For debugging (to debug, set PstDebug=1)
\def\psset@PstDebug#1{\pst@getint{#1}\psk@PstDebug}
\psset@PstDebug{0}
\fi
% DG addition end

% Main macro:

\def\psfs@boxfill{%
  \ifvoid\pst@fillbox
    \@pstrickserr{Fill box is empty. Use \string\psboxfill\space first.}\@ehpa
  \else
    \ifx\psk@boxfillsize\relax
      \pst@AutoBoxFill
    \else
      \pst@ManualBoxFill
    \fi
  \fi}

% Manual box fill:

\def\pst@ManualBoxFill{%
  \leavevmode
  \begingroup
    \pst@FlushCode
    \begin@psclip
    \pstVerb{clip}%
    \expandafter\pst@AddFillBox\psk@boxfillsize
    \end@psclip
  \endgroup}

\def\pst@FlushCode{%
  \pst@Verb{%
    /mtrxc CM def
    CP CP T
    \tx@STV
    \psk@origin
    \psk@swapaxes
    \pst@newpath
    \pst@code
    mtrxc setmatrix
    moveto
    0 setgray}%
  \gdef\pst@code{}}

\def\pst@AddFillBox#1 #2 #3 #4 {%
  \begingroup
    \setbox\pst@fillbox=\vbox{%
      \hbox{\unhcopy\pst@fillbox\kern\psk@fillsepx\p@}%
      \vskip\psk@fillsepy\p@}%
    \psk@boxfillsize
    \pst@cnta=\pst@dimc
    \advance\pst@cnta-\pst@dima
    \divide\pst@cnta\wd\pst@fillbox
    \pst@cntb=\pst@dimd
    \advance\pst@cntb-\pst@dimb
    \pst@dimd=\ht\pst@fillbox
    \divide\pst@cntb\pst@dimd
    \def\pst@tempa{%
      \pst@tempg
      \copy\pst@fillbox
      \advance\pst@cntc\@ne
      \ifnum\pst@cntc<\pst@cntd\expandafter\pst@tempa\fi}%
    \let\pst@tempg\relax
    \pst@cntc-\tw@
    \pst@cntd\pst@cnta
    \setbox\pst@fillbox=\hbox to \z@{%
      \kern\pst@dima
      \kern-\wd\pst@fillbox
      \pst@tempa
      \hss}%
    \pst@cntd\pst@cntb
% DG modification begin - Dec. 11, 1997 - Patch 2
    \ifx\PstTiling\@undefined
      \ifnum\psk@fillcycle=\z@\pst@ManualFillCycle\fi
    \else
      \ifnum\psk@fillcyclex=\z@\pst@ManualFillCycle\fi
    \fi
% DG modification end
    \global\setbox\pst@boxg=\vbox to\z@{%
      \offinterlineskip
      \vss
      \pst@tempa
      \vskip\pst@dimb}%
  \endgroup
  \setbox\pst@fillbox\box\pst@boxg
  \pst@rotate\psk@boxfillangle\pst@fillbox
  \box\pst@fillbox}

\def\pst@ManualFillCycle{%
% DG modification begin - Dec. 11, 1997 - Patch 2
  \ifx\PstTiling\@undefined
    \pst@cntg=\psk@fillcycle
  \else
    \pst@cntg=\psk@fillcyclex
  \fi
% DG modification end
  \pst@dimg=\wd\pst@fillbox
% DG modification begin - Mar. 20, 1997 - Patch 1 (to avoid division by 0)
%  \divide\pst@dimg\pst@cntg
  \ifnum\pst@cntg=\z@
  \else
  \divide\pst@dimg\pst@cntg
  \fi
% DG modification end
  \ifnum\pst@cntg<\z@\pst@cntg=-\pst@cntg\fi
  \advance\pst@cntg\m@ne
  \pst@cnth=\pst@cntg
  \def\pst@tempg{%
    \ifnum\pst@cnth<\pst@cntg\advance\pst@cnth\@ne\else\pst@cnth\z@\fi
    \moveright\pst@cnth\pst@dimg}}

% Auto box fill:        !! Fix dictionary

% DG addition begin - Apr. 8, 1997 and Dec. 1997 - Patch 2
\ifx\PstTiling\@undefined
% DG addition end
% Original version
\pst@def{AutoFillCycle}<%
  /c ED
  /n 0 def
  /s {
    /x x w c div n mul add def
    /n n c abs 1 sub lt { n 1 add } { 0 } ifelse def
  } def>

\pst@def{BoxFill}<%
  gsave
    gsave \tx@STV CM grestore dtransform CM idtransform
    abs /h ED abs /w ED
    pathbbox
    h div round 2 add cvi /y2 ED
    w div round 2 add cvi /x2 ED
    h div round 2 sub cvi /y1 ED
    w div round 2 sub cvi /x1 ED
    /y2 y2 y1 sub def
    /x2 x2 x1 sub def
    CP
    y1 h mul sub neg /y1 ED
    x1 w mul sub neg /x1 ED
    clip
    y2 {
      /x x1 def
      s
      x2 {
        save CP x y1 T moveto Box restore
        /x x w add def
      } repeat
      /y1 y1 h add def
    } repeat
    % Next line not useful... To see that, suppress clipping (DG)
    CP x y1 T moveto Box
  currentpoint currentfont grestore setfont moveto>
\else
% DG modification begin - Apr. 8, 1997 and Nov. / Dec. 1997 - Patch 2
\pst@def{AutoFillCycleX}<%
  /cX ED
  /nX 0 def
  /CycleX {
    /x x w cX div nX mul add def
    /nX nX cX abs 1 sub lt { nX 1 add } { 0 } ifelse def
  } def>
\pst@def{AutoFillCycleY}<%
  /cY ED
  /mY 0 def
  /nY 0 def
  /CycleY {
    /y1 y1 h cY div mY mul sub def
    nY cY abs 1 sub lt { /nY nY 1 add def /mY 1 def }
                       { /nY 0 def        /mY cY abs 1 sub neg def } ifelse
  } def>

\pst@def{BoxFill}<%
  gsave
    gsave \tx@STV CM grestore dtransform CM idtransform
    abs /h ED abs /w ED
    pathbbox
    h div round 2 add cvi /y2 ED
    w div round 2 add cvi /x2 ED
    h div round 2 sub cvi /y1 ED
    w div round 2 sub cvi /x1 ED
% We must enlarge the area if fillangle, fillcycle, fillmove or fillsep are used
    /CoefLoopX 0 def
    /CoefLoopY 0 def
    /CoefMoveX 0 def
    /CoefMoveY 0 def
    \psk@boxfillangle 0 ne {/CoefLoopX 8 def /CoefLoopY 8 def} if
    \psk@fillcyclex 0 ne {/CoefLoopX CoefLoopX 1 add def} if
    \psk@fillcycley 0 ne {/CoefLoopY CoefLoopY 1 add def} if
    \psk@fillmovex 0 ne
      {/CoefLoopX CoefLoopX 2 add def
       \psk@fillmovex 0 gt {/CoefMoveX CoefLoopX def}
                           {/CoefMoveX CoefLoopX neg def} ifelse} if
    \psk@fillmovey 0 ne
      {/CoefLoopY CoefLoopY 2 add def
       \psk@fillmovey 0 gt {/CoefMoveY CoefLoopY def}
                           {/CoefMoveY CoefLoopY neg def} ifelse} if
    \psk@fillsepx 0 ne {/CoefLoopX CoefLoopX 1 add def} if
    \psk@fillsepy 0 ne {/CoefLoopY CoefLoopY 1 add def} if
    /CoefLoopX CoefLoopX \psk@fillloopaddx add def
    /CoefLoopY CoefLoopY \psk@fillloopaddy add def
%
    /x2 x2 x1 sub 4 sub CoefLoopX 2 mul add def
    /y2 y2 y1 sub 4 sub CoefLoopY 2 mul add def
% We must fix the origin of tiling, as it must not vary according other stuff
% in the page!
    w x1 CoefLoopX add CoefMoveX add mul
      h y1 y2 add 1 sub CoefLoopY sub CoefMoveY sub mul moveto
%
    CP
    y1 h mul sub neg /y1 ED
    x1 w mul sub neg /x1 ED
    \psk@PstDebug 0 eq {clip} if
    \psk@fillmovex \psk@fillmovey
    gsave \tx@STV CM grestore dtransform CM idtransform
    /hmove ED /wmove ED
%
    /row 0 def
   y2 {
       /row row 1 add def
       /column 0 def
       /x x1 def
       CycleX
       save
       x2 {
          /column column 1 add def
          CycleY
          save CP x y1 T moveto Box restore
          /x x w add def
          0 hmove translate
          } repeat
       restore
       /y1 y1 h add def
       wmove 0 translate
       } repeat
  currentpoint currentfont grestore setfont moveto>
\fi
% DG modification end

\def\pst@AutoBoxFill{%
  \leavevmode
  \begingroup
% DG addition begin - Dec. 2, 1997 - Patch 2
    \pst@stroke
% DG addition end
    \pst@FlushCode
    \pst@Verb{\psk@boxfillangle \tx@RotBegin}%
    \pstVerb{\pst@dict /Box \pslbrace end}%
% DG addition begin - Apr. 8, 1997 and Nov. 5, 1997 - Patch 2
% Useful when the starting point is not (0,0)
    \ifx\PstTiling\@undefined
    \else
      \ifx\pst@tempa\@undefined % Undefined for instance for \pscharpath
      \else
        \def\pst@temph{0}%
        \ifx\pst@tempa\pst@temph
        \else
          \pstVerb{/TR{pop pop currentpoint translate \pst@tempa translate}def}%
        \fi
      \fi
    \fi
% DG addition end
    \hbox to \z@{\vbox to\z@{\vss\copy\pst@fillbox\vskip-\dp\pst@fillbox}\hss}%
% DG addition begin - Dec. 8, 1997 - Patch 2
    \ifx\PstTiling\@undefined
% DG addition end
      \pstVerb{%
        tx@Dict begin \psrbrace def
        \ifnum\psk@fillcycle=\z@
          /s {} def
        \else
          \psk@fillcycle \tx@AutoFillCycle
        \fi
        \pst@number{\wd\pst@fillbox}%
        \psk@fillsepx add
        \pst@number{\ht\pst@fillbox}%
        \pst@number{\dp\pst@fillbox}%
        \psk@fillsepy add add
        \tx@BoxFill
        end}%
% DG modification begin - Dec. 8, 1997 - Patch 2
      \else
      \pstVerb{%
        tx@Dict begin \psrbrace def
        \ifnum\psk@fillcyclex=\z@
          /CycleX {} def
        \else
          \psk@fillcyclex \tx@AutoFillCycleX
        \fi
        \ifnum\psk@fillcycley=\z@
          /CycleY {} def
        \else
          \psk@fillcycley \tx@AutoFillCycleY
        \fi
        \pst@number{\wd\pst@fillbox}%
        \psk@fillsepx add
        \pst@number{\ht\pst@fillbox}%
        \pst@number{\dp\pst@fillbox}%
        \psk@fillsepy add add
        \tx@BoxFill
        end}%
      \fi
% DG modification end
    \pst@Verb{\tx@RotEnd}%
  \endgroup}

\catcode`\@=\TheAtCode\relax

\endinput
%%
%% END pst-fill.tex


==> texmf/tex/latex/pstricks/pst-ghsb.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%% -*- Mode: Plain-Tex -*- %%%%%%%%%%%%%%%%%%%%%%%%%%
%% pst-ghsb.tex --- For the PSTricks HSB mode gradient fillstyle
%%                  Based on pst-grad.tex from Timothy van Zandt
%%
%%                  Take care that Hue value is cyclic, so 1=0 !
%%
%% Author          : Denis GIROU (CNRS/IDRIS - France) <Denis.Girou@idris.fr>
%% Created the     : Tue May 13 11:12:36 1997
%% Last mod. by    : Denis GIROU (CNRS/IDRIS - France) <Denis.Girou@idris.fr>
%% Last mod. the   : Thu Jan 29 17:20:13 1998
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\fileversion{1.0}
\def\filedate{1997/05/13}

%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.

% This defines a new fill style, "gradient", for use with PSTricks,
% which has gradiated color. The following parameters are used:
%
%    gradbegin=color    : Beginning color.
%    gradend=color      : Final color.
%    gradlines=int      : Number of lines to use. The higher the number,
%                           the slower the rendering.
%    gradmidpoint=num   : Gradient color goes from gradbegin to gradend,
%                           and then back to beginning. Midpoint (point
%                           where "gradend" color appears, is gradmidpoint
%                           from the top.  (0 <= Gmidpoint <= 1).
%    gradangle=angle    : Rotate image by angle.

\message{ v\fileversion, \filedate}

\csname GradientHSBLoaded\endcsname
\let\GradientHSBLoaded\endinput

\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }\expandafter\next
\fi

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

\pstheader{pst-ghsb.pro}

\newrgbcolor{gradbegin}{0 .1 .95}
\def\psset@gradbegin#1{\pst@getcolor{#1}\psgradbegin}
\psset@gradbegin{gradbegin}

\newrgbcolor{gradend}{0 1 1}
\def\psset@gradend#1{\pst@getcolor{#1}\psgradend}
\psset@gradend{gradend}

\def\psset@gradlines#1{%
  \pst@getint{#1}\psgradlines
  \ifnum\psgradlines<2
    \@pstrickserr{gradlines must be at least 2}\@epha
    \def\psgradlines{2 }%
  \fi}
\psset@gradlines{300}

\def\psset@gradmidpoint#1{\pst@checknum{#1}\psgradmidpoint}
\psset@gradmidpoint{.9}

\def\psset@gradangle#1{\pst@getangle{#1}\psk@gradangle}
\psset@gradangle{0}

\newif\ifgradientHSB
\def\psset@gradientHSB#1{\@nameuse{gradientHSB#1}}
\psset@gradientHSB{false}

\def\psfs@gradient{%
\ifgradientHSB
\addto@pscode{gsave
    gsave \pst@usecolor\psgradbegin currenthsbcolor grestore
    gsave \pst@usecolor\psgradend currenthsbcolor grestore
    \psgradlines
    \psgradmidpoint
    \psk@gradangle
    tx@GradientHSBDict begin GradientFillHSB end grestore}
\else
\addto@pscode{gsave
    gsave \pst@usecolor\psgradbegin currentrgbcolor grestore
    gsave \pst@usecolor\psgradend currentrgbcolor grestore
    \psgradlines
    \psgradmidpoint
    \psk@gradangle
    tx@GradientDict begin GradientFill end grestore}
\fi}

\catcode`\@=\TheAtCode\relax
\endinput
%% END pst-ghsb.tex


==> texmf/tex/latex/pstricks/pst-gr3d.tex <==
%%
%% This is file `pst-gr3d.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-gr3d.dtx  (with options: `pst-gr3d')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-gr3d.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-gr3d.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% Package `pst-gr3d.ins'
%%
%% Denis Girou (CNRS/IDRIS - France) <Denis.Girou@idris.fr>
%% September 16, 1998
%%
%%
%% Denis Girou, <Denis.Girou@idris.fr>, 1998.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-gr3d' is PSTricks package to draw three dimensional grids
%%   with various customizations.
%%
\def\fileversion{1.2}
\def\filedate{98/09/16}
\message{`PST-Grids3d v\fileversion, \filedate\space (Denis Girou)}
\csname PSTGridsThreeD\endcsname
\let\PSTGridsThreeD\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
\ifx\PSTthreeDLoaded\endinput\else\input pst-3d.tex\fi
\ifx\MultidoLoaded\endinput\else\input multido.tex\fi
\input pst-key.tex
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
\def\psset@PstDebug#1{\pst@getint{#1}\psk@PstDebug}
\newif\ifPst@PstPicture
\define@key{psset}{PstPicture}[true]{\@nameuse{Pst@PstPicture#1}}
\newif\ifPst@GridThreeDNodes
\define@key{psset}{GridThreeDNodes}[true]{\@nameuse{Pst@GridThreeDNodes#1}}
\define@key{psset}{GridThreeDXUnit}{%
\pst@cntg=#1\relax
\edef\psk@GridThreeDXUnit{\the\pst@cntg}}
\define@key{psset}{GridThreeDYUnit}{%
\pst@cntg=#1\relax
\edef\psk@GridThreeDYUnit{\the\pst@cntg}}
\define@key{psset}{GridThreeDZUnit}{%
\pst@cntg=#1\relax
\edef\psk@GridThreeDZUnit{\the\pst@cntg}}
\define@key{psset}{GridThreeDXPos}{%
\pst@cntg=#1\relax
\edef\psk@GridThreeDXPos{\the\pst@cntg}}
\define@key{psset}{GridThreeDYPos}{%
\pst@cntg=#1\relax
\edef\psk@GridThreeDYPos{\the\pst@cntg}}
\define@key{psset}{GridThreeDZPos}{%
\pst@cntg=#1\relax
\edef\psk@GridThreeDZPos{\the\pst@cntg}}
\def\psset@Rx#1{\psset@XnodesepA{#1}}
\def\psset@Ry#1{\psset@offsetA{#1}}
\psset@viewpoint{1.2 -0.6 0.8}
\setkeys{psset}{%
PstDebug=0,PstPicture=true,GridThreeDNodes=false,
GridThreeDXPos=1,GridThreeDYPos=1,GridThreeDZPos=1,
GridThreeDXUnit=1,GridThreeDYUnit=1,GridThreeDZUnit=1}
\def\PstGridThreeD{%
\@ifnextchar[\@PstGridThreeD{\@PstGridThreeD[]}}
\def\@PstGridThreeD[#1](#2,#3,#4){{%
\psset{dimen=middle}%
\setkeys{psset}{#1}%
\pst@cnta=#2
\advance\pst@cnta\m@ne
\pst@cnth=\pst@cnta
\multiply\pst@cnth\psk@GridThreeDXUnit
\divide\pst@cnth\tw@
\ifodd\pst@cnth
  \edef\Pst@PictureYmin{-\the\pst@cnth}%
\else
  \edef\Pst@PictureYmin{-\the\pst@cnth.5}%
\fi
\pst@cntb=#3
\advance\pst@cntb\m@ne
\pst@cntc=#4
\advance\pst@cntc\m@ne
\pst@cntg=\pst@cntb
\multiply\pst@cntg\psk@GridThreeDYUnit
\divide\pst@cnta\tw@
\pst@cnth=\pst@cnta
\multiply\pst@cnth\psk@GridThreeDXUnit
\advance\pst@cntg\pst@cnth
\pst@cnth=\pst@cntb
\advance\pst@cnth\m@ne
\multiply\pst@cnth\psk@GridThreeDYUnit
\divide\pst@cnth\tw@
\pst@cntd=\pst@cntc
\multiply\pst@cntd\psk@GridThreeDZUnit
\advance\pst@cntd\pst@cnth
\ifnum\pst@cnth=\z@
  \edef\Pst@PictureYmax{\the\pst@cntd.5}%
\else
  \edef\Pst@PictureYmax{\the\pst@cntd}%
\fi
\ifPst@PstPicture
  \ifnum\psk@PstDebug>\z@
    \psframebox[framesep=0]{%
  \fi
  \pspicture(0,\Pst@PictureYmin)(\the\pst@cntg,\Pst@PictureYmax)
\fi
\pst@cntd=\psk@GridThreeDXPos
\advance\pst@cntd\m@ne
\multiply\pst@cntd\psk@GridThreeDXUnit
\pst@cntg=\psk@GridThreeDYPos
\advance\pst@cntg\m@ne
\multiply\pst@cntg\psk@GridThreeDYUnit
\pst@cnth=\psk@GridThreeDZPos
\advance\pst@cnth\m@ne
\multiply\pst@cnth\psk@GridThreeDZUnit
\ifx\PstGridThreeDHookZFace\empty
\else
  \multido{\iz=\pst@cntc+-\psk@GridThreeDZUnit}{#4}{% Z face hook
    \ThreeDput[normal=0 0 1](\pst@cntd,\pst@cntg,\iz){\PstGridThreeDHookZFace}}
\fi
\multido{\ix=\pst@cntd+\psk@GridThreeDXUnit}{#2}{%
  \ThreeDput[normal=1 0 0](\ix,\pst@cntg,\pst@cnth){%
    \PstGridThreeDHookXFace
    \psgrid[xunit=\psk@GridThreeDYUnit,yunit=\psk@GridThreeDZUnit,
            subgriddiv=0,gridlabels=0](\pst@cntb,\pst@cntc)}}
\pst@cnta=#3
\advance\pst@cnta\m@ne
\multiply\pst@cnta\psk@GridThreeDYUnit
\advance\pst@cnta\pst@cntg
\multido{\iy=\pst@cnta+-\psk@GridThreeDYUnit}{#3}{%
  \ThreeDput[normal=0 1 0](\pst@cntd,\iy,\pst@cnth){%
    \PstGridThreeDYFace{#2}{#4}{\iy}}}
\PstGridThreeD@HookEnd

\ifPst@PstPicture
  \endpspicture
  \ifnum\psk@PstDebug>\z@
    }
  \fi
\fi}}
\def\PstGridThreeDYFace#1#2#3{%
\pst@cnta=#1
\advance\pst@cnta\m@ne
\pst@cntb=#2
\advance\pst@cntb\m@ne
\PstGridThreeDHookYFace%
\psgrid[xunit=\psk@GridThreeDXUnit,yunit=\psk@GridThreeDZUnit,
        subgriddiv=0,gridlabels=0](-\pst@cnta,\pst@cntb)
\pst@cntg=#3%
\advance\pst@cntg\@ne
\multido{\ia=0+-\psk@GridThreeDXUnit}{#1}{%
  \pst@cnth=\multidocount
  \multido{\ib=0+\psk@GridThreeDZUnit}{#2}{%
    \ifPst@GridThreeDNodes
      \pnode(\ia,\ib){Gr3dNode\the\pst@cnth\the\pst@cntg\the\multidocount}
    \fi
    \ifx\PstGridThreeDHookNode\empty
    \else
      \rput(\ia,\ib){\PstGridThreeDHookNode}
    \fi}}}
\def\PstGridThreeDHookNode{}
\def\PstGridThreeDHookXFace{}
\def\PstGridThreeDHookYFace{}
\def\PstGridThreeDHookZFace{}
\def\PstGridThreeDHookEnd{}
\def\PstGridThreeD@HookEnd{%
\def\PstGridThreeD@HookEnd{}%
\PstGridThreeDHookEnd}
\def\PstGridThreeDNodeProcessor#1{%
\psset{unit=0.3}
\pspicture(-0.5,-0.5)(0.5,0.5)
  \pscircle*[linecolor=#1]{0.5}
  \pscircle*[linecolor=white]{0.2}
\endpspicture}
\catcode`\@=\PstAtCode\relax
\endinput
%%
%% End of file `pst-gr3d.tex'.


==> texmf/tex/latex/pstricks/pst-grad.tex <==
%% BEGIN pst-grad.tex
%%
%% Gradient fillstyle with PSTricks 97.
%% See the PSTricks User's Guide for description.
%% This uses the header file `pst-grad.pro'.
%%
%% Based on some EPS files by leeweyr!bill@nuchat.sccsi.com (W. R. Lee).
%%
\def\fileversion{97 patch 1}
\def\filedate{1997/04/28}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%% This defines a new fill style, "gradient", for use with PSTricks,
%% which has gradiated color. The following parameters are used:
%%
%%    gradbegin=color    : Beginning color.
%%    gradend=color      : Final color.
%%    gradlines=int      : Number of lines to use. The higher the number,
%%                           the slower the rendering.
%%    gradmidpoint=num   : Gradient color goes from gradbegin to gradend,
%%                           and then back to beginning. Midpoint (point
%%                           where "gradend" color appears, is gradmidpoint
%%                           from the top.  (0 <= Gmidpoint <= 1).
%%    gradangle=angle    : Rotate image by angle.

\message{ v\fileversion, \filedate}

\csname GradientLoaded\endcsname
\let\GradientLoaded\endinput

\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }\expandafter\next
\fi

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

\pstheader{pst-grad.pro}

\newrgbcolor{gradbegin}{0 .1 .95}
\def\psset@gradbegin#1{\pst@getcolor{#1}\psgradbegin}
\psset@gradbegin{gradbegin}

\newrgbcolor{gradend}{0 1 1}
\def\psset@gradend#1{\pst@getcolor{#1}\psgradend}
\psset@gradend{gradend}

\def\psset@gradlines#1{%
  \pst@getint{#1}\psgradlines
  \ifnum\psgradlines<2
    \@pstrickserr{gradlines must be at least 2}\@epha
    \def\psgradlines{2 }%
  \fi}
\psset@gradlines{300}

\def\psset@gradmidpoint#1{\pst@checknum{#1}\psgradmidpoint}
\psset@gradmidpoint{.9}

\def\psset@gradangle#1{\pst@getangle{#1}\psk@gradangle}
\psset@gradangle{0}

\def\psfs@gradient{%
  %\pst@fill{%
\addto@pscode{gsave
    gsave \pst@usecolor\psgradbegin currentrgbcolor grestore
    gsave \pst@usecolor\psgradend currentrgbcolor grestore
    \psgradlines
    \psgradmidpoint
    \psk@gradangle
    tx@GradientDict begin GradientFill end grestore}}

\catcode`\@=\TheAtCode\relax

\endinput
%%
%% END pst-grad.tex


==> texmf/tex/latex/pstricks/pst-node.tex <==
%% BEGIN pst-node.tex
%%
%% Nodes with PSTricks 97.
%% See the betadoc documentation for usage. 
%% This uses the header file `pst-node.pro'.
%%
\def\fileversion{97 patch 8}
\def\filedate{1998/11/27}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\message{ v\fileversion, \filedate}
\csname PSTnodesLoaded\endcsname
\let\PSTnodesLoaded\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi\relax
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
\pstheader{pst-node.pro}
\def\pst@nodedict{tx@NodeDict begin }
\def\pst@zapspace#1 #2{%
#1%
\ifx#2\@empty\else\expandafter\pst@zapspace\fi
#2}
\def\pst@getnode#1#2{%
\pst@expandafter\pst@@getnode{#1},,\@nil#2}
\def\pst@@getnode#1,#2,#3\@nil#4{%
\ifx\@empty#3\@empty
\edef#4{/N@\pst@zapspace#1 \@empty\space}%
\else
\pst@cntg=#1\relax
\pst@cnth=#2\relax
\edef#4{/N@M-\ifnum\psmatrixcnt=\z@ 1\else\the\psmatrixcnt\fi
-\the\pst@cntg-\the\pst@cnth\space}%
\fi}
\def\tx@NewNode{NewNode }
\def\pst@newnode#1#2#3#4{%
\leavevmode
\pst@getnode{#1}\pst@thenode
\pst@Verb{%
\pst@nodedict
{#3}
\ifx\psk@name\relax false \else \psk@name true \fi
\pst@thenode
#2
{#4}
\tx@NewNode
end}%
\global\let\psk@name\relax
\pstree@nodehook
\global\let\pstree@nodehook\relax}
\let\pstree@nodehook\relax
\newif\ifnodealign
\def\psset@nodealign#1{\@nameuse{nodealign#1}}
\psset@nodealign{false}
\def\pst@nodealign{%
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg-\dp\pst@hbox
\divide\pst@dimg2
\lower\pst@dimg}
\def\tx@InitPnode{InitPnode }
\def\pnode{\@ifnextchar({\pnode@}{\pnode@(0,0)}}
\def\pnode@(#1)#2{%
\pst@@getcoor{#1}%
\pst@newnode{#2}{10}{\pst@coor}{\tx@InitPnode}%
\ignorespaces}
\def\tx@InitCnode{InitCnode }
\def\cnode{\pst@object{cnode}}
\def\cnode@i{\@ifnextchar({\cnode@ii}{\cnode@ii(0,0)}}
\def\cnode@ii(#1)#2#3{%
\leavevmode
\hbox{%
\use@par
\pst@@getcoor{#1}%
\pssetlength\pst@dimc{#2}%
\pst@dimg=\psk@dimen\pslinewidth
\advance\pst@dimc-\pst@dimg
\advance\pst@dimc.5\pslinewidth
\ifnodealign
\kern\pst@dimc
\vrule width\z@ height \pst@dimc depth \pst@dimc
\fi
\pscircle@do(#1){#2}%
\pst@newnode{#3}{11}{\pst@coor \pst@number\pst@dimc}{\tx@InitCnode}%
% DG/SR modification begin - Jul. 30, 1997 - Patch 2
%\ifnodealign \kern\pst@dimc\egroup \fi}%
\ifnodealign\kern\pst@dimc\fi}%
% DG/SR modification end
\ignorespaces}
\def\Cnode{\pst@object{Cnode}}
\def\Cnode@i{\@ifnextchar({\Cnode@ii}{\Cnode@ii(0,0)}}
\def\Cnode@ii(#1)#2{\cnode@ii(#1){\psk@radius}{#2}}%
\def\cnodeput{\pst@object{cnodeput}}
\def\cnodeput@i{\@ifnextchar({\cnodeput@iii}{\cnodeput@ii}}
\def\cnodeput@ii#1{%
\addto@par{rot={#1}}%
\@ifnextchar({\cnodeput@iii}{\cnodeput@iii(\z@,\z@)}}
\def\cnodeput@iii(#1)#2{%
\pst@killglue
\@fixedradiusfalse
\def\pst@nodehook{\cnodeput@iv{#2}}%
\pst@makebox{\cput@v{#1}}}
\def\cnodeput@iv#1{%
\pst@newnode{#1}{11}{\pscirclebox@iv \pst@number\pslinewidth add}%
{\tx@InitCnode}%
\global\let\pst@nodehook\relax}
\def\Cnodeput{\pst@object{Cnodeput}}
\def\Cnodeput@i{\@ifnextchar({\Cnodeput@iii}{\Cnodeput@ii}}
\def\Cnodeput@ii#1{%
\addto@par{rot={#1}}%
\@ifnextchar({\Cnodeput@iii}{\Cnodeput@iii(\z@,\z@)}}
\def\Cnodeput@iii(#1)#2{%
\pst@killglue
\@fixedradiustrue
\def\pst@nodehook{\Cnodeput@iv{#2}}%
\pst@makebox{\cput@iv{#1}}}
\def\Cnodeput@iv#1{%
\pst@newnode{#1}{11}{%
\pst@number{\wd\pst@hbox} 2 div \pst@number\pst@dima % x y
\pst@number\pst@dimb \pst@number\pslinewidth \psk@dimen .5 sub mul sub }% r
{\tx@InitCnode}%
\global\let\pst@nodehook\relax}
\def\circlenode{\pst@object{circlenode}}
\def\circlenode@i#1{\pst@makebox{\circlenode@ii{#1}}}
\def\circlenode@ii#1{%
\begingroup
\pst@useboxpar
\setbox\pst@hbox=\hbox{%
\cnodeput@iv{#1}%
\pscirclebox@iii
\box\pst@hbox}%
\ifnodealign \psboxseptrue \fi
\ifpsboxsep \pscirclebox@sep \fi
\leavevmode
\ifnodealign\pst@nodealign\fi
\box\pst@hbox
\endgroup}
\def\Circlenode{\pst@object{Circlenode}}
\def\Circlenode@i#1{\pst@makebox{\Circlenode@ii{#1}}}
\def\Circlenode@ii#1{%
\begingroup
\pst@useboxpar
\pst@dima=\ht\pst@hbox
\advance\pst@dima\dp\pst@hbox
\divide\pst@dima\tw@
\pssetlength\pst@dimb\psk@radius
\setbox\pst@hbox=\hbox{%
\Cnodeput@iv{#1}%
\pscircle(.5\wd\pst@hbox,\pst@dima){\pst@dimb}%
\box\pst@hbox}%
\ifnodealign \psboxseptrue \fi
\ifpsboxsep \psCirclebox@sep \fi
\leavevmode
\ifnodealign\pst@nodealign\fi
\box\pst@hbox
\endgroup}
\def\tx@GetRnodePos{GetRnodePos }
\def\tx@InitRnode{InitRnode }
\def\rnode{\@ifnextchar[{\rnode@i}{\def\pst@par{}\rnode@ii}}
\def\rnode@i[#1]{\def\pst@par{ref=#1}\rnode@ii}
\def\rnode@ii#1{\pst@makebox{\rnode@iii\rnode@iv{#1}}}
\def\rnode@iii#1#2{%
% DG modification begin - Jan. 1997
\leavevmode
% DG modification end
\begingroup
% DG/SR modification begin - Apr. 28, 1998 - Patch 6
\pst@useboxpar
% DG/SR modification end
#1%
\if@star\pst@starbox\fi
\ifnodealign\lower\pst@dimb\fi
\hbox{%
\pst@newnode{#2}{16}{%
\pst@number{\ht\pst@hbox}%
\pst@number{\dp\pst@hbox}%
\pst@number{\wd\pst@hbox}%
\pst@number\pst@dima
\pst@number\pst@dimb}%
{\tx@InitRnode}%
\box\pst@hbox}%
\endgroup}
\def\rnode@iv{%
\pst@dima=\psk@xref\wd\pst@hbox
\ifx\psk@yref\relax
\pst@dimb=\z@
\else
\pst@dimb=\ht\pst@hbox
\advance\pst@dimb\dp\pst@hbox
\pst@dimb=\psk@yref\pst@dimb
\advance\pst@dimb-\dp\pst@hbox
\fi}
\def\psset@href#1{\pst@checknum{#1}\psk@href}
\psset@href{0}
\def\psset@vref#1{\def\psk@vref{#1}}
\psset@vref{.7ex}
\def\Rnode{\pst@object{Rnode}}
\def\Rnode@i#1{\pst@makebox{\rnode@iii\Rnode@ii{#1}}}
\def\Rnode@ii{%
% DG modification begin - Jan. 1997
%   - \begingroup removed  as it seems to doesn't work any more
%   - \Rnode doesn't process the optional parameter changes
%\begingroup
\use@par
% DG modification end
\pst@dima=\psk@href\wd\pst@hbox
\advance\pst@dima\wd\pst@hbox
\divide\pst@dima 2
\pssetlength\pst@dimb{\psk@vref}}
\def\tx@DiaNodePos{DiaNodePos }
\def\dianode{\pst@object{dianode}}
\def\dianode@i#1{\pst@makebox{\dianode@ii{#1}}}
\def\dianode@ii#1{%
\begingroup
\pst@useboxpar
\psdiabox@iii
\setbox\pst@hbox=\hbox{%
\pst@newnode{#1}{14}{}{%
/X \pst@number\pst@dima def
/Y \pst@number\pst@dimb def
/w \pst@number\pst@dimc 2 mul def
/h \pst@number\pst@dimd 2 mul def
/NodePos { \tx@DiaNodePos } def}%
\box\pst@hbox}%
\ifnodealign\psboxseptrue\fi
\ifpsboxsep\psdiabox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
\leavevmode
% DG/SR modification end
\ifnodealign\lower\pst@dimb\fi
\box\pst@hbox
\endgroup}
\def\tx@TriNodePos{TriNodePos }
\def\tx@InitTriNode{InitTriNode }
\def\trinode{\pst@object{trinode}}
\def\trinode@i#1{\pst@makebox{\trinode@ii{#1}}}
\def\trinode@ii#1{%
\begingroup
\pst@useboxpar
\pstribox@iii
\setbox\pst@hbox=\hbox{%
\pst@newnode{#1}{14}{}{%
\pst@number\pst@dimc
\pst@number\pst@dimd
\ifodd\psk@trimode
exch
\pst@number\pst@dima
\else
\pst@number\pst@dimb
\fi
\psk@trimode
\pst@number{\wd\pst@hbox}%
\pst@number{\ht\pst@hbox}%
\pst@number{\dp\pst@hbox}%
\tx@InitTriNode}%
\box\pst@hbox}%
\ifnodealign\psboxseptrue\fi
\ifpsboxsep\pstribox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
\leavevmode
% DG/SR modification end
\ifnodealign\lower\pst@tempa\fi
\box\pst@hbox
\endgroup}
\def\tx@OvalNodePos{OvalNodePos }
\def\ovalnode{\pst@object{ovalnode}}
\def\ovalnode@i#1{\pst@makebox{\ovalnode@ii{#1}}}
\def\ovalnode@ii#1{%
\begingroup
\pst@useboxpar
\psovalbox@iii
\setbox\pst@hbox=\hbox{%
\pst@newnode{#1}{14}{}{%
/X \pst@number\pst@dima def
/Y \pst@number\pst@dimb def
/w \pst@number\pst@dimc def
/h \pst@number\pst@dimd def
/NodePos { \tx@OvalNodePos } def}%
\unhbox\pst@hbox}%
\ifnodealign\psboxseptrue\fi
\ifpsboxsep\psovalbox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
\leavevmode
% DG/SR modification end
\ifnodealign\lower\pst@dimb\fi
\box\pst@hbox
\endgroup}
\def\dotnode{\pst@object{dotnode}}
\def\dotnode@i{\@ifnextchar({\dotnode@ii}{\dotnode@ii(\z@,\z@)}}
\def\dotnode@ii(#1)#2{%
\leavevmode
\hbox{%
\use@par
\pst@@getcoor{#1}%
\pst@getdotsize
\pstree@nodehook
\ifnodealign
\pst@dima=\pst@dimg
\kern\pst@dima
\vrule width\z@ height \pst@dimh depth \pst@dimh
\fi
\pst@newnode{#2}{14}{}{%
\pst@coor
/Y ED /X ED
/w \pst@number\pst@dimg def
/h \pst@number\pst@dimh def
/NodePos { \tx@OvalNodePos } def}%
\psdot@ii(#1)%
\ifnodealign\kern\pst@dima\fi}%
\ignorespaces}
\def\psset@framesize#1{\pst@expandafter\psset@@framesize{#1} \@nil}
\def\psset@@framesize#1 #2\@nil{%
\pssetlength\pst@dimg{#1}%
\divide\pst@dimg2
\edef\psk@framewidth{\pst@number\pst@dimg}%
\ifx\@empty#2\@empty
\let\psk@frameheight\psk@framewidth
\else
\pssetlength\pst@dimg{#2}%
\divide\pst@dimg2
\edef\psk@frameheight{\pst@number\pst@dimg}%
\fi}
\psset@framesize{10pt}
\def\fnode{\pst@object{fnode}}
\def\fnode@i{\@ifnextchar({\fnode@ii}{\fnode@ii(\z@,\z@)}}
\def\fnode@ii(#1)#2{%
\leavevmode
\pst@killglue
\hbox{%
\use@par
\begin@ClosedObj
\ifnodealign
\kern\psk@framewidth\p@
\vrule width\z@ height \psk@frameheight\p@ depth \psk@frameheight\p@
\edef\pst@coor{0 0 }%
\else
\pst@@getcoor{#1}%
\fi
\pst@newnode{#2}{14}{}{%
\pst@coor
/Y ED /X ED
/d \psk@dimen .5 sub CLW mul neg def
/r \psk@framewidth d add def
/l r neg def
/u \psk@frameheight d add def
/d u neg def
/NodePos { \tx@GetRnodePos } def}%
\addto@pscode{%
/x2 \psk@framewidth CLW \psk@dimen mul sub def
/y2 \psk@frameheight CLW \psk@dimen mul sub def
\pst@coor 2 copy
y2 sub /y1 ED
x2 sub /x1 ED
y2 add /y2 ED
x2 add /x2 ED
\psk@cornersize
1 index 0 eq { pop pop \tx@Rect } { \tx@OvalFrame } ifelse}%
\def\pst@linetype{2}%
\showpointsfalse
\end@ClosedObj
\ifnodealign\kern\psk@framewidth\p@\fi}%
\ignorespaces}
\def\psset@nodesepA#1{%
\pst@getlength{#1}\psk@nodesepA
\def\psk@nodeseptypeA{0 }}
\def\psset@nodesepB#1{%
\pst@getlength{#1}\psk@nodesepB
\def\psk@nodeseptypeB{0 }}
\def\psset@nodesep#1{%
\pst@getlength{#1}\psk@nodesepA
\let\psk@nodesepB\psk@nodesepA
\def\psk@nodeseptypeA{0 }%
\def\psk@nodeseptypeB{0 }}
\psset@nodesep{0pt}
\def\psset@XnodesepA#1{%
\pst@getlength{#1}\psk@nodesepA
\def\psk@nodeseptypeA{1 }}
\def\psset@XnodesepB#1{%
\pst@getlength{#1}\psk@nodesepB
\def\psk@nodeseptypeB{1 }}
\def\psset@Xnodesep#1{%
\pst@getlength{#1}\psk@nodesepA
\let\psk@nodesepB\psk@nodesepA
\def\psk@nodeseptypeA{1 }%
\def\psk@nodeseptypeB{1 }}
\def\psset@YnodesepA#1{%
\pst@getlength{#1}\psk@nodesepA
\def\psk@nodeseptypeA{2 }}
\def\psset@YnodesepB#1{%
\pst@getlength{#1}\psk@nodesepB
\def\psk@nodeseptypeB{2 }}
\def\psset@Ynodesep#1{%
\pst@getlength{#1}\psk@nodesepA
\let\psk@nodesepB\psk@nodesepA
\def\psk@nodeseptypeA{2 }%
\def\psk@nodeseptypeB{2 }}
\def\psset@armA#1{%
\pst@getlength{#1}\psk@armA
\def\psk@armtypeA{0 }}
\def\psset@armB#1{%
\pst@getlength{#1}\psk@armB
\def\psk@armtypeB{0 }}
\def\psset@arm#1{%
\pst@getlength{#1}\psk@armA
\let\psk@armB\psk@armA
\def\psk@armtypeA{0 }%
\def\psk@armtypeB{0 }}
\psset@arm{10pt}
\def\psset@XarmA#1{%
\pst@getlength{#1}\psk@armA
\def\psk@armtypeA{1 }}
\def\psset@XarmB#1{%
\pst@getlength{#1}\psk@armB
\def\psk@armtypeB{1 }}
\def\psset@Xarm#1{%
\pst@getlength{#1}\psk@armA
\let\psk@armB\psk@armA
\def\psk@armtypeA{1 }%
\def\psk@armtypeB{1 }}
\def\psset@YarmA#1{%
\pst@getlength{#1}\psk@armA
\def\psk@armtypeA{2 }}
\def\psset@YarmB#1{%
\pst@getlength{#1}\psk@armB
\def\psk@armtypeB{2 }}
\def\psset@Yarm#1{%
\pst@getlength{#1}\psk@armA
\let\psk@armB\psk@armA
\def\psk@armtypeA{2 }%
\def\psk@armtypeB{2 }}
\def\psset@offsetA#1{\pst@getlength{#1}\psk@offsetA}
\def\psset@offsetB#1{\pst@getlength{#1}\psk@offsetB}
\def\psset@offset#1{\psset@offsetA{#1}\let\psk@offsetB\psk@offsetA}
\psset@offset{0pt}
\def\psset@angleA#1{\pst@getangle{#1}\psk@angleA}
\def\psset@angleB#1{\pst@getangle{#1}\psk@angleB}%
\def\psset@angle#1{%
\pst@getangle{#1}\psk@angleA
\let\psk@angleB\psk@angleA}
\psset@angle{0}
\def\psset@arcangleA#1{\pst@getangle{#1}\psk@arcangleA}
\def\psset@arcangleB#1{\pst@getangle{#1}\psk@arcangleB}%
\def\psset@arcangle#1{%
\pst@getangle{#1}\psk@arcangleA
\let\psk@arcangleB\psk@arcangleA}
\psset@arcangle{8}
\def\psset@ncurvA#1{\pst@checknum{#1}\psk@ncurvA}
\def\psset@ncurvB#1{\pst@checknum{#1}\psk@ncurvB}%
\def\psset@ncurv#1{\psset@ncurvA{#1}\let\psk@ncurvB\psk@ncurvA}
\psset@ncurv{.67}
\def\tx@GetCenter{GetCenter }
\def\tx@XYPos{XYPos }
\def\tx@GetEdge{GetEdge }
\def\tx@AddOffset{AddOffset }
\def\tx@GetEdgeA{GetEdgeA }
\def\tx@GetEdgeB{GetEdgeB }
\def\tx@GetArmA{GetArmA }
\def\tx@GetArmB{GetArmB }
\def\check@arrow#1#2{%
\check@@arrow#2-\@nil
\if@pst
\addto@par{arrows=#2}%
\def\next{#1}%
\else
\def\next{#1{#2}}%
\fi
\next}
\def\check@@arrow#1-#2\@nil{%
\ifx\@nil#2\@nil\@pstfalse\else\@psttrue\fi}
\def\tx@InitNC{InitNC }
\def\nc@object#1#2#3#4#5{%
\csname begin@#1Obj\endcsname
\showpointsfalse
\pst@getnode{#2}\pst@tempa
\pst@getnode{#3}\pst@tempb
\gdef\npos@default{#4 }%
\addto@pscode{%
/NCLW CLW def
\pst@nodedict
\psk@offsetA
\psk@offsetB neg
\psk@nodesepA
\psk@nodesepB
\psk@nodeseptypeA
\psk@nodeseptypeB
\pst@tempa
\pst@tempb
\tx@InitNC { #5 } if
end}%
\def\use@pscode{%
\pst@Verb{gsave \tx@STV newpath \pst@code\space grestore}%
\gdef\pst@code{}}%
\csname end@#1Obj\endcsname
\pst@shortput}
\def\npos@default{.5 }
\def\pc@object#1{%
\@ifnextchar({\pc@@object#1}{\pst@getarrows{\pc@@object#1}}}
\def\pc@@object#1(#2)(#3){%
\pnode(#2){@@A}\pnode(#3){@@B}%
#1{@@A}{@@B}}
\def\tx@LPutLine{LPutLine }
\def\tx@LPutLines{LPutLines }
\def\tx@BezierMidpoint{BezierMidpoint }
\def\tx@HPosBegin{HPosBegin }
\def\tx@HPosEnd{HPosEnd }
\def\tx@HPutLine{HPutLine }
\def\tx@HPutLines{HPutLines }
\def\tx@VPosBegin{VPosBegin }
\def\tx@VPosEnd{VPosEnd }
\def\tx@VPutLine{VPutLine }
\def\tx@VPutLines{VPutLines }
\def\tx@HPutCurve{HPutCurve }
\def\tx@NCCoor{NCCoor }
\def\tx@NCLine{NCLine }
\def\ncline{\pst@object{ncline}}
\def\ncline@i{\check@arrow{\ncline@ii}}
\def\ncline@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{\tx@NCLine}}
\def\pcline{\pst@object{pcline}}
\def\pcline@i{\pc@object\ncline@ii}
\def\ncLine{\pst@object{ncLine}}
\def\ncLine@i{\check@arrow{\ncLine@ii}}
\def\ncLine@ii#1#2{\nc@object{Open}{#1}{#2}{.5}%
{\tx@NCLine /LPutPos { xB xA yB yA \tx@LPutLine } def}}
\def\tx@NCLines{NCLines }
\def\nclines{\pst@object{nclines}}
\def\nclines@i{\check@arrow\nclines@ii}
\def\nclines@ii#1#2{%
\begingroup
\use@par
\def\pst@aftercoors{\nclines@iii{#1}{#2}}%
\def\pst@coors{}%
\pst@@getcoors}
\def\nclines@iii#1#2{%
\nc@object{Open}{#1}{#2}{.5}{%
tx@Dict begin \psline@iii pop end
mark \pst@coors \tx@NCLines}%
\endgroup
\ignorespaces}
\def\tx@NCCurve{NCCurve }
\def\nccurve{\pst@object{nccurve}}
\def\nccurve@i{\check@arrow{\nccurve@ii}}
\def\nccurve@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
/AngleA \psk@angleA\space def /AngleB \psk@angleB\space def
\psk@ncurvB\space \psk@ncurvA\space
\tx@NCCurve}}
\def\pccurve{\pst@object{pccurve}}
\def\pccurve@i{\pc@object\nccurve@ii}
\def\ncarc{\pst@object{ncarc}}
\def\ncarc@i{\check@arrow{\ncarc@ii}}
\def\ncarc@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
yB yA sub xB xA sub \tx@Atan dup
\psk@arcangleA\space add /AngleA ED
\psk@arcangleB\space sub 180 add /AngleB ED
\psk@ncurvB\space \psk@ncurvA\space
\tx@NCCurve}}
\def\pcarc{\pst@object{pcarc}}
\def\pcarc@i{\pc@object\ncarc@ii}
\def\tx@NCAngles{NCAngles }
\def\ncangles{\pst@object{ncangles}}
\def\ncangles@i{\check@arrow{\ncangles@ii}}
\def\ncangles@ii#1#2{%
\nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \tx@NCAngles}}
\def\ncangles@iii{%
tx@Dict begin \psline@iii pop end
/AngleA \psk@angleA def
/AngleB \psk@angleB def
/ArmA \psk@armA def
/ArmB \psk@armB def
/ArmTypeA \psk@armtypeA def
/ArmTypeB \psk@armtypeB def }
\def\pcangles{\pst@object{pcangles}}
\def\pcangles@i{\pc@object\ncangles@ii}
\def\tx@NCAngle{NCAngle }
\def\ncangle{\pst@object{ncangle}}
\def\ncangle@i{\check@arrow{\ncangle@ii}}
\def\ncangle@ii#1#2{%
\nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \tx@NCAngle}}
\def\pcangle{\pst@object{pcangle}}
\def\pcangle@i{\pc@object\ncangle@ii}
\def\tx@NCBar{NCBar }
\def\ncbar{\pst@object{ncbar}}
\def\ncbar@i{\check@arrow{\ncbar@ii}}
\def\ncbar@ii#1#2{\nc@object{Open}{#1}{#2}{1.5}{%
\ncangles@iii /AngleB \psk@angleA def \tx@NCBar}}
\def\pcbar{\pst@object{pcbar}}
\def\pcbar@i{\pc@object\ncbar@ii}
\def\tx@NCDiag{NCDiag }
\def\ncdiag{\pst@object{ncdiag}}
\def\ncdiag@i{\check@arrow{\ncdiag@ii}}
\def\ncdiag@ii#1#2{%
\nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \tx@NCDiag}}
\def\pcdiag{\pst@object{pcdiag}}
\def\pcdiag@i{\pc@object\ncdiag@ii}
\def\tx@NCDiagg{NCDiagg }
\def\ncdiagg{\pst@object{ncdiagg}}
\def\ncdiagg@i{\check@arrow{\ncdiagg@ii}}
\def\ncdiagg@ii#1#2{%
\nc@object{Open}{#1}{#2}{.5}{\ncangles@iii \tx@NCDiagg}}
\def\pcdiagg{\pst@object{pcdiagg}}
\def\pcdiagg@i{\pc@object\ncdiagg@ii}
\def\tx@NCLoop{NCLoop }
\def\psset@loopsize#1{\pst@getlength{#1}\psk@loopsize}
\psset@loopsize{1cm}
\def\ncloop{\pst@object{ncloop}}
\def\ncloop@i{\check@arrow{\ncloop@ii}}
\def\ncloop@ii#1#2{%
\nc@object{Open}{#1}{#2}{2.5}%
{\ncangles@iii /loopsize \psk@loopsize def \tx@NCLoop}}
\def\pcloop{\pst@object{pcloop}}
\def\pcloop@i{\pc@object\ncloop@ii}
\def\tx@NCCircle{NCCircle }
\def\nccircle{\pst@object{nccircle}}
\def\nccircle@i{\check@arrow{\nccircle@ii}}
\def\nccircle@ii#1#2{%
\pssetlength\pst@dima{#2}%
\nc@object{Open}{#1}{#1}{.5}{%
/AngleA \psk@angleA def
/r \pst@number\pst@dima def
\tx@NCCircle \psarc@v end}}
\def\tx@NCBox{NCBox }
\def\ncbox{\pst@object{ncbox}}
\def\ncbox@i{\check@arrow{\ncbox@ii}}
\def\ncbox@ii#1#2{%
\def\pst@linetype{2}%
\nc@object{Closed}{#1}{#2}{.5}{%
tx@Dict begin \psline@iii pop end
\psk@boxheight \psk@boxdepth
\tx@NCBox}}
\def\pcbox{\pst@object{pcbox}}
\def\pcbox@i{\pc@object\ncbox@ii}
\def\tx@NCArcBox{NCArcBox }
\def\psset@boxheight#1{\pst@getlength{#1}\psk@boxheight}
\def\psset@boxdepth#1{\pst@getlength{#1}\psk@boxdepth}
\def\psset@boxsize#1{%
\psset@boxheight{#1}%
\let\psk@boxdepth\psk@boxheight}
\psset@boxsize{.4cm}
\def\ncarcbox{\pst@object{ncarcbox}}
\def\ncarcbox@i{\check@arrow{\ncarcbox@ii}}
\def\ncarcbox@ii#1#2{%
\def\pst@linetype{1}%
\nc@object{Closed}{#1}{#2}{.5}{%
\psk@arcangleA \psk@boxheight \psk@boxdepth \pst@number\pslinearc
\tx@NCArcBox}}
\def\pcarcbox{\pst@object{pcarcbox}}
\def\pcarcbox@i{\pc@object\ncarcbox@ii}
\def\tx@Tfan{Tfan }
% Changed according pst-beta.bug December 3, 1993
% nrot=:<angle> does not work when : is active.
\begingroup
\catcode`\:=13
\gdef\pst@activerot{\def:{\string:}}
\endgroup
\def\psset@nrot#1{%
\begingroup
\pst@activerot
\pst@expandafter{\@ifnextchar:{\psset@@nrot}{\psset@@rot}}{#1}\@nil
\global\let\pst@tempg\psk@rot
\endgroup
\let\psk@nrot\pst@tempg}
\def\psset@@nrot:#1\@nil{%
\psset@@rot#1\@nil
\edef\psk@rot{NAngle \ifx\psk@rot\@empty\else\psk@rot add \fi}}
\psset@nrot{0}
\def\tx@LPutCoor{LPutCoor }
\def\tx@LPut{LPut }
\def\psset@npos#1{%
\def\pst@tempa{#1}%
\ifx\pst@tempa\@empty
\def\psk@npos{\npos@default}%
\else
\pst@checknum{#1}\psk@npos
\fi}
\psset@npos{}
\def\ncput{\pst@object{ncput}}
\def\ncput@i{\pst@killglue\pst@makebox{\ncput@ii}}
\def\ncput@ii{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\pst@makesmall\pst@hbox
\pst@rotate\psk@nrot\pst@hbox
\ncput@iii
\endgroup
\pst@shortput}
\def\ncput@iii{%
\leavevmode
\hbox{%
\pst@Verb{%
\pst@nodedict
/t \psk@npos def
\tx@LPut
end
\tx@PutBegin}%
\box\pst@hbox
\pst@Verb{\tx@PutEnd}}}
\def\naput{\pst@object{naput}}
\def\naput@i{\pst@killglue\pst@makebox{\naput@ii{NAngle 90 add}}}
\def\naput@ii#1{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\def\psk@refangle{#1 }%
\let\psk@rot\psk@nrot
\uput@vii
{exch pop add a \tx@PtoC h1 add exch w1 add exch }%
{tx@Dict /NCLW known { NCLW add } if }%
\ncput@iii
\endgroup
\pst@shortput}
\def\nbput{\pst@object{nbput}}
\def\nbput@i{\pst@killglue\pst@makebox{\naput@ii{NAngle 90 sub}}}
\def\psset@tpos#1{%
\pst@checknum{#1}\psk@tpos
\ifdim\psk@tpos \p@<\z@
\def\psk@tpos{.5}%
% DG/SR modification begin - Sep. 23, 1998 - Patch 7
%\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@epha
\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@ehpa
% DG/SR modification end
\else
\ifdim\psk@tpos \p@>\p@
\def\psk@tpos{.5}%
% DG/SR modification begin - Sep. 23, 1998 - Patch 7
%\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@epha
\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@ehpa
% DG/SR modification end
\fi
\fi}
\psset@tpos{.5}
\def\tvput{\pst@object{tvput}}
\def\tvput@i{\pst@makebox{\psput@tput{H}{1}}}
\def\tlput{\pst@object{tlput}}
\def\tlput@i{\pst@makebox{\psput@tput{H}{true}}}
\def\trput{\pst@object{trput}}
\def\trput@i{\pst@makebox{\psput@tput{H}{false}}}
\def\thput{\pst@object{thput}}
\def\thput@i{\pst@makebox{\psput@tput{V}{1}}}
\def\taput{\pst@object{taput}}
\def\taput@i{\pst@makebox{\psput@tput{V}{true}}}
\def\tbput{\pst@object{tbput}}
\def\tbput@i{\pst@makebox{\psput@tput{V}{false}}}
\def\tx@HPutAdjust{HPutAdjust }
\def\tx@VPutAdjust{VPutAdjust }
\def\psput@tput#1#2{%
\begingroup
\use@par
\pst@tputmakesmall
\leavevmode
\hbox{%
\pst@Verb{%
\pst@nodedict
/t \psk@tpos \pst@tposflip def
tx@NodeDict /HPutPos known
{ #1PutPos }
{ CP /Y ED /X ED /NAngle 0 def /NCLW 0 def }
ifelse
/Sin NAngle sin def
/Cos NAngle cos def
/s \pst@number\pslabelsep NCLW add def
/l \pst@number\pst@dima def
/r \pst@number\pst@dimb def
/h \pst@number\pst@dimc def
/d \pst@number\pst@dimd def
% DG/SR modification begin - Sep. 26, 1997 - Patch 4
%\ifnum1=0#2\else
\ifnum1=0#2 \else
% DG/SR modification end
/flag #2 def
\csname tx@#1PutAdjust\endcsname
\fi
\tx@LPutCoor
end
\tx@PutBegin}%
\box\pst@hbox
\pst@Verb{\tx@PutEnd}}%
\endgroup
\pst@shortput}
\def\pst@tposflip{}
\def\pst@tputmakesmall{%
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\pst@dimg=\psk@href\pst@dimg
\pst@dimb\pst@dima
\advance\pst@dima\pst@dimg % leftsize
\advance\pst@dimb-\pst@dimg % rightsize
\pst@dimd=\psk@vref\relax
\pst@dimc=\ht\pst@hbox
\advance\pst@dimc-\pst@dimd % height
\advance\pst@dimd\dp\pst@hbox % depth
\setbox\pst@hbox=\hbox to\z@{%
\kern-\pst@dima\vbox to\z@{\vss\box\pst@hbox\vskip-\pst@dimd}\hss}}
\def\MakeShortNab#1#2{%
  \def\pst@shortput@nab{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \let\pst@tempg\naput
    \else
      \ifx#2\next
        \let\pst@tempg\nbput
      \else
        \ifx\@sptoken\next
          \let\pst@tempg\pst@shortput
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortNab{^}{_}
\def\MakeShortTablr#1#2#3#4{%
  \def\pst@shortput@tablr{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \let\pst@tempg\taput
    \else
      \ifx#2\next
        \let\pst@tempg\tbput
      \else
        \ifx#3\next
          \let\pst@tempg\tlput
        \else
          \ifx#4\next
            \let\pst@tempg\trput
          \else
            \ifx\@sptoken\next
              \let\pst@tempg\pst@shortput
            \fi
          \fi
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortTablr{^}{_}{<}{>}
\def\MakeShortTab#1#2{%
  \def\pst@shortput@tab{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \def\pst@tempg{%
        \@nameuse{%
          t\ifodd\psk@treemode\ifpstreeflip b\else a\fi
          \else\ifpstreeflip r\else l\fi\fi put}}%
    \else
      \ifx#2\next
        \def\pst@tempg{%
          \@nameuse{%
            t\ifodd\psk@treemode\ifpstreeflip a\else b\fi
            \else\ifpstreeflip l\else r\fi\fi put}}%
      \else
        \ifx\@sptoken\next
          \let\pst@tempg\pst@shortput
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortTab{^}{_}
\def\psset@shortput#1{%
\def\pst@tempg{#1}%
\ifx\pst@tempg\@none
\let\pst@shortput\ignorespaces
\else
\@ifundefined{pst@shortput@#1}%
{\@pstrickserr{Bad short put: `#1'}\@ehpa}%
{\edef\pst@shortput{\noexpand\afterassignment\expandafter\noexpand
\csname pst@shortput@#1\endcsname\noexpand\let\noexpand\next}}%
\fi}
\psset@shortput{none}
\def\lput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\lput@i}{\lput@ii}}}
\def\lput@i[#1]{\addto@par{ref=#1}\lput@ii}
\def\lput@ii{\@ifnextchar({\lput@iv}{\lput@iii}}
\def\lput@iii#1{\addto@par{nrot=#1}\@ifnextchar({\lput@iv}{\ncput@i}}
\def\lput@iv(#1){\addto@par{npos=#1}\ncput@i}
\def\mput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\mput@i}{\ncput@i}}}
\def\mput@i[#1]{\addto@par{ref=#1}\ncput@i}
\def\Lput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Lput@ii}{\Lput@i}}}
\def\Lput@i#1{\addto@par{labelsep=#1}\Lput@ii}
\def\Lput@ii[#1]{\addto@par{ref={#1}}\@ifnextchar({\Lput@iv}{\Lput@iii}}
\def\Lput@iii#1{\addto@par{nrot={#1}}\@ifnextchar({\Lput@iv}{\Lput@v}}
\def\Lput@iv(#1){\addto@par{npos=#1}\Lput@v}
\def\Lput@v{\pst@killglue\pst@makebox{\Lput@vi}}
\def\Lput@vi{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\Rput@vi
\pst@makesmall\pst@hbox
\pst@rotate\psk@nrot\pst@hbox
\ncput@iii
\endgroup
\pst@shortput}
\def\Mput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Mput@ii}{\Mput@i}}}
\def\Mput@i#1{\addto@par{labelsep=#1}\Mput@ii}
\def\Mput@ii[#1]{\addto@par{ref={#1}}\Lput@v}
\def\aput@#1{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\aput@i#1}{\aput@ii#1}}}
\def\aput@i#1[#2]{\addto@par{labelsep=#2}\aput@ii#1}
\def\aput@ii#1{\@ifnextchar({\aput@iv#1}{\aput@iii#1}}
\def\aput@iii#1#2{\addto@par{nrot=#2}\@ifnextchar({\aput@iv#1}{#1}}
\def\aput@iv#1(#2){\addto@par{npos=#2}#1}
\def\aput{\aput@\naput@i}
\def\bput{\aput@\nbput@i}
\def\Aput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Aput@i}{\naput@i}}}
\def\Aput@i[#1]{\addto@par{labelsep=#1}\naput@i}
\def\Bput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Bput@i}{\nbput@i}}}
\def\Bput@i[#1]{\addto@par{labelsep=#1}\nbput@i}
\def\node@coor#1;#2\@nil{%
\pst@getnode{#1}\pst@tempg
\edef\pst@coor{%
\pst@nodedict
tx@NodeDict \pst@tempg known
{ \pst@tempg load \tx@GetCenter }
{ 0 0 }
ifelse
end }}
\def\Node@coor[#1]#2;#3\@nil{%
\begingroup
\psset{#1}%
\@ifnextchar\bgroup{\Node@@@coor}{\Node@@coor}#2\@nil
\endgroup
\let\pst@coor\pst@tempg}
\def\Node@@coor#1\@nil{%
\pst@getnode{#1}\pst@tempg
\xdef\pst@tempg{%
\pst@nodedict
tx@NodeDict \pst@tempg known
{ \psk@nodesepA \psk@angleA
\pst@tempg load \psk@nodeseptypeA \tx@GetEdge
\psk@offsetA \psk@angleA \tx@AddOffset
\pst@tempg load \tx@GetCenter
3 -1 roll add 3 1 roll add exch }
{ CP }
ifelse
end }}%
\def\Node@@@coor#1{%
\pst@@getcoor{#1}%
\def\psk@angleA{%
\pst@tempg load \tx@GetCenter \pst@coor
3 -1 roll sub 3 1 roll sub neg \tx@Atan}%
\Node@@coor}
\def\nput{\pst@object{nput}}
\def\nput@i#1#2{\pst@killglue\pst@makebox{\nput@ii{#1}{#2}}}
\def\nput@ii#1#2{%
\begingroup
\use@par
\psset@refangle{#1}%
\let\psk@angleA\psk@refangle
\edef\psk@nodesepA{\pst@number\pslabelsep}%
\def\psk@nodeseptypeA{0 }%
\pslabelsep\z@
\uput@vi
\Node@@coor#2\@nil
\let\pst@coor\pst@tempg
\leavevmode
\psput@special\pst@hbox
\endgroup
\ignorespaces}
\newcount\psrow
\newcount\pscol
\newcount\psmatrixcnt
\newskip\psrowsep
\newskip\pscolsep
\def\psset@colsep#1{\pssetlength\pscolsep{#1}}
\def\psset@rowsep#1{\pssetlength\psrowsep{#1}}
\psset@colsep{1.5cm}
\psset@rowsep{1.5cm}
\newif\ifpsmatrix
% DG/SR modification begin - Nov. 27, 1998 - Patch 8
%\let\mscount\@multicnt
\ifx\mscount\@undefined\let\mscount\@multicnt\fi
% DG/SR modification end
\def\psmatrix{%
  \begingroup
{\ifnum0=`}\fi % Don't want to expand any &.
\@ifnextchar[{\psmatrix@i}{\ifnum0=`{\fi}{}\psmatrix@ii}}
\def\psmatrix@i[#1]{%
\ifnum0=`{\fi}{}%
\psset{#1}%
\psmatrix@ii}
\def\psmatrix@ii{%
\KillGlue
\edef\psm@beginmath{%
\ifmmode$\m@th\ifinner\textstyle\else\displaystyle\fi\fi}%
\edef\psm@endmath{\ifmmode$\fi}%
\let\\\psm@cr
\advance\psmatrixcnt 1
\def\psm@thenode{M-\the\psmatrixcnt-\the\psrow-\the\pscol}%
\tabskip\z@
\psrow1
\pscol\z@
\psset@shortput{tablr}%
\leavevmode
\vbox\bgroup\halign\bgroup&%
\begingroup
\global\advance\pscol 1
\csname psrowhook\romannumeral\psrow\endcsname
\csname pscolhook\romannumeral\pscol\endcsname
\psm@beginnode##\psm@endnode\endgroup
\cr}
\def\endpsmatrix{%
\crcr\egroup\unskip\egroup
\endgroup}
\def\psm@cr{{\ifnum0=`}\fi\@ifnextchar[{\psm@@cr}{\psm@@@cr{}}}
\def\psm@@cr[#1]{\psm@@@cr{\vskip#1\relax}}
\def\psm@@@cr#1{%
\ifnum0=`{\fi}{}\cr
\noalign{%
\global\advance\psrow 1
\global\pscol\z@
\vskip\psrowsep
#1}}
\def\psm@beginnode{%
\@ifnextchar\psm@endnode
{\let\psm@endnode@i\relax\setbox\pst@hbox=\hbox{}}%
{\pst@object{psm@beginnode}}}
\def\psm@beginnode@i{%
\setbox\pst@hbox=\hbox\bgroup
\psm@beginmath
\begingroup
\ignorespaces}
\def\psm@endnode@i{%
\unskip
\endgroup
\psm@endmath
\egroup
\use@par
\@psttrue}
\def\psm@endnode{%
\@pstfalse
\psm@endnode@i
\ifnum\pscol>1 \hskip\pscolsep \fi
\psk@mnodesize
\hfil
\nodealigntrue
\if@pst
\csname mnode@\psk@mnode\endcsname
\else
\csname mnode@\psk@emnode\endcsname
\fi
\psk@mcol
\psk@@mnodesize}
\def\psspan#1{\mscount#1\relax\loop\ifnum\mscount>\@ne \sp@n\repeat}
\def\psset@name#1{\pst@getnode{#1}\psk@name}
\let\psk@name\relax
\def\psset@mcol#1{%
\ifx r#1\relax
\let\psk@mcol\relax
\else
\ifx l#1\relax
\let\psk@mcol\hfill
\else
\let\psk@mcol\hfil
\fi
\fi}
\psset@mcol{c}
\def\psset@mnodesize#1{%
\pssetlength\pst@dimg{#1}%
\ifdim\pst@dimg<\z@
\let\psk@mnodesize\relax
\let\psk@@mnodesize\relax
\else
\edef\psk@mnodesize{\noexpand\hbox to\number\pst@dimg sp\noexpand\bgroup}%
\let\psk@@mnodesize\egroup
\fi}
\psset@mnodesize{-1pt}
\def\mnode@R{\rnode@iii\Rnode@ii{\psm@thenode}}
\def\mnode@r{\rnode@iii\rnode@iv{\psm@thenode}}
\def\mnode@oval{\ovalnode@ii{\psm@thenode}}
\def\mnode@tri{\trinode@ii{\psm@thenode}}
\def\mnode@dia{\dianode@ii{\psm@thenode}}
\def\mnode@C{{\nodealigntrue\cnode@ii(\z@,\z@){\psk@radius}{\psm@thenode}}}
\def\mnode@f{{\nodealigntrue\fnode@ii(\z@,\z@){\psm@thenode}}}
\def\mnode@circle{\circlenode@ii{\psm@thenode}}
\def\mnode@p{\pnode(\z@,\z@){\psm@thenode}}
% DG/SR modification begin - Jul. 22, 1997 - Patch 1
\def\mnode@dot{\dotnode@ii(\z@,\z@){\psm@thenode}}
% DG/SR modification end
\def\mnode@none{\box\pst@hbox}
\def\psset@mnode#1{%
\@ifundefined{mnode@#1}%
{\@pstrickserr{\string\psmatrix\space node `#1' not defined.}\@ehpa}%
{\edef\psk@mnode{#1}}}
\def\psset@emnode#1{%
\@ifundefined{mnode@#1}%
{\@pstrickserr{\string\psmatrix\space node `#1' not defined.}\@ehpa}%
{\edef\psk@emnode{#1}}}
\psset@mnode{R}
\psset@emnode{none}
%%%% FROM pst-coil.tex
\def\nccoil{\pst@object{nccoil}}
\def\nccoil@i{\check@arrow{\nccoil@ii}}
\def\nccoil@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
\tx@NCCoor
tx@Dict begin
% DG/SR modification begin - Mar. 19, 1998 - Patch 5
4 2 roll
% DG/SR modification end
\psk@coilwidth \pscoilheight
\psk@coilarmA \psk@coilarmB
\psk@coilaspect \psk@coilinc
\pst@coildict \tx@Coil end
end}}
\def\nczigzag{\pst@object{nczigzag}}
\def\nczigzag@i{\check@arrow{\nczigzag@ii}}
\def\nczigzag@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
\tx@NCCoor
tx@Dict begin
% DG/SR modification begin - Mar. 19, 1998 - Patch 5
4 2 roll
% DG/SR modification end
\pscoilheight
\psk@coilwidth
\psk@coilarmA
\psk@coilarmB
\pst@coildict \tx@ZigZag end
\psline@iii
\tx@Line
end}}
\catcode`\@=\TheAtCode\relax
\endinput
%%
%% END pst-node.tex


==> texmf/tex/latex/pstricks/pst-plot.tex <==
%% BEGIN pst-plot.tex
%%
%% Plots and axes with PSTricks 97.
%% See the PSTricks User's Guide for documentation.
%%
\def\fileversion{97 patch 1}
\def\filedate{1997/04/28}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\message{ v\fileversion, \filedate}

\csname PSTplotLoaded\endcsname
\let\PSTplotLoaded\endinput

\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }
  \expandafter\next
\fi

\ifx\MultidoLoaded\endinput\else
  \def\next{\input multido.tex }
  \expandafter\next
\fi

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

% Using lists of data is optimized for \dataplot and \fileplot
% Here is the tricky part. As each line is read from file,
% we want to ignore trailing delimiters, and convert arbitrary
% strings of non-trailing delimiters to _D_.
% We end up with
%   D x1 D y1 D x2 D y2 ... D xn D yn
%
\begingroup
\catcode`\{=13
\catcode`\}=13
\catcode`\(=13
\catcode`\)=13
\catcode`\,=13
\catcode`\!=1
\catcode`\*=2
\catcode`\ =13
\catcode`\_=13
\catcode`\^^M=13
\gdef\pst@datadelimiters!% Begin def
\catcode`\{=13%
\catcode`\}=13%
\catcode`\(=13%
\catcode`\)=13%
\catcode`\,=13%
\catcode`\ =13%
\catcode`\^^M=13%
\def,##1!%
\ifcat\noexpand,\noexpand##1%
\expandafter##1%
\else\space%
D\space##1%
\fi*%
\let(,\let),\let{,\let},\let ,\let^^M,\let_\@empty*% End def
\endgroup
\begingroup
\catcode`\,=13
\catcode`\_=13
\gdef\savedata@#1[#2]{%
  \xdef\pst@tempg{#2_}%
  \endgroup
  \let#1\pst@tempg
  \global\let\pst@tempg\relax
  \ignorespaces}
\gdef\readdata@{%
  \read1 to \pst@tempa
  \expandafter\readdata@@\pst@tempa_\@nil
  \ifeof1\else\expandafter\readdata@\fi}
\gdef\pst@@readfile#1#2\@nil{\addto@pscode{,#1#2}}%
\gdef\readdata@@#1#2\@nil{\xdef\pst@tempg{\pst@tempg,#1#2}}%
\endgroup

\def\readdata#1#2{%
  \openin1=#2
  \begingroup
  \def\pst@tempg{}%
  \ifeof1
    \@pstrickserr{Data file `#2' not found.}\@ehpa
  \else
    \pst@datadelimiters
    \catcode`\[=1
    \catcode`\]=2
    \readdata@%
  \fi
  \endgroup
  \let#1\pst@tempg
  \global\let\pst@tempg\relax
  \ignorespaces}

\def\pst@readfile#1{{\let\readdata@@\pst@@readfile\readdata\pst@tempg{#1}}}
\def\pst@altreadfile#1{%
  \openin1=#1
  \ifeof1
    \@pstrickserr{Data file `#1' not found.}\@ehpa
  \else
    \catcode`\{=10
    \catcode`\}=10
    \catcode`\(=10
    \catcode`\)=10
    \catcode`\,=10
    \catcode`\^^M=10
    \catcode`\[=1
    \catcode`\]=2
    \pst@@altreadfile
  \fi}
\def\pst@@altreadfile{%
  \read1 to \pst@tempg
  \expandafter\pst@@@altreadfile\pst@tempg\@empty\@nil
  \ifeof1\else\expandafter\pst@@@altreadfile\fi}
\def\pst@@@altreadfile#1#2\@nil{\addto@pscode{#1#2}}%

\def\savedata#1{\begingroup\pst@datadelimiters\savedata@{#1}}

\def\beginplot@line{\begin@OpenObj}
\def\endplot@line{\psline@ii}
\def\beginplot@polygon{\begin@ClosedObj}
\def\endplot@polygon{\pspolygon@ii}
\def\beginplot@curve{\begin@OpenObj}
\def\endplot@curve{\pscurve@ii}
\def\beginplot@ecurve{\begin@OpenObj}
\def\endplot@ecurve{\psecurve@ii}
\def\beginplot@ccurve{\begin@ClosedObj}
\def\endplot@ccurve{\psccurve@ii}
\def\beginplot@dots{\begin@SpecialObj}
\def\endplot@dots{\psdots@ii}
\def\beginplot@bezier{\begin@OpenObj}
\def\endplot@bezier{\psbezier@ii}
\def\beginplot@cbezier{\begin@ClosedObj}
\def\endplot@cbezier{\pscbezier@ii}

\def\psset@plotstyle#1{%
  \@ifundefined{beginplot@#1}%
    {\@pstrickserr{Plot style `#1' not defined}\@eha}%
    {\edef\psplotstyle{#1}}}
\psset@plotstyle{line}

\def\psset@plotpoints#1{%
  \pst@cntg=#1\relax
  \ifnum\pst@cntg<2
    \@pstrickserr{plotpoints parameter must be at least 2}\@ehpa
  \else
    \advance\pst@cntg-1
    \edef\psk@plotpoints{\the\pst@cntg\space}%
  \fi}
\psset@plotpoints{50}

% For quick plots, define:
%   \beginqp@<foo>   : What to do to first point (PS code only).
%   \doqp@<foo>      : What to do to subsequent points (PS code only).
%   \endqp@<foo>     : How to end plot.
%   \testqp@<foo>    : Set \@psttrue if OK to use quick plot.

\def\beginqp@line{\pst@oplineto}
\def\doqp@line{L }
\def\endqp@line{\end@OpenObj}%
\def\testqp@line{%
  \ifdim\pslinearc>\z@\else
    \ifshowpoints\else
      \ifx\psk@arrowA\@empty
        \ifx\psk@arrowB\@empty
          \@psttrue
        \fi
      \fi
    \fi
  \fi}

\def\beginqp@polygon{moveto }
\def\doqp@polygon{L }
\def\endqp@polygon{%
  \addto@pscode{closepath}%
  \end@ClosedObj}
\def\testqp@polygon{%
  \ifdim\pslinearc>\z@\else
    \ifshowpoints\else
      \@psttrue
    \fi
  \fi}

\def\beginqp@dots{%
  \psk@dotsize
  \@nameuse{psds@\psk@dotstyle}
% DG/SR modification begin - 1996/1997
%  Dot }
%\def\doqp@dots{Dot }
  /TheDot { gsave \psk@dotangle \psk@dotscale Dot grestore } def
  TheDot }
% DG/SR modification end
\def\doqp@dots{TheDot }
\def\endqp@dots{\end@SpecialObj}
\def\testqp@dots{\@psttrue}

\def\beginqp@bezier{/n 0 def \pst@oplineto}
\def\doqp@bezier{/n n 1 add def n 3 mod 0 eq { curveto } if }
\def\endqp@bezier{%
  \addto@pscode{n 3 mod { pop pop } repeat}
  \end@OpenObj}%
\def\testqp@bezier{%
  \ifshowpoints\else
    \ifx\psk@arrowA\@empty
      \ifx\psk@arrowB\@empty
        \@psttrue
      \fi
    \fi
  \fi}

\def\beginqp@cbezier{/n 0 def moveto }
\def\doqp@cbezier{\doqp@bezier}
\def\endqp@cbezier{%
  \addto@pscode{n 3 mod { pop pop } repeat closepath}
  \end@ClosedObj}%
\def\testqp@cbezier{\ifshowpoints\else\@psttrue\fi}

\def\dataplot{\def\pst@par{}\pst@object{dataplot}}
\def\dataplot@i#1{%
  \pst@killglue
  \begingroup
    \use@par
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst
      \dataplot@ii{\addto@pscode{#1}}%
    \else
      \listplot@ii{\addto@pscode{#1}}%
    \fi
  \endgroup
  \ignorespaces}
\def\dataplot@ii#1{%
  \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{%
      /Dx { \pst@number\psxunit mul /D { Dy } def } def
      /Dy { \pst@number\psyunit mul Do /D { Dx } def } def
      /D { /D { Dx } def } def
      /Do {
        \@nameuse{beginqp@\psplotstyle}%
        /Do { \@nameuse{doqp@\psplotstyle}} def
      } def}%
    #1%
    \addto@pscode{D}%
  \@nameuse{endqp@\psplotstyle}}

\def\fileplot{\def\pst@par{}\pst@object{fileplot}}
\def\fileplot@i#1{%
  \pst@killglue
  \begingroup
    \use@par
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst
      \dataplot@ii{\pst@readfile{#1}}%
    \else
      \listplot@ii{\pst@altreadfile{#1}}%
    \fi
  \endgroup
  \ignorespaces}

\pst@def{ScalePoints}<%
  /y ED /x ED
  counttomark dup dup cvi eq not { exch pop } if
  /m exch def /n m 2 div cvi def
  n { y mul m 1 roll x mul m 1 roll /m m 2 sub def } repeat>

\def\listplot{\def\pst@par{}\pst@object{listplot}}
\def\listplot@i#1{\listplot@ii{\addto@pscode{#1}}}
\def\listplot@ii#1{%
  \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{/D {} def mark}%
    #1%
    \addto@pscode{\pst@number\psxunit \pst@number\psyunit \tx@ScalePoints}%
  \@nameuse{endplot@\psplotstyle}}

% \psplot

\def\psplotinit#1{\xdef\psplot@init{#1 }}
\def\psplot@init{}

\def\psplot{\def\pst@par{}\pst@object{psplot}}
\def\psplot@i#1#2#3{%
  \pst@killglue
  \begingroup
    \use@par
    \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{%
      \psplot@init
      /x #1 def
      /x1 #2 def
      /dx x1 x sub \psk@plotpoints div def
      /xy {
        x \pst@number\psxunit mul
        #3 \pst@number\psyunit mul
      } def}%
    \gdef\psplot@init{}%
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst
      \psplot@ii
    \else
      \psplot@iii
    \fi
  \endgroup
  \ignorespaces}
\def\psplot@ii{%
    \addto@pscode{%
      xy \@nameuse{beginqp@\psplotstyle}
      \psk@plotpoints 1 sub {
        /x x dx add def
        xy \@nameuse{doqp@\psplotstyle}
      } repeat
      /x x1 def
      xy \@nameuse{doqp@\psplotstyle}}%
  \@nameuse{endqp@\psplotstyle}}
\def\psplot@iii{%
    \addto@pscode{%
      mark
      /n 2 def
      \psk@plotpoints {
        xy
        n 2 roll
        /n n 2 add def
        /x x dx add def
      } repeat
      /x x1 def
      xy
      n 2 roll}%
  \@nameuse{endplot@\psplotstyle}}

\def\parametricplot{\def\pst@par{}\pst@object{parametricplot}}
\def\parametricplot@i#1#2#3{%
  \pst@killglue
  \begingroup
    \use@par
    \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{%
      \psplot@init
      /t #1 def
      /t1 #2 def
      /dt t1 t sub \psk@plotpoints div def
      /xy {
        #3
        \pst@number\psyunit mul exch
        \pst@number\psxunit mul exch
      } def}%
    \gdef\psplot@init{}%
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst
      \parametricplot@ii
    \else
      \parametricplot@iii
    \fi
  \endgroup
  \ignorespaces}
\def\parametricplot@ii{%
    \addto@pscode{%
      xy \@nameuse{beginqp@\psplotstyle}
      \psk@plotpoints 1 sub {
        /t t dt add def
        xy \@nameuse{doqp@\psplotstyle}
      } repeat
      /t t1 def
      xy \@nameuse{doqp@\psplotstyle}}%
  \@nameuse{endqp@\psplotstyle}}
\def\parametricplot@iii{%
    \addto@pscode{%
      mark
      /n 2 def
      \psk@plotpoints {
        xy
        n 2 roll
        /n n 2 add def
        /t t dt add def
      } repeat
      /t t1 def
      xy
      n 2 roll}%
  \@nameuse{endplot@\psplotstyle}}

% These axes macros are complicated. Be careful.

% \pst@ticks{angle}{dx}{n}{int}
% int=1 if ticks appear on top of axes, 0 otherwise.
\def\pst@ticks#1#2#3#4{%
  \begin@SpecialObj
    \addto@pscode{%
      #1 rotate
      /n #3 def
      /dx #2 def
      n 0 lt { /dx dx neg def /n n neg def } if
      /y2 \psk@ticksize CLW 2 div add def
      /y1 y2 neg def
      \ifnum\psk@tickstyle=1
        \ifdim#4<\z@ /y2 \else /y1 \fi 0 def
      \else
        \ifnum\psk@tickstyle=-1
          \ifdim#4<\z@ /y1 \else /y2 \fi 0 def
        \fi
      \fi
      /x dx def
      n { x y1 moveto x y2 lineto stroke /x x dx add def } repeat}%
  \end@SpecialObj}


\def\psset@ticksize#1{\pst@getlength{#1}\psk@ticksize}
\psset@ticksize{3pt}

\def\psset@tickstyle#1{\pst@expandafter\psset@@tickstyle{#1}\@nil}
\def\psset@@tickstyle#1#2\@nil{%
  \ifx#1f\let\psk@tickstyle\z@\else
    \ifx#1t\let\psk@tickstyle\@ne\else
      \ifx#1b\let\psk@tickstyle\m@ne\else
        \@pstrickserr{Bad tick style: `#1#2'}\@ehpa
  \fi\fi\fi}
\psset@tickstyle{full}

\def\psset@ticks#1{\pst@expandafter\psset@@ticks{#1}\@nil\psk@ticks}
\def\psset@@ticks#1#2\@nil#3{%
  \ifx#1a\let#3\z@\else
    \ifx#1x\let#3\@ne\else
      \ifx#1y\let#3\tw@\else
        \ifx#1n\let#3\thr@@\else
          \@pstrickserr{Bad argument: `#1#2'}\@ehpa
  \fi\fi\fi\fi}
\psset@ticks{all}

\def\psset@labels#1{\pst@expandafter\psset@@ticks{#1}\@nil\psk@labels}
\psset@labels{all}

\def\psset@Ox#1{\edef\psk@Ox{#1}}
\psset@Ox{0}
\def\psset@Dx#1{\edef\psk@Dx{#1}}
\psset@Dx{1}
\def\psset@dx#1{%
  \pssetxlength\pst@dimg{#1}%
  \edef\psk@dx{\number\pst@dimg}}
\psset@dx{0}

\def\psset@Oy#1{\edef\psk@Oy{#1}}
\psset@Oy{0}
\def\psset@Dy#1{\edef\psk@Dy{#1}}
\psset@Dy{1}
\def\psset@dy#1{%
  \pssetylength\pst@dimg{#1}%
  \edef\psk@dy{\number\pst@dimg}}
\psset@dy{0}

\newif\ifshoworigin
\def\psset@showorigin#1{\@nameuse{showorigin#1}}
\psset@showorigin{true}


\def\psaxes{\def\pst@par{}\pst@object{psaxes}}
\def\psaxes@i{\pst@getarrows\psaxes@ii}
\def\psaxes@ii(#1){\@ifnextchar({\psaxes@iii(#1)}{\psaxes@iv(0,0)(0,0)(#1)}}
\def\psaxes@iii(#1)(#2){%
  \@ifnextchar(%
    {\psaxes@iv(#1)(#2)}%
    {\psaxes@iv(#1)(#1)(#2)}}
\def\psaxes@iv(#1,#2)(#3,#4)(#5,#6){%
  \setbox\pst@hbox=\hbox\bgroup
    \use@par
    \pssetxlength\pst@dimg{#1}% o-x
    \pssetylength\pst@dimh{#2}% o-y
    \pssetxlength\pst@dima{#3}% bl-x
    \pssetylength\pst@dimb{#4}% bl-y
    \pssetxlength\pst@dimc{#5}% ur-x
    \pssetylength\pst@dimd{#6}% ur-y
% Whole thing will be translated to origin:
    \advance\pst@dima-\pst@dimg % Dist. from bl-x to o-x
    \advance\pst@dimb-\pst@dimh % Dist. from bl-y to o-y
    \advance\pst@dimc-\pst@dimg % Dist. from ur-x to o-x
    \advance\pst@dimd-\pst@dimh % Dist. from ur-y to o-y
% Make lines/arrows or frame:
    \@nameuse{psxs@\psk@axesstyle}%
% "\pslabelsep" should be from the edge of the axis.
    \advance\pslabelsep.5\pslinewidth
% Now the ticks and labels. Start by checking for "\multido".
% !!Need to fix this so that does nothing when there are 0 ticks.!!
    \begingroup
      \ifdim\pst@dimb=\z@\else\showoriginfalse\fi
      \ifnum\psk@dx=\z@
        \pst@dimg=\psk@Dx\psxunit
        \edef\psk@dx{\number\pst@dimg}%
      \fi
      \ifnum\psk@ticks<\tw@
        \ifnum\psk@tickstyle>\z@\else
          \advance\pslabelsep\psk@ticksize\p@
        \fi
      \fi
      \pst@hlabels\pst@dimc\psk@arrowB
      \pst@hlabels\pst@dima\psk@arrowA
    \endgroup
    \begingroup
      \ifdim\pst@dima=\z@\else\showoriginfalse\fi
      \ifnum\psk@dy=\z@
         \pst@dimg=\psk@Dy\psyunit
         \edef\psk@dy{\number\pst@dimg}%
      \fi
      \ifodd\psk@ticks\else
        \ifnum\psk@tickstyle>\z@\else
          \advance\pslabelsep\psk@ticksize\p@
        \fi
      \fi
      \pst@vlabels\pst@dimd\psk@arrowB
      \pst@vlabels\pst@dimb\psk@arrowA
    \endgroup
% Now close "\pst@hbox" (which is 0-dimensional), and put it at the origin.
  \egroup
  \pssetxlength\pst@dimg{#1}%
  \pssetylength\pst@dimh{#2}%
  \leavevmode\psput@cartesian\pst@hbox
  \ignorespaces}

\def\psxs@axes{%
  \psxs@@axes\pst@dima\pst@dimc{}%
  \psxs@@axes\pst@dimb\pst@dimd{exch}}
\def\psxs@@axes#1#2#3{%
  \begin@SpecialObj
    \ifdim#1=\z@
      \def\psk@arrowA{C}%
    \else
      \ifdim#2=\z@
        \def\psk@arrowB{C}%
      \fi
    \fi
    \let\pst@linetype\pst@arrowtype
    \pst@addarrowdef
    \addto@pscode{%
      \pst@number#2 0 #3
      \pst@number#1 0 #3
      ArrowA
      CP 4 2 roll
      ArrowB
      L
      pop pop}%
    \pst@stroke
  \end@SpecialObj}

\def\psxs@frame{%
  \begin@SpecialObj
    \addto@pscode{%
      0 0 moveto \pst@number\pst@dimc 0 L
      0 \pst@number\pst@dimd 2 copy rlineto L closepath}%
    \pst@stroke
    \psk@fillstyle
  \end@SpecialObj
  \let\psk@arrowA\@empty
  \let\psk@arrowB\@empty}

\def\psset@axesstyle#1{%
  \@ifundefined{psxs@#1}%
    {\@pstrickserr{Axes style `#1' not defined}\@eha}%
    {\edef\psk@axesstyle{#1}}}
\psset@axesstyle{axes}

\def\psxs@none{\let\psk@arrowA\@empty\let\psk@arrowB\@empty}

% The origin is never the only label.
\def\pst@hlabels#1#2{%
  \ifdim#1=\z@\else
    \ifx#2\empty\else
      \advance#1\ifdim#1>\z@-\fi7\pslinewidth
    \fi
    \pst@cnta=#1\relax                % Distance (in sp) to end.
    \divide\pst@cnta\psk@dx\relax     % Number of ticks/labels
    \ifnum\pst@cnta=\z@\else
      \pst@dimb=\psk@dx sp            % Space between ticks.
      \ifnum\psk@ticks<\tw@
        \pst@ticks{0}{\pst@number\pst@dimb}{\the\pst@cnta}{\pst@dimd}%
      \fi
      \ifnum\psk@labels<\tw@ \pst@@hlabels\fi
      \showoriginfalse
    \fi
  \fi}

% Knows \pst@dimb and \pst@cnta
\def\pst@@hlabels{%
  \vbox to\z@{%
    \ifdim\pst@dimd>\z@\vskip\pslabelsep\else\vss\fi
    \ifnum\pst@cnta<\z@
      \pst@dimb=-\pst@dimb
    \fi
    \hbox to\z@{%
      \ifshoworigin\hbox to \z@{\hss\pshlabel{\psk@Ox}\hss}\fi
      \mmultido
        {\n=\psk@Ox+\psk@Dx}%
        {\pst@cnta}%
        {\hskip\pst@dimb\hbox to \z@{\hss\pshlabel{\n}\hss}}%
      \hss}%
    \ifdim\pst@dimd>\z@\vss\else\vskip\pslabelsep\fi}}%

\def\pshlabel#1{$#1$}

\def\pst@vlabels#1#2{%
  \ifdim#1=\z@\else
    \ifx#2\empty\else
      \advance#1\ifdim#1>\z@-\fi7\pslinewidth
    \fi
    \pst@cnta=#1\relax                % Distance (in sp) to end.
    \divide\pst@cnta\psk@dy\relax     % Number of ticks/labels
    \ifnum\pst@cnta=\z@\else
      \pst@dima=\psk@dy sp            % Space between ticks.
      \ifodd\psk@ticks\else
        \pst@ticks{90}{\pst@number\pst@dima}{\the\pst@cnta}{-\pst@dimc}%
      \fi
      \ifodd\psk@labels\else\pst@@vlabels\fi
      \showoriginfalse
    \fi
  \fi}

% Knows \pst@dima and \pst@cnta
\def\pst@@vlabels{%
  \vbox to\z@{%
    \ifnum\pst@cnta>\z@
      \pst@dima=-\pst@dima
    \fi
    \offinterlineskip
    \ifshoworigin
      \vbox to \z@{\vss\hbox to\z@{%
        \ifdim\pst@dimc>\z@\hss\else\hskip\pslabelsep\fi
        \psvlabel{\psk@Oy}%
        \ifdim\pst@dimc>\z@\hskip\pslabelsep\else\hss\fi}\vss}%
    \fi
    \mmultido
      {\n=\psk@Oy+\psk@Dy}%
      {\pst@cnta}%
      {\vbox to\pst@dima{\vss}\vbox to \z@{\vss\hbox to\z@{%
        \ifdim\pst@dimc>\z@\hss\else\hskip\pslabelsep\fi
        \psvlabel{\n}%
        \ifdim\pst@dimc>\z@\hskip\pslabelsep\else\hss\fi}\vss}}%
    \vss}}

\def\psvlabel#1{$#1$}

\catcode`\@=\TheAtCode\relax
\endinput
%%
%% END pst-plot.tex


==> texmf/tex/latex/pstricks/pst-poly.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% -*- Mode: Latex -*- %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pst-poly.tex --- Generation of polygons with PSTricks
%%
%% Author          : Denis GIROU (CNRS/IDRIS - France) <Denis.Girou@idris.fr>
%% Created the     : Mon Jan 16 19:01:42 1995
%% Last mod. by    : Denis GIROU (CNRS/IDRIS - France) <Denis.Girou@idris.fr>
%% Last mod. the   : Thu Jul  9 22:48:58 1998
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\fileversion{1.4}
\def\filedate{98/07/09}

%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.

\message{`PST-Polygon' v\fileversion, \filedate\space (Denis Girou)}

\csname PSTPolygonLoaded\endcsname
\let\PSTPolygonLoaded\endinput

% Require PSTricks, pst-node and multido packages
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
\ifx\MultidoLoaded\endinput\else\input multido.tex\fi

% DPC interface to the `keyval' package (until keyval based version of PSTricks)
\input pst-key.tex

\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax

% Definition of the parameters
% ----------------------------

% "pspicture" environment or not?
\newif\ifPst@PstPicture
\define@key{psset}{PstPicture}[true]{%
\@nameuse{Pst@PstPicture#1}}

% Rotation of the polygon (on 360 degrees)
\define@key{psset}{PolyRotation}{%
\edef\psk@PolyRotation{#1}}

% Number of sides of the polygon
\define@key{psset}{PolyNbSides}{%
\pst@cntg=#1\relax
\edef\psk@PolyNbSides{\the\pst@cntg}}

% Offset to obtain next node
\define@key{psset}{PolyOffset}{%
\pst@cntg=#1\relax
\edef\psk@PolyOffset{\the\pst@cntg}}

% Position of the intermediate point
\newdimen\psl@PolyIntermediatePoint
\define@key{psset}{PolyIntermediatePoint}{%
\edef\psk@PolyIntermediatePoint{#1}}

% Name of the polygon
\define@key{psset}{PolyName}{%
\edef\ps@PolyName{#1}}

% Nodes joined by lines or curves?
\newif\ifPst@PolyCurves
\define@key{psset}{PolyCurves}[true]{%
\@nameuse{Pst@PolyCurves#1}}

% Polygon or epicycloid?
\newif\ifPst@PolyEpicycloid
\define@key{psset}{PolyEpicycloid}[true]{%
\@nameuse{Pst@PolyEpicycloid#1}}

% Default values
% --------------
% 0 degree rotation, 5 sides, no offset, no intermediate point
% (9999 i.e. not used), no name, points joined by lines, no epicycloid
\setkeys{psset}{%
PstPicture=true,PolyRotation=0,PolyNbSides=5,PolyOffset=1,
PolyIntermediatePoint=,PolyName=,PolyCurves=false,PolyEpicycloid=false}

% The macro \PstPolygon for generic polygons
% ------------------------------------------

\def\PstPolygon{%
\pst@ifstar{\@ifnextchar[\@PstPolygon{\@PstPolygon[]}}}
\def\@PstPolygon[#1]{{%
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
%
% Validation of the parameters
\ifnum\psk@PolyNbSides<3
{\@pstrickserr{PolyNbSides must be greater than
   2 (and not `\psk@PolyNbSides')}\@eha}%
\fi
\ifnum\psk@PolyNbSides>200
{\@pstrickserr{PolyNbSides must be less than
   201 (and not `\psk@PolyNbSides')}\@eha}%
\fi
\ifnum\psk@PolyOffset<1
{\@pstrickserr{PolyOffset must be greater than
   0 (and not `\psk@PolyOffset')}\@eha}%
\fi
%
% Now the "real" code
\ifodd\psk@PolyOffset
  \def\Pst@PolyDecimal{.5}%
\else
  \def\Pst@PolyDecimal{}%
\fi
%
\SpecialCoor                    % To be able to use polar coordinates
\ifPst@PstPicture\pspicture(-1,-1)(1,1)\fi % "pspicture" environment
\rput{\psk@PolyRotation}(0,0){%   Rotation if needed
  \degrees[\psk@PolyNbSides]
  % We must recompute it here if unit has change after affectation
  % (for instance \psset{PolyIntermediatePoint=0.38}\PstPolygon{unit=2})
  \pssetlength{\psl@PolyIntermediatePoint}{\psk@PolyIntermediatePoint}
  % If we have to define names for nodes
  \ifx\ps@PolyName\@empty
  \else
    \pnode(0,0){\ps@PolyName 0}   % Center of the polygon
    \ifnum\psxunit=\psyunit
      \def\Pst@PolyNode{\pnode(1;\i)}%
    \else
      \def\Pst@PolyNode{%
        \pnode(!\i\space 360 \psk@PolyNbSides\space div mul cos %
                \i\space 360 \psk@PolyNbSides\space div mul sin)}%
    \fi
    \multido{\i=0+1}{\psk@PolyNbSides}{%
      \Pst@PolyNode{\ps@PolyName\the\multidocount}}
  \fi
  %
  \pscustom{%
    \ifPst@PolyEpicycloid       % Code for epicycloids
      \pst@cnta=\psk@PolyNbSides
      \divide\pst@cnta\tw@
      % We just draw lines between each point and it opposite, with possible gap
      \multido{\i=0+1}{\psk@PolyNbSides}{%
        \moveto(1;\i)
        \lineto(1;\the\pst@cnta)
        \advance\pst@cnta\psk@PolyOffset}
    \else                       % Code for polygons
      % Starting point
      \ifnum\psxunit=\psyunit
        \moveto(1,0)
      \else
        \moveto(! 1 0)
      \fi
      \ifx\psk@PolyIntermediatePoint\@empty % No intermediate points
        \ifnum\psxunit=\psyunit
          \def\Pst@PolyJunction{\lineto(1;\i)}%
        \else
          \def\Pst@PolyJunction{\lineto%
            (!\i\space 360 \psk@PolyNbSides\space div mul cos %
              \i\space 360 \psk@PolyNbSides\space div mul sin)}%
        \fi
        \multido{\i=\psk@PolyOffset+\psk@PolyOffset}{\psk@PolyNbSides}{%
          \Pst@PolyJunction}    % End \multido
      \else                     % Intermediate points
        \ifPst@PolyCurves       % Type of junction
          \let\Pst@PolyJunctionType\pscurve
        \else
          \let\Pst@PolyJunctionType\psline
        \fi
        \ifnum\psxunit=\psyunit
          \def\Pst@PolyJunction{\Pst@PolyJunctionType%
            (\psl@PolyIntermediatePoint;\the\pst@cnta\Pst@PolyDecimal)(1;\i)}%
        \else
          \def\Pst@PolyJunction{\Pst@PolyJunctionType%
            (!\psk@PolyIntermediatePoint\space %
                \the\pst@cnta\Pst@PolyDecimal\space 360 %
                  \psk@PolyNbSides\space div mul cos mul %
              \psk@PolyIntermediatePoint\space %
                \the\pst@cnta\Pst@PolyDecimal\space 360 %
                  \psk@PolyNbSides\space div mul sin mul)
            (!\i\space 360 \psk@PolyNbSides\space div mul cos %
              \i\space 360 \psk@PolyNbSides\space div mul sin)}%
        \fi
        \pst@cnta=\psk@PolyOffset
        \divide\pst@cnta\tw@
        \multido{\i=\psk@PolyOffset+\psk@PolyOffset}{\psk@PolyNbSides}{%
          \Pst@PolyJunction
          \advance\pst@cnta\psk@PolyOffset} % End \multido
      \fi                       % End \ifx\psk@PolyIntermediatePoint
    \fi}                        % End \ifPst@PolyEpicycloid and \pscustom
    \ifx\PstPolygonNode\@undefined
    \else
      \multido{\INode=0+\psk@PolyOffset}{\psk@PolyNbSides}{%
        \PstPolygonNode}        % Command to execute at each node
    \fi}                        % End \rput
\ifPst@PstPicture\endpspicture\fi}} % End of "pspicture" environment

% Pre-defined polygons
% --------------------

% Triangle (three sides)
\def\PstTriangle{%
\pst@ifstar{\@ifnextchar[\@PstTriangle{\@PstTriangle[]}}}
\def\@PstTriangle[#1]{{%
\setkeys{psset}{PolyNbSides=3,PolyRotation=90}% For triangle (360/3*(3/4))
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Square (four sides)
\def\PstSquare{%
\pst@ifstar{\@ifnextchar[\@PstSquare{\@PstSquare[]}}}
\def\@PstSquare[#1]{{%
\setkeys{psset}{PolyNbSides=4,PolyRotation=45}% For square (360/4/2)
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Pentagon (five sides)
\def\PstPentagon{%
\pst@ifstar{\@ifnextchar[\@PstPentagon{\@PstPentagon[]}}}
\def\@PstPentagon[#1]{{%
\setkeys{psset}{PolyNbSides=5,PolyRotation=18}% For pentagon (360/5/4)
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Hexagon (six sides)
\def\PstHexagon{%
\pst@ifstar{\@ifnextchar[\@PstHexagon{\@PstHexagon[]}}}
\def\@PstHexagon[#1]{{%
\setkeys{psset}{PolyNbSides=6}%   For hexagon
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Heptagon (seven sides)
\def\PstHeptagon{%
\pst@ifstar{\@ifnextchar[\@PstHeptagon{\@PstHeptagon[]}}}
\def\@PstHeptagon[#1]{{%
\setkeys{psset}{PolyNbSides=7,PolyRotation=38.57}% For heptagon (360/7*(3/4))
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Octogon (height sides)
\def\PstOctogon{%
\pst@ifstar{\@ifnextchar[\@PstOctogon{\@PstOctogon[]}}}
\def\@PstOctogon[#1]{{%
\setkeys{psset}{PolyNbSides=8,PolyRotation=22.5}% For octogon (360/8/2)
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Nonagon (nine sides)
\def\PstNonagon{%
\pst@ifstar{\@ifnextchar[\@PstNonagon{\@PstNonagon[]}}}
\def\@PstNonagon[#1]{{%
\setkeys{psset}{PolyNbSides=9,PolyRotation=10}% For nonagon (360/9/4)
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Decagon (ten sides)
\def\PstDecagon{%
\pst@ifstar{\@ifnextchar[\@PstDecagon{\@PstDecagon[]}}}
\def\@PstDecagon[#1]{{%
\setkeys{psset}{PolyNbSides=10}%  For decagon
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Dodecagon (twelve sides)
\def\PstDodecagon{%
\pst@ifstar{\@ifnextchar[\@PstDodecagon{\@PstDodecagon[]}}}
\def\@PstDodecagon[#1]{{%
\setkeys{psset}{PolyNbSides=12,PolyRotation=15}% For dodecagon (360/12/2)
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Star with five leaves, with internal lines
\def\PstStarFiveLines{%
\pst@ifstar{\@ifnextchar[\@PstStarFiveLines{\@PstStarFiveLines[]}}}
\def\@PstStarFiveLines[#1]{{%
\setkeys{psset}{PolyOffset=2,PolyRotation=18}% For star with internal lines
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

% Star with five leaves
\def\PstStarFive{%
\pst@ifstar{\@ifnextchar[\@PstStarFive{\@PstStarFive[]}}}
\def\@PstStarFive[#1]{{%
\setkeys{psset}{PolyIntermediatePoint=0.38,PolyRotation=18}%  For star
\setkeys{psset}{#1}%            % Affectation of local parameters
\if@star\solid@star\fi          % Stared version
\PstPolygon}}

\catcode`\@=\PstAtCode\relax
\endinput
%%
%% END: pst-poly.tex


==> texmf/tex/latex/pstricks/pst-slpe.tex <==
%%
%% This is file `pst-slpe.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-slpe.dtx  (with options: `texfile')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-slpe.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-slpe.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\def\pstslpefileversion{1.0}
\def\pstslpefiledate{98/09/15}
\message{ v\pstslpefileversion, \pstslpefiledate}
\csname PstSlopeLoaded\endcsname
\let\PstSlopeLoaded\endinput
\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }\expandafter\next
\fi
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
\pstheader{pst-slpe.pro}
\newrgbcolor{slopebegin}{0.9 1 0}
\def\psset@slopebegin#1{\pst@getcolor{#1}\psslopebegin}
\psset@slopebegin{slopebegin}

\newrgbcolor{slopeend}{0 0 1}
\def\psset@slopeend#1{\pst@getcolor{#1}\psslopeend}
\psset@slopeend{slopeend}

\def\psset@slopesteps#1{\pst@getint{#1}\psslopesteps}
\psset@slopesteps{100}

\def\psset@slopeangle#1{\pst@getangle{#1}\psx@slopeangle}
\psset@slopeangle{0}
\def\psset@slopecolors#1{\def\psx@slopecolors{#1}}
\def\psx@slopecolors{
0.0 1 0 0
0.4 0 1 0
0.8 0 0 1
1.0 1 0 1
4}
\def\psset@slopecenter#1{\def\psx@slopecenter{#1}}
\def\psx@slopecenter{0.5 0.5}
\def\psset@sloperadius#1{\pst@getlength{#1}\psx@sloperadius}
\def\psx@sloperadius{0}
\def\psfs@slopes{%
 \addto@pscode{
  \psx@slopecolors\space
  \psslopesteps
  \psx@slopeangle
  tx@PstSlopeDict begin SlopesFill end}}
\def\psfs@slope{%
 \addto@pscode{%
  gsave
    0 \pst@usecolor\psslopebegin currentrgbcolor
    1 \pst@usecolor\psslopeend currentrgbcolor
    2
  grestore
  \psslopesteps \psx@slopeangle tx@PstSlopeDict begin SlopesFill end}}
\def\psfs@ccslopes{%
 \addto@pscode{%
  \psx@slopecolors\space
  \psslopesteps \psx@slopecenter\space \psx@sloperadius\space
  tx@PstSlopeDict begin CcSlopesFill end}}
\def\psfs@ccslope{%
 \addto@pscode{%
  gsave 0 \pst@usecolor\psslopebegin currentrgbcolor
    1 \pst@usecolor\psslopeend currentrgbcolor
    2 grestore
  \psslopesteps \psx@slopecenter\space \psx@sloperadius\space
  tx@PstSlopeDict begin CcSlopesFill end}}
\def\psfs@radslopes{%
 \addto@pscode{%
  \psx@slopecolors\space
  \psslopesteps\psx@slopecenter\space\psx@sloperadius\space\psx@slopeangle
  tx@PstSlopeDict begin RadSlopesFill end}}
\def\psfs@radslope{%
 \addto@pscode{%
  gsave 0 \pst@usecolor\psslopebegin currentrgbcolor
    1 \pst@usecolor\psslopeend currentrgbcolor
    2 \pst@usecolor\psslopebegin currentrgbcolor
    3 \pst@usecolor\psslopeend currentrgbcolor
    4 \pst@usecolor\psslopebegin currentrgbcolor
    5 grestore
  \psslopesteps\psx@slopecenter\space\psx@sloperadius\space\psx@slopeangle
  tx@PstSlopeDict begin RadSlopesFill end}}

\catcode`\@=\TheAtCode\relax
\endinput
%%
%% End of file `pst-slpe.tex'.


==> texmf/tex/latex/pstricks/pst-text.tex <==
%% BEGIN pst-text.tex
%%
%% Placing text on a path with PSTricks 97.
%% See the PSTricks User's Guide for description.
%% See tp-test.tex for sample input and tp-test.ps for sample output.
%% This uses the header file `pst-text.pro'.
%%
\def\fileversion{97}
\def\filedate{1997/03/25}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\message{ v\fileversion, \filedate}

\csname PSTextPathLoaded\endcsname
\let\PSTextPathLoaded\endinput

\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex}\expandafter\next
\fi

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

\pstheader{pst-text.pro}

\def\pstextpath{\@ifnextchar[{\pstextpath@}{\pstextpath@[l]}}
\def\pstextpath@[#1]{%
  \@ifnextchar({\pstextpath@@[#1]}{\pstextpath@@[#1](0,\TPoffset)}}
\def\pstextpath@@[#1](#2)#3{\pst@makebox{\pstextpath@@@[#1](#2){#3}}}
\def\pstextpath@@@[#1](#2,#3)#4{%
  \pst@killglue
  \begingroup
    \ifx c#1\relax
      \def\pst@tempa{.5}%
    \else
      \ifx r#1\relax
        \def\pst@tempa{1}%
      \else
        \def\pst@tempa{0}%
      \fi
    \fi
    \def\use@pscode{%
      \pst@Verb{%
        /mtrxc CM def
        \tx@STV
        CP translate
        newpath
        \pst@code\space
        mtrxc setmatrix
        0 setgray}%
      \gdef\pst@code{}}%
    \def\psclip#1{\pst@misplaced\psclip}%
    \let\endpsclip\relax
    \def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
    \def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
    \def\PSTtoEPS@i##1##2{\pst@misplaced\PSTtoEPS}%
    \pssetlength\pst@dima{#2}%
    \pssetlength\pst@dimb{#3}%
    \setbox\pst@hbox\hbox{%
      \hbox to\z@{%
        \kern -\wd\pst@hbox
        % BoxWidth = CurrX - Hoffset.
        \pstVerb{tx@TextPathDict begin
          currentpoint pop /Hoffset exch def end}%
        \kern\pst@dima
        % XOffset = Voffset - Hoffset (extra horizontal skip)
        \pstVerb{tx@TextPathDict begin
          currentpoint pop /Voffset exch def end}%
        \hss
        \pstVerb{%
          /tx@TextPathSavedShow /show load def
          \pst@dict \tx@PathLength end
          dup 0 gt
          { tx@TextPathDict begin \pst@tempa\space InitTextPath end
            /show { tx@TextPathDict begin TextPathShow end } def
          }
          { pop }
          ifelse}}%
      \raise\pst@dimb\box\pst@hbox
      \pstVerb{%
        currentpoint newpath moveto
        /show /tx@TextPathSavedShow load def}}%
    \wd\pst@hbox=\z@ \dp\pst@hbox=\z@ \ht\pst@hbox=\z@
    \leavevmode
    \hbox{{#4}\box\pst@hbox}%
  \endgroup\ignorespaces}
\def\TPoffset{-.7ex}

\catcode`\@=\TheAtCode\relax

\endinput
%%
%% END pst-text.tex


==> texmf/tex/latex/pstricks/pst-tree.tex <==
%% BEGIN pst-tree.tex
%%
%% Trees with PSTricks 97.
%%
\def\fileversion{97 patch 3}
\def\filedate{1997/09/24}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\message{ v\fileversion, \filedate}

\csname PSTreeLoaded\endcsname
\let\PSTreeLoaded\endinput

\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi\relax

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11

\newbox\pstree@rootbox
\newbox\pstree@box
\def\pstree@succrow{%
\ifpstreeflip
\def\pssubtree@vertical{\pssubtree@vertical@vflip}%
\else
\def\pssubtree@vertical{\pssubtree@vertical@v}%
\fi
\def\pstree@node{\pstree@node@v}%
\def\pssubtree@horizontal{\pssubtree@horizontal@v}}%
\def\pssubtree@vertical@v{%
\vrule height \pst@dimc depth \pst@dimd width \z@
\ifnum\psnodecnt=\z@
\global\let\pstree@theleftprofile\pstree@leftprofile
\global\let\pstree@therightprofile\pstree@rightprofile
\else
\psk@thistreefit\pstree@therightprofile\pstree@leftprofile
\kern\the\pst@cnth sp
\pstree@zip\pstree@therightprofile
\pstree@rightprofile\pstree@therightprofile
\global\advance\pstree@cnt\pst@cnth
\pst@cnth=\pstree@cnt
\pstree@zip\pstree@leftprofile
\pstree@theleftprofile\pstree@theleftprofile
\fi
\box\pstree@box
\global\advance\psnodecnt 1\relax}%
\def\pssubtree@vertical@vflip{%
\vrule height \pst@dimc depth \pst@dimd width \z@
\ifnum\psnodecnt=\z@
\global\let\pstree@theleftprofile\pstree@leftprofile
\global\let\pstree@therightprofile\pstree@rightprofile
\else
\psk@thistreefit\pstree@theleftprofile\pstree@rightprofile
\kern-\pst@cnth sp
\pstree@zip\pstree@theleftprofile
\pstree@leftprofile\pstree@theleftprofile
\global\advance\pstree@cnt\pst@cnth
\pst@cnth=\pstree@cnt
\pstree@zip\pstree@rightprofile
\pstree@therightprofile\pstree@therightprofile
\fi
\box\pstree@box
\global\advance\psnodecnt 1\relax}%
\def\pstree@node@v{%
\edef\pstree@leftprofile{\psk@thistreenodesize\pst@dima,\pstree@stop,}%
\edef\pstree@rightprofile{\psk@thistreenodesize\pst@dimb,\pstree@stop,}%
\pssubtree@vertical}%
\def\pssubtree@horizontal@v{%
\pstree@max\pstree@upprofile\pst@cntg
\pst@dimc=\pst@cntg sp
\pstree@max\pstree@downprofile\pst@cntg
\pst@dimd=\pst@cntg sp
\pstree@treebboxadjust
\edef\pstree@leftprofile{\number\pst@dima,\pstree@stop,}%
\edef\pstree@rightprofile{\number\pst@dimb,\pstree@stop,}%
\pssubtree@vertical}%
\def\pstree@tightfit#1#2{%
\pst@cnth=\z@
\edef\next{\noexpand\pstree@@tightfit#1\noexpand\@nil#2\noexpand\@nil}%
\next
\advance\pst@cnth\psk@thistreesep\relax
\advance\pst@cnth\pstree@tspace\relax
\gdef\pstree@tspace{\z@}}
\def\pstree@@tightfit#1,#2\@nil#3,#4\@nil{%
\ifnum#1=\pstree@stop
\let\next\relax
\else
\ifnum#3=\pstree@stop
\let\next\relax
\else
\pst@cntg=#1
\advance\pst@cntg#3
\ifnum\pst@cntg>\pst@cnth
\pst@cnth=\pst@cntg
\fi
\def\next{\pstree@@tightfit#2\@nil#4\@nil}%
\fi
\fi
\next}
\def\pstree@loosefit#1#2{%
\pstree@max{#1}\pst@cnth
\pstree@max{#2}\pst@cntg
\advance\pst@cnth\pst@cntg
\advance\pst@cnth\psk@thistreesep\relax
\advance\pst@cnth\pstree@tspace\relax
\gdef\pstree@tspace{\z@}}
\def\tspace#1{%
\pst@@killglue
\pssetlength\pst@dimg{#1}%
\xdef\pstree@tspace{\number\pst@dimg}%
\ignorespaces}
\def\psset@treefit#1{%
\@ifundefined{pstree@#1fit}%
{\@pstrickserr{Bad `treefit' parameter value: `#1'}\@ehpa}%
{\expandafter\let\expandafter\psk@treefit\csname pstree@#1fit\endcsname}}
\psset@treefit{tight}
\def\psset@thistreefit#1{%
\@ifundefined{pstree@#1fit}%
{\@pstrickserr{Bad `treefit' parameter value: `#1'}\@ehpa}%
{\expandafter\let\expandafter\psk@thistreefit
\csname pstree@#1fit\endcsname}}
\psset@treefit{tight}
\def\pstree@zip#1#2#3{%
\def\pst@tempg{}%
\edef\next{\noexpand\pstree@@zip#1\noexpand\@nil#2\noexpand\@nil}%
\next
\global\let#3\pst@tempg}
\def\pstree@@zip#1,#2\@nil#3,#4\@nil{%
\ifnum#1=\pstree@stop
\edef\pst@tempg{\pst@tempg#3,#4}%
\let\next\relax
\else
\ifnum#3=\pstree@stop
\pst@cntg=#1
\advance\pst@cntg-\pst@cnth
\edef\pst@tempg{\pst@tempg\the\pst@cntg,}%
\def\next{\pstree@@zip#2\@nil\pstree@stop,\@nil}%
\else
\edef\pst@tempg{\pst@tempg#3,}%
\def\next{\pstree@@zip#2\@nil#4\@nil}%
\fi
\fi
\next}
\def\pstree@max#1#2{%
\pst@cntg=\z@
\expandafter\pstree@@max#1%
#2=\pst@cntg}%
\def\pstree@@max#1,{%
\ifnum#1=\pstree@stop\else
\ifnum#1>\pst@cntg \pst@cntg=#1 \fi
\expandafter\pstree@@max
\fi}
\def\pstree@add#1{%
\def\pst@tempg{}%
\expandafter\pstree@@add#1%
\xdef#1{\pst@tempg\pstree@stop,}}
\def\pstree@@add#1,{%
\ifnum#1=\pstree@stop\else
\pst@cnth=#1
\advance\pst@cnth\pst@cntg
\xdef\pst@tempg{\pst@tempg\the\pst@cnth,}%
\expandafter\pstree@@add
\fi}
\newcount\psnodecnt
\let\c@psnodecnt\psnodecnt
\newcount\pstreelevel
\let\c@pstreelevel\pstreelevel
\newcount\pstreecnt
\let\c@pstreecnt\pstreecnt
\newcount\pstree@cnt
\def\pstree{\def\pst@par{}\pst@object{pstree}}
\def\pstree@i{\def\pstree@makebox{\pst@@makebox}\pstree@ii}
\def\psTree{\def\pst@par{}\pst@object{psTree}}
\def\psTree@i{\def\pstree@makebox{\pst@makelongbox}\pstree@ii}
\def\endpsTree{\pst@endlongbox\ignorespaces}
\def\pstree@ii{%
\ifnum\pstreelevel=\z@
\let\pstree@savedshortput\pst@shortput
\psset@shortput{tab}%
\else
\pst@@killglue
\fi
\begingroup
\begingroup
\def\pstree@node{%
\xdef\pstree@next{%
\noexpand\@psttrue
\noexpand\def\noexpand\pst@tempa{\number\pst@dima}%
\noexpand\def\noexpand\pst@tempb{\number\pst@dimb}%
\noexpand\def\noexpand\pst@tempc{\number\pst@dimc}%
\noexpand\def\noexpand\pst@tempd{\number\pst@dimd}}%
\box\pstree@box}%
\def\pssubtree@horizontal{\pssubtree@horizontal@o}%
\def\pssubtree@vertical{\pssubtree@vertical@o}%
\global\let\pstree@next\relax
\pst@makebox\pstree@iii}
\def\pstree@iii{%
\global\setbox\pst@boxg=\box\pst@hbox
\endgroup
\setbox\pstree@rootbox=\box\pst@boxg
\@pstfalse
\pstree@next
\if@pst
\ifdim\wd\pstree@rootbox=\z@\else
\@pstrickserr{Extraneous space in root node}\@ehpa
\wd\pstree@rootbox=\z@
\fi
\else
\@pstrickserr{Missing or bad root node
(level \the\pstreelevel, node \the\psnodecnt)}\@ehpa
\def\pstree@next{%
\def\pst@tempa{0}%
\def\pst@tempb{0}%
\def\pst@tempc{0}%
\def\pst@tempd{0}}%
\wd\pstree@rootbox=\z@
\fi
\pstree@savevalues
\begingroup
\pstree@initsuccvalues
\pstree@setlevelpar
\pstree@do}
\def\pstree@setlevelpar{%
\advance\pstreelevel1
\let\psk@thislevelsep\relax
\let\psk@thistreesep\relax
\let\psk@thistreefit\relax
\let\psk@thistreenodesize\relax
\csname pstreehook\romannumeral\pstreelevel\endcsname
\use@par
\ifx\psk@thistreesep\relax
\let\psk@thistreesep\psk@treesep
\fi
\ifx\psk@thistreenodesize\relax
\let\psk@thistreenodesize\psk@treenodesize
\fi
\ifx\psk@thistreefit\relax
\let\psk@thistreefit\psk@treefit
\fi
\ifx\psk@thislevelsep\relax
\let\psk@thislevelsep\psk@levelsep
\let\psk@thislevelsepmode\psk@levelsepmode
\fi
\ifnum\psk@treemode=\pstree@predmode\else
\global\advance\pstreecnt1
\edef\pstree@thetree{\the\pstreecnt}%
\let\pstree@predmode\psk@treemode
\fi
\ifx\psk@thislevelsepmode\relax
\pst@dimg=\psk@thislevelsep\relax
\pst@cntg=0\@nameuse{%
pstree@levelsepadjust-\pstree@thetree-\the\pstreelevel}%
\advance\pst@dimg\pst@cntg sp
\edef\psk@thislevelsep{\number\pst@dimg sp}%
\fi
\ifnum\psk@treemode>1
\def\pst@tposflip{1 sub neg }%
\else
\def\pst@tposflip{}%
\fi
\ifx\pstree@bboxadjust\@empty\else
\xdef\pstree@treebboxadjust{%
\pstree@bboxadjust
\ifpsshowbbox\noexpand\pstree@showbbox\fi}%
\gdef\pstree@bboxadjust{}%
\fi
\let\pst@thispsbox\@skiplevelfalse}
\def\pstree@predmode{-1}
\def\pstree@savevalues{%
\edef\pstree@restorevalues{%
\noexpand\gdef\noexpand\pstree@theleftprofile{\pstree@theleftprofile}%
\noexpand\gdef\noexpand\pstree@therightprofile{\pstree@therightprofile}%
\noexpand\gdef\noexpand\pstree@theupprofile{\pstree@theupprofile}%
\noexpand\gdef\noexpand\pstree@thedownprofile{\pstree@thedownprofile}%
\noexpand\gdef\noexpand\pstree@tspace{\pstree@tspace}%
\noexpand\gdef\noexpand\pssucc{\pssucc}%
\global\psnodecnt=\the\psnodecnt\relax
\global\pstree@cnt=\the\pstree@cnt\relax}%
\let\pstree@savebboxadjust\pstree@treebboxadjust}
\def\pstree@initsuccvalues{%
\def\pstree@therightprofile{\pstree@stop,}%
\let\pstree@theleftprofile\pstree@therightprofile
\let\pstree@theupprofile\pstree@therightprofile
\let\pstree@thedownprofile\pstree@therightprofile
\psnodecnt=\z@
\pstree@cnt\z@
\gdef\pstree@tspace{\z@}%
\let\pspred\pssucc}
\def\pssucc{T}
\pstree@initsuccvalues
\def\pstree@down{%
\pstree@succrow
\pstree@makebox{\pstree@vertical{\lower}}}
\def\pstree@up{%
\pstree@succrow
\pstree@makebox{\pstree@vertical{\raise}}}
\def\pstree@levelsepadjust#1#2{%
% DG/SR modification begin - May 14, 1997 - Patch 1
% Problem with levelsep=*...
%\pst@cntg=0\@nameuse{pstree@levelsepadjust-#1}%
\pst@cntg=0\@nameuse{pstree@levelsepadjust-#1}
% DG/SR modification end
\ifnum#2>\pst@cntg
\expandafter\xdef\csname pstree@levelsepadjust-#1\endcsname
{#2}%
\fi}
\def\pstree@initlevelsepadjust{%
\@ifundefined{@latexerr}{%
\immediate\openin1 \jobname.pst
\ifeof1 \else
\input \jobname.pst
\fi
\immediate\closein1
\csname newwrite\endcsname\pstree@auxout
\immediate\openout\pstree@auxout \jobname.pst }%
{\let\pstree@auxout\@auxout}%
\global\let\pstree@initlevelsepadjust\relax}
\newcount\pstree@stop
\pstree@stop=-987654321
\def\pstree@vertical#1{%
\pst@cntg=\ifpstreeflip-\fi\wd\pst@hbox
\divide\pst@cntg 2
\pstree@add\pstree@theleftprofile
\pstree@add\pstree@therightprofile
\pst@dimg=\psk@thislevelsep\relax
\ifx\psk@thislevelsepmode\relax
\pstree@vertlevelsepadjust{#1}%
\fi
\global\setbox\pstree@box=\hbox{%
\vrule height \pst@tempc sp depth \pst@tempd sp width \z@
\unhbox\pstree@rootbox
#1\pst@dimg\hbox to\z@{\hss\unhbox\pst@hbox\hss}}%
\if@skiplevel
\skiplevel@vertical
\else
\endgroup
\fi
\edef\pstree@leftprofile{\pst@tempa,\pstree@theleftprofile}%
\edef\pstree@rightprofile{\pst@tempb,\pstree@therightprofile}%
\pst@dimc=\ht\pstree@box
\pst@dimd=\dp\pstree@box
\ifpsshowbbox
\pstree@max\pstree@leftprofile\pst@cntg
\pst@dima=\pst@cntg sp
\pstree@max\pstree@rightprofile\pst@cntg
\pst@dimb=\pst@cntg sp
\pstree@showbbox
\fi
\dp\pstree@box=\z@
\ht\pstree@box=\z@
\pstree@restorevalues
\pssubtree@vertical
\global\let\pstree@treebboxadjust\pstree@savebboxadjust
\endgroup
\ifnum\pstreelevel>\z@\expandafter\ignorespaces\fi}
\def\pstree@vertlevelsepadjust#1{%
\ifx\if@filesw\iffalse\else
\ifx#1\lower
\pst@dimh=\pst@tempd sp
\advance\pst@dimh\ht\pst@hbox
\else
\pst@dimh=\pst@tempc sp
\advance\pst@dimh\dp\pst@hbox
\fi
\immediate\write\@auxout{%
\string\pstree@levelsepadjust
{\pstree@thetree-\the\pstreelevel}{\number\pst@dimh}}%
\fi}
\def\pstree@succcolumn{%
\def\pssubtree@vertical{\pssubtree@vertical@h}%
\def\pssubtree@horizontal{\pssubtree@horizontal@h}%
\def\pstree@node{\pstree@node@h}}%
\def\pssubtree@horizontal@h{%
\xdef\pstree@theleftprofile{\number\pst@dima,\pstree@theleftprofile}%
\xdef\pstree@therightprofile{\number\pst@dimb,\pstree@therightprofile}%
\ifnum\psnodecnt=\z@
\global\let\pstree@theupprofile\pstree@upprofile
\global\let\pstree@thedownprofile\pstree@downprofile
\box\pstree@box
\else
\ifpstreeflip
\pssubtree@horizontal@@hflip
\else
\pssubtree@horizontal@@h
\fi
\fi
\global\advance\psnodecnt 1\relax}
\def\pssubtree@horizontal@@h{%
\psk@thistreefit\pstree@thedownprofile\pstree@upprofile
\global\advance\pstree@cnt\pst@cnth
\lower\the\pstree@cnt sp\box\pstree@box
\pstree@zip\pstree@thedownprofile\pstree@downprofile\pstree@thedownprofile
\pst@cnth=\pstree@cnt
\pstree@zip\pstree@upprofile\pstree@theupprofile\pstree@theupprofile}
\def\pssubtree@horizontal@@hflip{%
\psk@thistreefit\pstree@theupprofile\pstree@downprofile
\global\advance\pstree@cnt\pst@cnth
\raise\the\pstree@cnt sp\box\pstree@box
\pstree@zip\pstree@theupprofile\pstree@upprofile\pstree@theupprofile
\pst@cnth=\pstree@cnt
\pstree@zip\pstree@downprofile\pstree@thedownprofile\pstree@thedownprofile}
\def\pstree@node@h{%
\edef\pstree@upprofile{\psk@thistreenodesize\pst@dimc,\pstree@stop,}%
\edef\pstree@downprofile{\psk@thistreenodesize\pst@dimd,\pstree@stop,}%
\pssubtree@horizontal@h}%
\def\pssubtree@vertical@h{%
\pstree@max\pstree@leftprofile\pst@cntg
\pst@dima=\pst@cntg sp
\pstree@max\pstree@rightprofile\pst@cntg
\pst@dimb=\pst@cntg sp
\pstree@treebboxadjust
\edef\pstree@upprofile{\number\pst@dimc,\pstree@stop,}%
\edef\pstree@downprofile{\number\pst@dimd,\pstree@stop,}%
\pssubtree@horizontal@h}%
\newif\if@psrighttree
\def\pstree@right{%
\@psrighttreetrue
\pstree@succcolumn
\pstree@makebox\pstree@horizontal}
\def\pstree@left{%
\@psrighttreefalse
\pstree@succcolumn
\pstree@makebox\pstree@horizontal}
\def\pstree@horizontal{%
\ifdim\wd\pst@hbox=\z@\else
\@pstrickserr{Extraneous space in tree successors}\@ehpa
\fi
\pst@cntg=\ifpstreeflip\ht\else\dp\fi\pst@hbox
\divide\pst@cntg 2
\pstree@add\pstree@theupprofile
\pstree@add\pstree@thedownprofile
% DG/SR modification begin - Sep. 24, 1997 - Patch 3
%\ifx\psk@thislevelsepmode\relax
%\pstree@horizlevelsepadjust
%\fi
% DG/SR modification end
\pst@dimg\psk@thislevelsep\relax
\global\setbox\pstree@box=\hbox{%
\unhbox\pstree@rootbox
\kern\if@psrighttree\else-\fi\pst@dimg
\ifpstreeflip\lower\else\raise\fi\pst@cntg sp\box\pst@hbox}%
% DG/SR modification begin - Sep. 24, 1997 - Patch 3
\ifx\psk@thislevelsepmode\relax
\pstree@horizlevelsepadjust
\fi
% DG/SR modification end
\if@psrighttree
\pst@dimh=\pst@dimg
\pstree@max\pstree@therightprofile\pst@cntg
\global\advance\pst@dimh\pst@cntg sp
\global\pst@dimg=\pst@tempa sp
\else
\pstree@max\pstree@theleftprofile\pst@cntg
\global\advance\pst@dimg\pst@cntg sp
\global\pst@dimh=\pst@tempb sp
\fi
\if@skiplevel
\skiplevel@horizontal
\else
\endgroup
\fi
\pst@dima=\pst@dimg
\pst@dimb=\pst@dimh
\edef\pstree@upprofile{\pst@tempc,\pstree@theupprofile}%
\edef\pstree@downprofile{\pst@tempd,\pstree@thedownprofile}%
\dp\pstree@box=\z@
\ht\pstree@box=\z@
\wd\pstree@box=\z@
\ifpsshowbbox
\pstree@max\pstree@upprofile\pst@cntg
\pst@dimc=\pst@cntg sp
\pstree@max\pstree@downprofile\pst@cntg
\pst@dimd=\pst@cntg sp
\pstree@showbbox
\fi
\pstree@restorevalues
\pssubtree@horizontal
\endgroup
\ifnum\pstreelevel>\z@\expandafter\ignorespaces\fi}
% DG/SR modification begin - Sep. 24, 1997 - Patch 2
%\def\pstree@horizlevelsepadjust#1{%
\def\pstree@horizlevelsepadjust{%
% DG/SR modification end
\ifx\if@filesw\iffalse\else
\if@psrighttree
\pst@dimh=\pst@tempb sp
\pstree@max\pstree@theleftprofile\pst@cntg
\advance\pst@dimh\pst@cntg sp
\else
\pst@dimh=\pst@tempa sp
\pstree@max\pstree@therightprofile\pst@cntg
\advance\pst@dimh\pst@cntg sp
\fi
\immediate\write\@auxout{%
\string\pstree@levelsepadjust
{\pstree@thetree-\the\pstreelevel}{\number\pst@dimh}}%
\fi}
\def\psset@treemode#1{%
\pst@cntg=
\ifx#1U\@empty2\else\ifx#1R\@empty1\else\ifx#1L\@empty3\else0\fi\fi\fi
\relax
\edef\psk@treemode{\the\pst@cntg}%
\ifcase\pst@cntg
\let\pstree@do\pstree@down
\or
\let\pstree@do\pstree@right
\or
\let\pstree@do\pstree@up
\or
\let\pstree@do\pstree@left
\fi}
\def\psk@treemode{0}
\let\pstree@do\pstree@down
\def\psset@treesep#1{%
\pssetlength\pst@dimg{#1}%
\edef\psk@treesep{\number\pst@dimg}}%
\psset@treesep{.75cm}
\def\psset@thistreesep#1{%
\pssetlength\pst@dimg{#1}%
\edef\psk@thistreesep{\number\pst@dimg}}%
\def\psset@treenodesize#1{%
\pssetlength\pst@dimg{#1}%
\ifdim\pst@dimg<\z@
\let\psk@treenodesize\number
\else
\edef\psk@treenodesize{\number\pst@dimg\noexpand\@gobble}%
\fi}
\psset@treenodesize{-1pt}
\def\psset@thistreenodesize#1{%
\pssetlength\pst@dimg{#1}%
\ifdim\pst@dimg<\z@
\let\psk@thistreenodesize\number
\else
\edef\psk@thistreenodesize{\number\pst@dimg\noexpand\@gobble}%
\fi}
\def\psset@levelsep#1{%
\pst@expandafter{\pst@ifstar\psset@@levelsep}{#1}\@nil}
\def\psset@@levelsep#1\@nil{%
\pst@@getlength{#1}\psk@levelsep
\if@star
\pstree@initlevelsepadjust
\let\psk@levelsepmode\relax
\else
\def\psk@levelsepmode{}%
\fi}
\psset@levelsep{2cm}
\def\psset@thislevelsep#1{%
\pst@expandafter{\pst@ifstar\psset@@thislevelsep}{#1}\@nil}
\def\psset@@thislevelsep#1\@nil{%
\pst@@getlength{#1}\psk@thislevelsep
\if@star
\pstree@initlevelsepadjust
\let\psk@thislevelsepmode\relax
\else
\def\psk@thislevelsepmode{}%
\fi}
\newif\ifpstreeflip
\def\psset@treeflip#1{\@nameuse{pstreeflip#1}}
\psset@treeflip{false}
\def\pstree@node@o{%
\leavevmode
\hbox{%
\vrule height \pst@dimc depth \pst@dimd width \z@
\kern\pst@dima
\box\pstree@box
\kern\pst@dimb}}
\def\pssubtree@vertical@o{%
\pstree@max\pstree@leftprofile\pst@cntg
\pst@dima=\pst@cntg sp
\pstree@max\pstree@rightprofile\pst@cntg
\pst@dimb=\pst@cntg sp
\pstree@treebboxadjust
\pstree@node}
\def\pssubtree@horizontal@o{%
\pstree@max\pstree@upprofile\pst@cntg
\pst@dimc=\pst@cntg sp
\pstree@max\pstree@downprofile\pst@cntg
\pst@dimd=\pst@cntg sp
\pstree@treebboxadjust
\pstree@node}
\def\pstree@outer{%
\def\pstree@node{\pstree@node@o}%
\def\pssubtree@vertical{\pssubtree@vertical@o}%
\def\pssubtree@horizontal{\pssubtree@horizontal@o}%
\pstreelevel=\z@
\def\pstree@predmode{-1}%
\def\pst@tposflip{}%
\let\pst@thisbox\relax
\let\pst@shortput\pstree@savedshortput}
\let\pstree@savedshortput\ignorespaces
\pstree@outer
\newif\ifpsshowbbox
\def\psset@showbbox#1{\@nameuse{psshowbbox#1}}%
\psset@showbbox{false}
\def\pstree@showbbox{%
\setbox\pstree@box=\hbox{%
\psframe[linewidth=0,linecolor=black,linestyle=solid,fillstyle=none]%
(-\pst@dima,-\pst@dimd)(\pst@dimb,\pst@dimc)%
\box\pstree@box}}%
\def\psset@edge#1{%
\def\psedge{#1}%
\ifx\psedge\@none
\def\psedge##1##2{}%
\fi}
\psset@edge{\ncline}
\def\pspred{T}
\def\pstree@makenodebox{%
\pst@@killglue
\let\pst@thispsbox\pstree@outer
\pst@makebox}
\def\begin@treenode{%
\pst@@killglue
\begingroup
\use@par
\global\let\pstree@edge\psedge
\xdef\pssucc{\pspred-\the\psnodecnt}}
\def\MakeShortTnput#1{%
\def\end@treenode{\@ifnextchar#1{\tnput@}{\end@@treenode}}}
\MakeShortTnput{~}
\def\end@@treenode{%
\pstree@bboxadjust
\gdef\pstree@bboxadjust{}%
\ifpsshowbbox\pstree@showbbox\fi
\pstree@node
\endgroup
\ifnum\pstreelevel>\z@
\pstree@edge{\pspred}{\pssucc}%
\expandafter\pst@shortput
\else
\expandafter\ignorespaces
\fi}
\def\pstree@bboxadjust{}
\def\pstree@setbboxadjust#1#2{%
\pssetlength\pst@dimg{#1}%
\xdef\pstree@bboxadjust{%
\pstree@bboxadjust
#2\number\pst@dimg sp\relax}}
\def\psset@bbl#1{\pstree@setbboxadjust{#1}{\pst@dima=}}
\def\psset@bbr#1{\pstree@setbboxadjust{#1}{\pst@dimb=}}
\def\psset@bbh#1{\pstree@setbboxadjust{#1}{\pst@dimc=}}
\def\psset@bbd#1{\pstree@setbboxadjust{#1}{\pst@dimd=}}
\def\psset@xbbl#1{\pstree@setbboxadjust{#1}{\advance\pst@dima}}
\def\psset@xbbr#1{\pstree@setbboxadjust{#1}{\advance\pst@dimb}}
\def\psset@xbbh#1{\pstree@setbboxadjust{#1}{\advance\pst@dimc}}
\def\psset@xbbd#1{\pstree@setbboxadjust{#1}{\advance\pst@dimd}}
\let\pstree@treebboxadjust\relax
\def\Tn{\def\pst@par{}\pst@object{Tn}}
\def\Tn@i{%
\pst@@killglue
\global\let\pssucc\pspred
\begingroup
\pst@dima=\z@
\pst@dimb=\z@
\pst@dimc=\z@
\pst@dimd=\z@
\setbox\pstree@box=\hbox{}%%
\pstree@node
\endgroup
\ignorespaces}
\def\Tp{\def\pst@par{}\pst@object{Tp}}
\def\Tp@i{%
\begin@treenode
\pst@dima=\z@
\pst@dimb=\z@
\pst@dimc=\z@
\pst@dimd=\z@
\setbox\pstree@box=\hbox{%
\pst@newnode{\pssucc}{10}{0 0 }{\tx@InitPnode}}%
\end@treenode}
\def\Tc{\def\pst@par{}\pst@object{Tc}}
\def\Tc@i#1{%
\begin@treenode
\pssetlength\pst@dima{#1}%
\pst@dimb=\pst@dima
\pst@dimc=\pst@dima
\pst@dimd=\pst@dima
\nodealignfalse
\setbox\pstree@box=\hbox{\cnode@ii(\z@,\z@){#1}{\pssucc}}%
\end@treenode}
\def\TC{\def\pst@par{}\pst@object{TC}}
\def\TC@i{\Tc@i{\psk@radius}}
\def\Toval{\def\pst@par{}\pst@object{Toval}}
\def\Toval@i{\pstree@makenodebox{\Toval@ii\ovalnode@ii}}
\def\Toval@ii#1{%
\begin@treenode
\nodealigntrue
\setbox\pstree@box=\hbox{#1\pssucc}%
\pst@dima=\wd\pstree@box
\divide\pst@dima 2
\pst@dimb=\pst@dima
\pst@dimc=\ht\pstree@box
\pst@dimd=\dp\pstree@box
\setbox\pstree@box=\hbox to\z@{\hss\unhbox\pstree@box\hss}%
\dp\pstree@box=\z@
\ht\pstree@box=\z@
\end@treenode}
\def\Tcircle{\def\pst@par{}\pst@object{Tcircle}}
\def\Tcircle@i{\pstree@makenodebox{\Toval@ii\circlenode@ii}}
\def\Tf{\def\pst@par{}\pst@object{Tf}}
\def\Tf@i{\Toval@ii{\fnode@ii()}}
\def\Tdia{\def\pst@par{}\pst@object{Tdia}}
\def\Tdia@i{\pstree@makenodebox{\Toval@ii\dianode@ii}}
\def\Ttri{\def\pst@par{}\pst@object{Ttri}}
\def\Ttri@i{\pstree@makenodebox{\Ttri@ii}}
\def\Ttri@ii{%
\begin@treenode
\nodealigntrue
\setbox\pstree@box=\hbox{\trinode@ii\pssucc}%
\pst@dima=\pst@dimg % Set by \pst@triboxsep
\pst@dimb=\wd\pstree@box
\advance\pst@dimb-\pst@dima
\pst@dimc=\ht\pstree@box
\pst@dimd=\dp\pstree@box
\setbox\pstree@box=\hbox to\z@{\hss\unhbox\pstree@box\hss}%
\dp\pstree@box=\z@
\ht\pstree@box=\z@
\end@treenode}
\def\Tr{\def\pst@par{}\pst@object{Tr}}
% SR modification begin - Oct. 27, 1996
%\def\Tr@i{\pstree@makenodebox{\Tr@ii{\begingroup\rnode@ii}}}
\def\Tr@i{\pstree@makenodebox{\Tr@ii{\rnode@iii\rnode@iv}}}
% SR modification end
\def\Tr@ii#1{%
\begin@treenode
\def\pstree@nodehook{%
\xdef\pstree@next{\pst@dima=\number\pst@dima sp\relax}}%
\nodealigntrue
\setbox\pstree@box\hbox{#1\pssucc}%
\pstree@next
\pst@dimb=\wd\pstree@box
\advance\pst@dimb-\pst@dima
\pst@dimc=\ht\pstree@box
\pst@dimd=\dp\pstree@box
\setbox\pstree@box\hbox to\z@{\kern-\pst@dima\unhbox\pstree@box\hss}%
\ht\pstree@box=\z@
\dp\pstree@box=\z@
\end@treenode}
\def\TR{\def\pst@par{}\pst@object{TR}}
% DG modification begin - Oct. 25, 1996
%\def\TR@i{\pstree@makenodebox{\Tr@ii{\Rnode@ii}}}
\def\TR@i{\pstree@makenodebox{\Tr@ii{\rnode@iii\Rnode@ii}}}
% DG modification end
\def\Tdot{\def\pst@par{}\pst@object{Tdot}}
\def\Tdot@i{%
\begin@treenode
\def\pstree@nodehook{\xdef\pstree@next{%
\pst@dima=\number\pst@dima sp\relax
\pst@dimc=\number\pst@dimb sp\relax}}%
\nodealignfalse
\setbox\pstree@box=\hbox{\dotnode@ii(\z@,\z@)\pssucc}%
\pstree@next
\pst@dimb=\pst@dima
\pst@dimd=\pst@dimc
\end@treenode}
\def\psset@fansize#1{\pst@@getlength{#1}\psk@fansize}
\psset@fansize{1cm}
\def\Tfan{\def\pst@par{}\pst@object{Tfan}}
\def\Tfan@i{%
\addto@par{edge=none}%
\begin@treenode
\solid@star
\pst@dimb=\psk@fansize
\pst@dimd=\pslinewidth
\advance\pst@dimb-\pst@dimd
\divide\pst@dimb 2
\divide\pst@dimd 2
\ifodd\psk@treemode\relax
\pst@dima=\pst@dimd
\pst@dimc=\pst@dimb
\else
\pst@dima=\pst@dimb
\pst@dimc=\pst@dimd
\fi
\setbox\pstree@box=\hbox{%
\pst@newnode{\pssucc}{16}{}{%
/Y 0 def
/X 0 def
/l \pst@number\pst@dima def
/r l def
/u \pst@number\pst@dimc def
/d u def
/NodePos { \tx@GetRnodePos } def}%
\def\pst@linetype{1}%
\nc@object{Closed}{\pspred}{\pssucc}{.5}{%
tx@Dict begin \psline@iii pop end
/w \pst@number\pst@dimb CLW 2 div sub def
/m \ifodd\psk@treemode false \else true \fi def
\tx@Tfan}}%
\pst@dimb=\pst@dima
\pst@dimd=\pst@dimc
\end@treenode}
\def\psset@tnsep#1{%
\def\pst@tempg{#1}%
\ifx\pst@tempg\@empty
\def\psk@tnsep{\number\pslabelsep sp}%
\else
\pst@@getlength{#1}\psk@tnsep
\fi}
\psset@tnsep{}
\def\psset@tnyref#1{\def\psk@tnyref{#1}}%
\psset@tnyref{}
\def\psset@tnheight#1{\edef\psk@tnheight{#1}}
\psset@tnheight{\ht\strutbox}
\def\psset@tndepth#1{\edef\psk@tndepth{#1}}
\psset@tndepth{\dp\strutbox}
\def\psset@tnpos#1{%
\def\pst@tempg{#1}%
\ifx\pst@tempg\@empty
\def\psk@tnpos{%
\ifcase\psk@treemode b\or r\or a\or l\fi}%
\else
\@ifundefined{pstree@tnput@#1}%
{\@pstrickserr{Bad tnpos: `#1'}\@ehpa}%
{\edef\psk@tnpos{#1}}%
\fi}
\psset@tnpos{}
\def\tnput@#1{\def\pst@par{}\pst@object{tnput}}
\def\tnput@i{\pstree@makenodebox{\tnput@ii}}
\def\tnput@ii{%
\begingroup
\use@par
\xdef\next{%
\if@star\noexpand\pst@starbox\fi
\noexpand\def\noexpand\psk@thistndepth{\psk@tndepth}%
\noexpand\def\noexpand\psk@thistnheight{\psk@tnheight}%
\noexpand\def\noexpand\psk@thistnyref{\psk@tnyref}%
\noexpand\def\noexpand\psk@thistnsep{\psk@tnsep}%
\expandafter\noexpand\csname pstree@tnput@\psk@tnpos\endcsname}%
\endgroup
\next
\end@treenode}
\@namedef{pstree@tnput@b}{%
\pstree@tnput@@v\pst@dimd\ht\dp\lower\psk@thistnheight}
\@namedef{pstree@tnput@a}{%
\pstree@tnput@@v\pst@dimc\dp\ht\raise\psk@thistndepth}
\def\pstree@tnput@@v#1#2#3#4#5{%
\pst@dimh=\wd\pst@hbox
\pst@dimg=\psk@href\pst@dimh
\advance\pst@dimg\pst@dimh
\divide\pst@dimg 2
\advance\pst@dimh-\pst@dimg
\ifdim\pst@dimg>\pst@dima
\pst@dima=\pst@dimg
\fi
\ifdim\pst@dimh>\pst@dimb
\pst@dimb=\pst@dimh
\fi
\pst@dimh=\psk@thistnsep\relax
\ifdim\pst@dimh<\z@
\pst@dimh=-\pst@dimh
\else
\advance\pst@dimh#1%
\fi
\pssetlength\dimen@{#5}%
\ifdim\dimen@>#2\pst@hbox
\advance\pst@dimh\dimen@\relax
\else
\advance\pst@dimh#2\pst@hbox
\fi
\setbox\pstree@box=\hbox{%
\box\pstree@box
#4\pst@dimh\hbox to\z@{\kern-\pst@dimg\unhbox\pst@hbox\hss}}%
#1=#3\pstree@box
\dp\pstree@box=\z@
\ht\pstree@box=\z@}
\@namedef{pstree@tnput@l}{%
\pstree@tnput@@h\pst@dima{%
\hss
\lower\pst@dimg\box\pst@hbox
\kern\pst@dimh
\box\pstree@box}}
\@namedef{pstree@tnput@r}{%
\pstree@tnput@@h\pst@dimb{%
\box\pstree@box
\kern\pst@dimh
\lower\pst@dimg\box\pst@hbox
\hss}}%
\def\pstree@tnput@@h#1#2{%
\ifx\psk@thistnyref\@empty
\pssetlength\pst@dimg\psk@vref
\else
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg\dp\pst@hbox
\pst@dimg=\psk@thistnyref\pst@dimg
\advance\pst@dimg-\dp\pst@hbox
\fi
\pst@dimh=\psk@thistnsep\relax
\ifdim\pst@dimh<\z@
\pst@dimh=-\pst@dimh
\else
\advance\pst@dimh#1%
\fi
#1=\pst@dimh
\advance#1\wd\pst@hbox
\setbox\pstree@box=\hbox to\z@{#2}%
\ifdim\ht\pstree@box>\pst@dimc
\pst@dimc=\ht\pstree@box
\fi
\ifdim\dp\pstree@box>\pst@dimd
\pst@dimd=\dp\pstree@box
\fi
\dp\pstree@box=\z@
\ht\pstree@box=\z@}
\newif\if@skiplevel
\def\skiplevel{\def\pst@par{}\pst@object{skiplevel}}
\def\skiplevel@i{\def\pstree@makebox{\pst@@makebox}\skiplevel@ii}
\def\skiplevel@ii{%
\pst@@killglue
\begingroup
\let\pssucc\pspred
\def\pst@tempa{0}%
\def\pst@tempb{0}%
\def\pst@tempc{0}%
\def\pst@tempd{0}%
\setbox\pstree@rootbox=\hbox{}%
\pstree@savevalues
\begingroup
\pstree@initsuccvalues
\pstree@setlevelpar
\@skipleveltrue
\pstree@do}
\def\pstree@gettop#1{\expandafter\pstree@@gettop#1\@nil}
\def\pstree@@gettop#1,#2\@nil{#1}
\def\skiplevel@horizontal{%
\pst@dimc=\pstree@gettop\pstree@theupprofile sp
\pst@dimd=\pstree@gettop\pstree@thedownprofile sp
\pstree@treebboxadjust
\gdef\pstree@treebboxadjust{}%
\xdef\pstree@next{%
\noexpand\def\noexpand\pst@tempc{\number\pst@dimc}%
\noexpand\def\noexpand\pst@tempd{\number\pst@dimd}}%
\endgroup
\pstree@next}
\def\skiplevel@vertical{%
\pst@dima=\pstree@gettop\pstree@theleftprofile sp
\pst@dimb=\pstree@gettop\pstree@therightprofile sp
\pstree@treebboxadjust
\gdef\pstree@treebboxadjust{}%
\xdef\pstree@next{%
\noexpand\def\noexpand\pst@tempa{\number\pst@dima}%
\noexpand\def\noexpand\pst@tempb{\number\pst@dimb}}%
\endgroup
\pstree@next}
\def\skiplevels{\def\pst@par{}\pst@object{skiplevels}}
\def\skiplevels@i#1{%
\pst@@killglue
\begingroup
\pst@cnta=#1\relax
\edef\skiplevels@num{\the\pst@cnta}%
\def\pstree@makebox{\pst@makelongbox}%
\def\endskiplevels{}%
\loop
\ifnum\pst@cnta>\z@
\advance\pst@cnta-1
\expandafter\def\expandafter\endskiplevels\expandafter{%
\endskiplevels\pst@endlongbox}
\skiplevel@ii
\repeat
\expandafter\def\expandafter\endskiplevels\expandafter{%
\endskiplevels\endgroup\ignorespaces}
\ignorespaces}

\catcode`\@=\TheAtCode\relax

\endinput
%%
%% END: pst-tree.tex


==> texmf/tex/latex/pstricks/pstricks.tex <==
%% BEGIN: pstricks.tex
%%
%% PostScript macros for Generic TeX: main input file for PSTricks 97.
%% See the PSTricks User's Guide for description.
%% This uses the header file `pstricks.pro'.
%%
\def\fileversion{97 patch 10}
\def\filedate{1999/03/24}
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\csname PSTricksLoaded\endcsname
\let\PSTricksLoaded\endinput
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
\expandafter\ifx\csname @latexerr\endcsname\relax
\long\def\@ifundefined#1#2#3{\expandafter\ifx\csname
#1\endcsname\relax#2\else#3\fi}
\def\@namedef#1{\expandafter\def\csname #1\endcsname}
\def\@nameuse#1{\csname #1\endcsname}
\def\@eha{%
Your command was ignored.^^J
Type \space I <command> <return> \space to replace
it with another command,^^J
or \space <return> \space to continue without it.}
\def\@spaces{\space\space\space\space}
\def\typeout#1{\immediate\write\@unused{#1}}
\alloc@7\write\chardef\sixt@@n\@unused
\def\@empty{}
\def\@gobble#1{}
\def\@nnil{\@nil}
\def\@ifnextchar#1#2#3{%
\let\@tempe#1\def\@tempa{#2}\def\@tempb{#3}\futurelet\@tempc\@ifnch}
\def\@ifnch{%
\ifx\@tempc\@sptoken
\let\@tempd\@xifnch
\else
\ifx\@tempc\@tempe \let\@tempd\@tempa \else \let\@tempd\@tempb \fi
\fi
\@tempd}
\begingroup
\def\:{\global\let\@sptoken= } \:
\def\:{\@xifnch} \expandafter\gdef\: {\futurelet\@tempc\@ifnch}
\endgroup
\fi
\typeout{`PSTricks' v\fileversion\space\space <\filedate> (tvz)}
\def\@pstrickserr#1#2{%
\begingroup
\newlinechar`\^^J
\edef\pst@tempc{#2}%
\expandafter\errhelp\expandafter{\pst@tempc}%
\typeout{%
PSTricks error. \space See User's Guide for further information.^^J
\@spaces\@spaces\@spaces\@spaces
Type \space H <return> \space for immediate help.}%
\errmessage{#1}%
\endgroup}
\def\@ehpa{%
Your command was ignored. Default value substituted.^^J
Type \space <return> \space to procede.}
\def\@ehpb{%
Your command was ignored. Will recover best I can.^^J
Type \space <return> \space to procede.}
\def\@ehpc{%
You better fix this before proceding.^^J
See the PSTricks User's Guide or ask your system administrator for help.^^J
Type \space X <return> \space to quit.}
\def\pst@misplaced#1{\@pstrickserr{Misplaced \string#1 command}\@ehpb}
\newdimen\pst@dima
\newdimen\pst@dimb
\newdimen\pst@dimc
\newdimen\pst@dimd
\newdimen\pst@dimg
\newdimen\pst@dimh
\newbox\pst@hbox
\newbox\pst@boxg
\newcount\pst@cnta
\newcount\pst@cntb
\newcount\pst@cntc
\newcount\pst@cntd
\newcount\pst@cntg
\newcount\pst@cnth
\newif\if@pst
\newtoks\pst@toks
\newif\if@star
\def\pst@ifstar#1{%
\@ifnextchar*{\@startrue\def\next*{#1}\next}{\@starfalse#1}}
\def\pst@expandafter#1#2{%
\def\next{#1}%
\edef\@tempa{#2}%
\ifx\@tempa\@empty
\@pstrickserr{Unexpected empty argument!}\@ehpb
\def\@tempa{\@empty}%
\fi
\expandafter\next\@tempa}
\def\pst@dimtonum#1#2{\edef#2{\pst@@dimtonum#1}}
\def\pst@@dimtonum#1{\expandafter\pst@@@dimtonum\the#1}
{\catcode`\p=12 \catcode`\t=12 \global\@namedef{pst@@@dimtonum}#1pt{#1}}
\def\pst@pyth#1#2#3{%
\ifdim#1>#2\pst@@pyth#1#2#3\else\pst@@pyth#2#1#3\fi}
\def\pst@@pyth#1#2#3{%
\ifdim4#1>9#2%
#3=#1\advance#3 .2122#2%
\else
#3=.8384#1\advance#3 .5758#2%
\fi}
\def\pst@divide#1#2#3{%
\pst@@divide{#1}{#2}%
\pst@dimtonum\pst@dimg{#3}}
\def\pst@@divide#1#2{%
\pst@dimg=#1\relax
\pst@dimh=#2\relax
\pst@cntg=\pst@dimh
\pst@cnth=67108863
\pst@@@divide\pst@@@divide\pst@@@divide\pst@@@divide
\divide\pst@dimg\pst@cntg}
\def\pst@@@divide{%
\ifnum
\ifnum\pst@dimg<\z@-\fi\pst@dimg<\pst@cnth
\multiply\pst@dimg\sixt@@n
\else
\divide\pst@cntg\sixt@@n
\fi}
\def\pst@configerr#1{%
\@pstrickserr{\string#1 not defined in pstricks.con}\@ehpc}
% % \begin{macrocode}
\def\pstVerb#1{\pst@configerr\pstVerb}
\def\pstverb#1{\pst@configerr\pstverb}
\def\pstverbscale{\pst@configerr\pstverbscale}
\def\pstrotate{\pst@configerr\pstrotate}
\def\pstheader#1{\pst@configerr\pstheader}
\def\pstdriver{\pst@configerr\pstdriver}
\@ifundefined{pstcustomize}%
{\def\pstcustomize{\endinput\let\pstcustomize\relax}}{}
\input pstricks.con
\newif\ifPSTricks
\PSTrickstrue
\def\PSTricksOff{%
\def\pstheader##1{}%
\def\pstverb##1{}%
\def\pstVerb##1{}%
\PSTricksfalse}
\@ifundefined{pst@def}{\def\pst@def#1<#2>{\@namedef{tx@#1}{#2 }}}{}
\@ifundefined{pst@ATH}{\def\pst@ATH<#1>{}}{}
\pstheader{pstricks.pro}
\def\pst@dict{tx@Dict begin }
\def\pst@theheaders{pstricks.pro}
\def\pst@Verb#1{\pstVerb{\pst@dict #1 end}}
\def\tx@Atan{Atan }
\def\tx@Div{Div }
\def\tx@NET{NET }
\def\tx@Pyth{Pyth }
\def\tx@PtoC{PtoC }
\def\tx@PathLength@{PathLength@ }
\def\tx@PathLength{PathLength }
\pst@dimg=\pstunit\relax
\ifdim\pst@dimg=1bp
\def\pst@stp{.996264 dup scale}
\else
\edef\pst@stp{1 \pst@@dimtonum\pst@dimg\space div dup scale}
\fi
\def\tx@STP{STP }
\def\tx@STV{STV }
\def\pst@number#1{\pst@@dimtonum#1\space}
\def\pst@checknum#1#2{%
\edef\next{#1}%
\ifx\next\@empty
\let\pst@num\z@
\else
\expandafter\pst@@checknum\next..\@nil
\fi
\ifnum\pst@num=\z@
\@pstrickserr{Bad number: `#1'. 0 substituted.}\@ehpa
\def#2{0 }%
\else
\edef#2{\ifnum\pst@num=\tw@-\fi\the\pst@cntg.%
\expandafter\@gobble\the\pst@cnth\space}%
\fi}
\def\pst@@checknum{%
\@ifnextchar-%
{\let\pst@num\tw@\expandafter\pst@@@checknum\@gobble}%
{\let\pst@num\@ne\pst@@@checknum}}
\def\pst@@@checknum#1.#2.#3\@nil{%
\afterassignment\pst@@@@checknum\pst@cntg=0#1\relax\@nil
\afterassignment\pst@@@@checknum\pst@cnth=1#2\relax\@nil}
\def\pst@@@@checknum#1\relax\@nil{%
\ifx\@nil#1\@nil\else\let\pst@num\z@\fi}
\def\pst@getnumii#1 #2 #3\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph}
\def\pst@getnumiii#1 #2 #3 #4\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph
\pst@checknum{#3}\pst@tempi}
\def\pst@getnumiv#1 #2 #3 #4 #5\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph
\pst@checknum{#3}\pst@tempi
\pst@checknum{#4}\pst@tempj}
\def\pst@getdimnum#1 #2 #3\@nil{%
\pssetlength\pst@dimg{#1}%
\pst@checknum{#2}\pst@tempg}
% DG/SR modification begin - Jan. 7, 1998 - Patch 9
% Missing from pstricks.bug 0.93
%\def\pst@getscale#1#2{%
%\pst@expandafter\pst@getnumii{#1 #1} {} {} {}\@nil
%\@psttrue
%\ifdim\pst@tempg\p@=\z@
%\@pstrickserr{Bad scaling argument `#1'}\@ehpa
%\def\pst@tempg{1 }%
%\@pstfalse
%\fi
%\ifdim\pst@temph\p@=\z@
%\if@pst\@pstrickserr{Bad scaling argument `#1'}\@ehpa\fi
%\def\pst@temph{1 }%
%\fi
%\edef#2{\pst@tempg\space \pst@temph\space scale }%
%\ifdim\pst@tempg\p@=\p@ \ifdim\pst@temph\p@=\p@
%\def#2{}%
%\fi\fi}
\def\pst@getscale#1#2{%
\edef\pst@tempg{#1}%
\ifx\pst@tempg\@none
\def#2{}%
\else
\pst@expandafter\pst@getnumii{#1 #1} {} {} {}\@nil
\ifdim\pst@tempg\p@=\z@
\@pstrickserr{Bad scaling argument `#1'}\@ehpa
\def#2{}%
\else
\ifdim\pst@temph\p@=\z@
\@pstrickserr{Bad scaling argument `#1'}\@ehpa
\def#2{}%
\else
\edef#2{\pst@tempg\space \pst@temph\space scale }%
\fi
\fi
\fi}
% DG/SR modification end
\def\pst@getint#1#2{%
\pst@cntg=#1\relax
\edef#2{\the\pst@cntg\space}}
\begingroup
\catcode`\{=12
\catcode`\}=12
\catcode`\[=1
\catcode`\]=2
\gdef\pslbrace[{ ]
\gdef\psrbrace[} ]
\endgroup
\def\@newcolor#1#2{%
\expandafter\edef\csname #1\endcsname{\noexpand\pst@color{#2}}%
\expandafter\edef\csname color@#1\endcsname{#2}%
\ignorespaces}
\def\pst@color#1{%
\def\pst@currentcolor{#1}\pstVerb{#1}\aftergroup\pst@endcolor}
\def\pst@endcolor{\pstVerb{\pst@currentcolor}}
\def\pst@currentcolor{0 setgray}
\def\altcolormode{%
\def\pst@color##1{%
\pstVerb{gsave ##1}\aftergroup\pst@endcolor}%
\def\pst@endcolor{\pstVerb{\pst@grestore}}}
\def\pst@grestore{%
currentpoint
matrix currentmatrix
currentfont
grestore
setfont
setmatrix
moveto}
\def\pst@usecolor#1{\csname color@#1\endcsname\space}
\def\newgray#1#2{%
\pst@checknum{#2}\pst@tempg
\@newcolor{#1}{\pst@tempg setgray}}
\def\newrgbcolor#1#2{%
\pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
\@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi setrgbcolor}}
\def\newhsbcolor#1#2{%
\pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
\@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi sethsbcolor}}
\def\newcmykcolor#1#2{%
\pst@expandafter\pst@getnumiv{#2} {} {} {} {} {}\@nil
\@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi \pst@tempj setcmykcolor}}
\newgray{black}{0}
\newgray{darkgray}{.25}
\newgray{gray}{.5}
\newgray{lightgray}{.75}
\newgray{white}{1}
\newrgbcolor{red}{1 0 0}
\newrgbcolor{green}{0 1 0}
\newrgbcolor{blue}{0 0 1}
\newrgbcolor{yellow}{1 1 0}
\newrgbcolor{cyan}{0 1 1}
\newrgbcolor{magenta}{1 0 1}
\def\psset#1{\@psset#1,\@nil\ignorespaces}
\def\@psset#1,{%
\@@psset#1==\@nil
\@ifnextchar\@nil{\@gobble}{\@psset}}
\def\@@psset#1=#2=#3\@nil{%
\@ifundefined{psset@#1}%
{\@pstrickserr{Graphics parameter `#1' not defined.}\@ehpa}%
{\@nameuse{psset@#1}{#2}}}%
\def\psset@style#1{%
\@ifundefined{pscs@#1}%
{\@pstrickserr{Custom style `#1' undefined}\@ehpa}%
{\@nameuse{pscs@#1}}}
\def\newpsstyle#1#2{\@namedef{pscs@#1}{\psset{#2}}}
\def\@none{none}
\def\pst@getcolor#1#2{%
\@ifundefined{color@#1}%
{\@pstrickserr{Color `#1' not defined}\@eha}%
{\edef#2{#1}}}
\newdimen\psunit \psunit 1cm
\newdimen\psxunit \psxunit 1cm
\newdimen\psyunit \psyunit 1cm
\let\psrunit\psunit
\def\pstunit@off{\let\@psunit\ignorespaces\ignorespaces}
\def\pssetlength#1#2{%
\let\@psunit\psunit
\afterassignment\pstunit@off
#1 #2\@psunit}
\def\psaddtolength#1#2{%
\let\@psunit\psunit
\afterassignment\pstunit@off
\advance#1 #2\@psunit}
\def\pssetxlength#1#2{%
\let\@psunit\psxunit
\afterassignment\pstunit@off
#1 #2\@psunit}
\def\pssetylength#1#2{%
\let\@psunit\psyunit
\afterassignment\pstunit@off
#1 #2\@psunit}
\def\psset@unit#1{%
\pssetlength\psunit{#1}%
\psxunit=\psunit
\psyunit=\psunit}
\def\psset@runit#1{\pssetlength\psrunit{#1}}
\def\psset@xunit#1{\pssetxlength\psxunit{#1}}
\def\psset@yunit#1{\pssetylength\psyunit{#1}}
\def\pst@getlength#1#2{%
\pssetlength\pst@dimg{#1}%
\edef#2{\pst@number\pst@dimg}}
\def\pst@@getlength#1#2{%
\pssetlength\pst@dimg{#1}%
\edef#2{\number\pst@dimg sp}}
\def\pst@getcoor#1#2{\pst@@getcoor{#1}\let#2\pst@coor}
\def\pst@coor{0 0 }
\def\pst@getcoors#1#2{%
\def\pst@aftercoors{\addto@pscode{#1 \pst@coors }#2}%
\def\pst@coors{}%
\pst@@getcoors}
\def\pst@@getcoors(#1){%
\pst@@getcoor{#1}%
\edef\pst@coors{\pst@coor\pst@coors}%
\@ifnextchar({\pst@@getcoors}{\pst@aftercoors}}
\def\pst@getangle#1#2{\pst@@getangle{#1}\let#2\pst@angle}
\def\pst@angle{0 }
\def\cartesian@coor#1,#2,#3\@nil{%
\pssetxlength\pst@dimg{#1}%
\pssetylength\pst@dimh{#2}%
\edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}}
\def\NormalCoor{%
\def\pst@@getcoor##1{\pst@expandafter\cartesian@coor{##1},\relax,\@nil}%
\def\pst@@getangle##1{%
\pst@checknum{##1}\pst@angle
\edef\pst@angle{\pst@angle \pst@angleunit}}%
\def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@cartesian}}
\NormalCoor
\def\degrees{\@ifnextchar[{\@degrees}{\def\pst@angleunit{}}}
\def\@degrees[#1]{%
\pst@checknum{#1}\pst@tempg
\edef\pst@angleunit{360 \pst@tempg div mul }%
\ignorespaces}
\def\radians{\def\pst@angleunit{57.2956 mul }}
\def\pst@angleunit{}
\def\SpecialCoor{%
\def\pst@@getcoor##1{%
\begingroup
\pst@activecoor
\xdef\pst@tempg{##1}%
\endgroup
\expandafter\special@coor\pst@tempg||\@nil}%
\def\pst@@getangle##1{%
\begingroup
\pst@activecoor
\xdef\pst@tempg{##1}%
\endgroup
\expandafter\special@angle\pst@tempg\@empty)\@nil}%
\def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@special}}
\begingroup
\catcode`\|=13
\catcode`\;=13
\catcode`\!=13
\gdef\pst@activecoor{%
\def|{\string|}%
\def;{\string;}%
\def!{\string!}}
\endgroup
\def\special@coor#1|#2|#3\@nil{%
\ifx#3|\relax
\mixed@coor{#1}{#2}%
\else
\special@@coor#1;;\@nil
\fi}
\def\special@@coor#1{%
\ifcat#1a\relax
\def\next{\node@coor#1}%
\else
\ifx#1[\relax
\def\next{\Node@coor[}%
\else
\ifx#1!\relax
\def\next{\raw@coor}%
\else
\def\next{\special@@@coor#1}%
\fi
\fi
\fi
\next}
\def\special@@@coor#1;#2;#3\@nil{%
\ifx#3;\relax
\polar@coor{#1}{#2}%
\else
\cartesian@coor#1,\relax,\@nil
\fi}
\def\mixed@coor#1#2{%
\begingroup
% DG/SR modification begin - Oct. 27, 1997 - Patch 6
%\specialcoor@ii#1;;\@nil
%\let\pst@tempa\pst@coor
%\specialcoor@ii#2;;\@nil
\special@@coor#1;;\@nil
\let\pst@tempa\pst@coor
\special@@coor#2;;\@nil
% DG/SR modification end
\xdef\pst@tempg{\pst@tempa pop \pst@coor exch pop }%
\endgroup
\let\pst@coor\pst@tempg}
\def\polar@coor#1#2{%
\pssetlength\pst@dimg{#1}%
\pst@@getangle{#2}%
\edef\pst@coor{\pst@number\pst@dimg \pst@angle \tx@PtoC}}
\def\raw@coor#1;#2\@nil{%
\edef\pst@coor{%
#1 \pst@number\psyunit mul exch \pst@number\psxunit mul exch }}
\def\node@coor#1\@nil{%
\@pstrickserr{You must load `pst-node.tex' to use node coordinates.}\@ehps
\def\pst@coor{0 0 }}
\def\Node@coor{\node@coor}
\def\special@angle#1#2)#3\@nil{%
\ifx!#1\relax
\edef\pst@angle{#2 \pst@angleunit}%
\else
\ifx(#1\relax
\pst@@getcoor{#2}%
\edef\pst@angle{\pst@coor exch \tx@Atan}%
\else
\pst@checknum{#1#2}\pst@angle
\edef\pst@angle{\pst@angle \pst@angleunit}%
\fi
\fi}
\def\Cartesian{%
\def\cartesian@coor##1,##2,##3\@nil{%
\pssetxlength\pst@dimg{##1}%
\pssetylength\pst@dimh{##2}%
\edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}}%
\@ifnextchar({\Cartesian@}{}}
\def\Cartesian@(#1,#2){%
\pssetxlength\psxunit{#1}%
\pssetylength\psyunit{#2}%
\ignorespaces}
\def\Polar{%
\def\psput@cartesian{\psput@special}%
\def\cartesian@coor##1,##2,##3\@nil{\polar@coor{##1}{##2}}}%
\def\psset@origin#1{%
\pst@@getcoor{#1}%
\edef\psk@origin{\pst@coor \tx@NET }}
\def\psk@origin{}
\newif\ifswapaxes
\def\psset@swapaxes#1{%
\@nameuse{@pst#1}%
\if@pst
\def\psk@swapaxes{-90 rotate -1 1 scale }%
\else
\def\psk@swapaxes{}%
\fi}
\psset@swapaxes{false}
\newif\ifshowpoints
\def\psset@showpoints#1{\@nameuse{showpoints#1}}
\psset@showpoints{false}
\let\pst@setrepeatarrowsflag\relax
\def\psset@border#1{%
\pst@getlength{#1}\psk@border
\pst@setrepeatarrowsflag}
\psset@border{0pt}
\def\psset@bordercolor#1{\pst@getcolor{#1}\psbordercolor}
\psset@bordercolor{white}
\newif\ifpsdoubleline
\def\psset@doubleline#1{%
\@nameuse{psdoubleline#1}%
\pst@setrepeatarrowsflag}
\psset@doubleline{false}
\def\psset@doublesep#1{\def\psdoublesep{#1}}
\psset@doublesep{1.25\pslinewidth}
\def\psset@doublecolor#1{\pst@getcolor{#1}\psdoublecolor}
\psset@doublecolor{white}
\newif\ifpsshadow
\def\psset@shadow#1{%
\@nameuse{psshadow#1}%
\pst@setrepeatarrowsflag}
\psset@shadow{false}
\def\psset@shadowsize#1{\pst@getlength{#1}\psk@shadowsize}
\psset@shadowsize{3pt}
\def\psset@shadowangle#1{\pst@getangle{#1}\psk@shadowangle}
\psset@shadowangle{-45}
\def\psset@shadowcolor#1{\pst@getcolor{#1}\psshadowcolor}
\psset@shadowcolor{darkgray}
\def\pst@repeatarrowsflag{\z@}
\def\pst@setrepeatarrowsflag{%
\edef\pst@repeatarrowsflag{%
\ifdim\psk@border\p@>\z@ 1\else\ifpsdoubleline 1\else
\ifpsshadow 1\else \z@\fi\fi\fi}}
\def\psls@none{}
\newdimen\pslinewidth
\def\psset@linewidth#1{\pssetlength\pslinewidth{#1}}
\psset@linewidth{.8pt}
\def\psset@linecolor#1{\pst@getcolor{#1}\pslinecolor}
\psset@linecolor{black}
\def\psls@solid{0 setlinecap stroke }
\def\pst@missing{%
\z@
\@pstrickserr{Missing number or dimension. 0 substituted}\@ehpa}
\def\psset@dash#1{%
\pst@expandafter\psset@@dash{#1} {\pst@missing} {\pst@missing} {}\@nil
\edef\psk@dash{\pst@number\pst@dimg \pst@number\pst@dimh}}
\def\psset@@dash#1 #2 #3\@nil{%
\pssetlength\pst@dimg{#1}%
\pssetlength\pst@dimh{#2}}
\psset@dash{5pt 3pt}
\newif\ifpsdashadjust
\def\psset@dashadjust#1{\@nameuse{psdashadjust#1}}
\psset@dashadjust{true}
\def\psls@dashed{%
\ifpsdashadjust
\psk@dash \pst@linetype\space \tx@DashLine
\else
[ \psk@dash ] 0 setdash stroke
\fi}
\def\tx@DashLine{DashLine }
\def\psset@dotsep#1{\pst@getlength{#1}\psk@dotsep}
\psset@dotsep{3pt}
\def\psls@dotted{%
\ifpsdashadjust
\psk@dotsep \pst@linetype\space \tx@DotLine
\else
[ 0 \psk@dotsep CLW add ] 0 setdash 1 setlinecap stroke
\fi}
\def\tx@DotLine{DotLine }
\def\psset@linestyle#1{%
\@ifundefined{psls@#1}%
{\@pstrickserr{Line style `#1' not defined}\@eha}%
{\edef\pslinestyle{#1}}}
\psset@linestyle{solid}
\def\psfs@none{}
\def\psset@fillcolor#1{\pst@getcolor{#1}\psfillcolor}
\psset@fillcolor{white}
\def\psfs@solid{\pst@fill{\pst@usecolor\psfillcolor fill}}
\def\psset@hatchwidth#1{\pst@getlength{#1}\psk@hatchwidth}
\psset@hatchwidth{.8pt}
\def\psset@hatchsep#1{\pst@getlength{#1}\psk@hatchsep}
\psset@hatchsep{4pt}
\def\psset@hatchcolor#1{\pst@getcolor{#1}\pshatchcolor}
\psset@hatchcolor{black}
\def\psset@hatchangle#1{\pst@getangle{#1}\psk@hatchangle}
\psset@hatchangle{45}
\def\pst@linefill{%
\psk@hatchangle rotate
\psk@hatchwidth SLW
\pst@usecolor\pshatchcolor
\psk@hatchsep \tx@LineFill}
\def\psfs@vlines{\pst@fill\pst@linefill}
\@namedef{psfs@vlines*}{\psfs@solid \psfs@vlines}
\def\psfs@hlines{\pst@fill{90 rotate \pst@linefill}}
\@namedef{psfs@hlines*}{\psfs@solid \psfs@hlines}
\def\psfs@crosshatch{\psfs@vlines \psfs@hlines}
\@namedef{psfs@crosshatch*}{\psfs@solid \psfs@vlines \psfs@hlines}
\def\tx@LineFill{LineFill }
\def\psset@fillstyle#1{%
\edef\pst@tempg{#1}\def\pst@temph{none}%
\ifx\pst@tempg\pst@temph
\let\psk@fillstyle\relax
\else
\@ifundefined{psfs@#1}%
{\@pstrickserr{Undefined fill style: `#1'}\@eha}%
{\edef\psk@fillstyle{\expandafter\noexpand\csname psfs@#1\endcsname}}%
\fi}
\def\psset@addfillstyle#1{%
\@ifundefined{psfs@#1}%
{\@pstrickserr{Undefined fill style: `#1'}\@eha}%
{\edef\psk@fillstyle{%
\expandafter\noexpand\psk@fillstyle
\expandafter\noexpand\csname psfs@#1\endcsname}}}
\psset@fillstyle{none}
\def\psset@arrows#1{%
\begingroup
\pst@activearrows
\xdef\pst@tempg{#1}%
\endgroup
\expandafter\psset@@arrows\pst@tempg\@empty-\@empty\@nil
\if@pst\else
\@pstrickserr{Bad arrows specification: #1}\@ehpa
\fi}
\def\psset@@arrows#1-#2\@empty#3\@nil{%
\@psttrue
\def\next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
\expandafter\next\pst@arrowtable,#1-#1,\@nil
\@ifundefined{psas@\pst@tempg}%
{\@pstfalse\def\psk@arrowA{}}%
{\let\psk@arrowA\pst@tempg}%
\@ifundefined{psas@#2}%
{\@pstfalse\def\psk@arrowB{}}%
{\def\psk@arrowB{#2}}}
\def\psk@arrowA{}
\def\psk@arrowB{}
\def\pst@arrowtable{,<->,<<->>,>-<,>>-<<,(-),[-]}
\begingroup
\catcode`\<=13
\catcode`\>=13
\catcode`\|=13
\gdef\pst@activearrows{\def<{\string<}\def>{\string>}\def|{\string|}}
\endgroup
\def\tx@BeginArrow{BeginArrow }
\def\tx@EndArrow{EndArrow }
\def\psset@arrowscale#1{\pst@getscale{#1}\psk@arrowscale}
\psset@arrowscale{1}
\def\psset@arrowsize#1{%
\pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
\edef\psk@arrowsize{\pst@number\pst@dimg \pst@tempg}}
\psset@arrowsize{1.5pt 2}
\def\psset@arrowlength#1{\pst@checknum{#1}\psk@arrowlength}
\psset@arrowlength{1.4}
\def\psset@arrowinset#1{\pst@checknum{#1}\psk@arrowinset}%
\psset@arrowinset{.4}
\def\tx@Arrow{Arrow }
\@namedef{psas@>}{%
false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\@namedef{psas@>>}{%
false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
0 h T
gsave
newpath
false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
CP
grestore
CP newpath moveto
2 copy
L
stroke
moveto}
\@namedef{psas@<}{%
true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\@namedef{psas@<<}{%
true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
CP newpath moveto 0 a neg L stroke 0 h neg T
false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\def\psset@tbarsize#1{%
\pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
\edef\psk@tbarsize{\pst@number\pst@dimg \pst@tempg}}
\psset@tbarsize{2pt 5}
\def\tx@Tbar{Tbar }
\@namedef{psas@|}{\psk@tbarsize \tx@Tbar}
\@namedef{psas@|*}{0 CLW -2 div T \psk@tbarsize \tx@Tbar}
\@namedef{psas@>|}{%
\psk@tbarsize \tx@Tbar
0 CLW 2 div T
newpath
false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\@namedef{psas@>|*}{%
0 CLW -2 div T
\psk@tbarsize \tx@Tbar
0 CLW 2 div T
newpath
false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\edef\pst@arrowtable{\pst@arrowtable,|<*->|*,|<->|}
\def\psset@bracketlength#1{\pst@checknum{#1}\psk@bracketlength}
\psset@bracketlength{.15}
\def\tx@Bracket{Bracket }
\@namedef{psas@]}{\psk@bracketlength \psk@tbarsize \tx@Bracket}
\def\psset@rbracketlength#1{\pst@checknum{#1}\psk@rbracketlength}
\psset@rbracketlength{.15}
\def\tx@RoundBracket{RoundBracket }
\@namedef{psas@)}{\psk@rbracketlength \psk@tbarsize \tx@RoundBracket}
\def\psas@c{1 \psas@@c}
\def\psas@cc{0 CLW 2 div T 1 \psas@@c}
\def\psas@C{2 \psas@@c}
\def\psas@@c{%
setlinecap
0 0 moveto
0 CLW 2 div L
stroke
0 0 moveto}
\def\psas@{}
\psset@arrows{-}
\def\tx@SD{SD }
\def\tx@EndDot{EndDot }
\def\psas@oo{{\pst@usecolor\psfillcolor true} true \psk@dotsize \tx@EndDot}
\def\psas@o{{\pst@usecolor\psfillcolor true} false \psk@dotsize \tx@EndDot}
\@namedef{psas@**}{{false} true \psk@dotsize \tx@EndDot}
\@namedef{psas@*}{{false} false \psk@dotsize \tx@EndDot}
\def\pst@par{}
\def\addto@par#1{%
\ifx\pst@par\@empty
\def\pst@par{#1}%
\else
\expandafter\def\expandafter\pst@par\expandafter{\pst@par,#1}%
\fi}
\def\addbefore@par#1{%
\ifx\pst@par\@empty
\def\pst@par{#1}%
\else
\toks@{#1}%
\pst@toks\expandafter{\pst@par}%
\edef\pst@par{\the\toks@,\the\pst@toks}%
\fi}
\def\use@par{%
\ifx\pst@par\@empty\else
\expandafter\@psset\pst@par,\@nil
\def\pst@par{}%
\fi}
\def\pst@object#1{%
\pst@ifstar{%
\@ifnextchar[%
{\pst@@object{#1}}%
{\def\pst@par{}\@nameuse{#1@i}}}}
\def\pst@@object#1[#2]{%
\def\pst@par{#2}%
\@ifnextchar+{\@nameuse{#1@i}}{\@nameuse{#1@i}}}
\def\newpsobject#1#2#3{%
\@ifundefined{#2@i}%
{\@pstrickserr{Graphics object `#2' not defined}\@eha}{%
\@namedef{#1}{\pst@object{#1}}%
\@namedef{#1@i}{\addbefore@par{#3}\@nameuse{#2@i}}}%
\ignorespaces}
\def\pst@getarrows#1{\@ifnextchar({#1}{\pst@@getarrows{#1}}}
\def\pst@@getarrows#1#2{\addto@par{arrows=#2}#1}
\def\begin@ClosedObj{%
\leavevmode
\pst@killglue
\begingroup
\use@par
\solid@star
\ifpsdoubleline \pst@setdoublesep \fi
\init@pscode}
\def\end@ClosedObj{%
\ifpsshadow \pst@closedshadow \fi
\ifdim\psk@border\p@>\z@ \pst@addborder \fi
\psk@fillstyle
\pst@stroke
\ifpsdoubleline \pst@doublestroke \fi
\ifshowpoints
% DG modification begin - Mar. 4, 1995
%\addto@pscode{Points aload length 2 div cvi /N ED \psdots@iii}%
\pst@OpenShowPoints
% DG modification end
\fi
\use@pscode
\endgroup
\ignorespaces}
\def\begin@OpenObj{%
\begin@ClosedObj
\let\pst@linetype\pst@arrowtype
\pst@addarrowdef}
\def\begin@AltOpenObj{%
\begin@ClosedObj
\def\pst@repeatarrowsflag{\z@}%
\def\pst@linetype{0}}
\def\end@OpenObj{%
\ifpsshadow \pst@openshadow \fi
\ifdim\psk@border\p@>\z@ \pst@addborder \fi
\psk@fillstyle
\pst@stroke
\ifpsdoubleline \pst@doublestroke \fi
\ifnum\pst@repeatarrowsflag>\z@ \pst@repeatarrows \fi
\ifshowpoints \pst@OpenShowPoints \fi
\use@pscode
\endgroup
\ignorespaces}
\def\begin@SpecialObj{%
\leavevmode
\pst@killglue
\begingroup
\use@par
\init@pscode}
\def\end@SpecialObj{%
\use@pscode
\endgroup
\ignorespaces}
\def\pst@code{}%
\def\init@pscode{%
\addto@pscode{%
\pst@number\pslinewidth SLW
\pst@usecolor\pslinecolor}}
\def\addto@pscode#1{\xdef\pst@code{\pst@code#1\space}}
\def\use@pscode{%
\pstverb{%
\pst@dict
\tx@STP
\pst@newpath
\psk@origin
\psk@swapaxes
\pst@code
end}%
\gdef\pst@code{}}
\def\pst@newpath{newpath }
\def\pst@@killglue{\unskip\ifdim\lastskip>\z@\expandafter\pst@@killglue\fi}
\def\KillGlue{\let\pst@killglue\pst@@killglue}
\def\DontKillGlue{\let\pst@killglue\relax}
\DontKillGlue
\def\solid@star{%
\if@star
\pslinewidth=\z@
\psdoublelinefalse
\def\pslinestyle{none}%
\def\psk@fillstyle{\psfs@solid}%
\let\psfillcolor\pslinecolor
\fi}
\def\pst@setdoublesep{%
\pst@getlength\psdoublesep\psdoublesep
\pslinewidth=2\pslinewidth
\advance\pslinewidth\psdoublesep\p@
\let\pst@setdoublesep\relax}
\def\tx@Shadow{Shadow }
\def\pst@closedshadow{%
\addto@pscode{%
gsave
\psk@shadowsize \psk@shadowangle \tx@PtoC
\tx@Shadow
\pst@usecolor\psshadowcolor
gsave fill grestore
stroke
grestore
gsave
\pst@usecolor\psfillcolor
gsave fill grestore
stroke
grestore}}
\def\pst@openshadow{%
\addto@pscode{%
gsave
\psk@shadowsize \psk@shadowangle \tx@PtoC
\tx@Shadow
\pst@usecolor\psshadowcolor
\ifx\psk@fillstyle\relax\else
gsave fill grestore
\fi
stroke}%
\pst@repeatarrows
\addto@pscode{grestore}
\ifx\psk@fillstyle\relax\else
\addto@pscode{%
gsave
\pst@usecolor\psfillcolor
gsave fill grestore
stroke
grestore}
\fi}
\def\pst@addborder{%
\addto@pscode{%
gsave
\psk@border 2 mul
CLW add SLW
\pst@usecolor\psbordercolor
stroke
grestore}}
\def\pst@stroke{%
\ifx\pslinestyle\@none\else
\addto@pscode{%
gsave
\pst@number\pslinewidth SLW
\pst@usecolor\pslinecolor
\@nameuse{psls@\pslinestyle}
grestore}%
\fi}
\def\pst@fill#1{\addto@pscode{gsave #1 grestore}}%
\def\pst@doublestroke{%
\addto@pscode{%
gsave
\psdoublesep SLW
\pst@usecolor\psdoublecolor
stroke
grestore}}
\def\pst@arrowtype{%
\ifx\psk@arrowB\@empty 0 \else -2 \fi
\ifx\psk@arrowA\@empty 0 \else -1 \fi
add}
\def\pst@addarrowdef{%
\addto@pscode{%
/ArrowA {
\ifx\psk@arrowA\@empty
\pst@oplineto
\else
\pst@arrowdef{A}
moveto
\fi
} def
/ArrowB {
\ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi
} def}}
\def\pst@arrowdef#1{%
\ifnum\pst@repeatarrowsflag>\z@
/Arrow#1c [ 6 2 roll ] cvx def Arrow#1c
\fi
\tx@BeginArrow
\psk@arrowscale
\@nameuse{psas@\@nameuse{psk@arrow#1}}
\tx@EndArrow}
\def\pst@repeatarrows{%
\addto@pscode{%
gsave
\ifx\psk@arrowA\@empty\else
ArrowAc ArrowA pop pop
\fi
\ifx\psk@arrowB\@empty\else
ArrowBc ArrowB pop pop pop pop
\fi
grestore}}
\def\pst@OpenShowPoints{%
\addto@pscode{%
gsave
\psk@dotsize
\@nameuse{psds@\psk@dotstyle}
newpath
Points aload length 2 div 2 sub cvi /N ED
N 0 ge
{ \ifx\psk@arrowA\@empty
Dot
\else
pop pop
\fi
N { Dot } repeat
\ifx\psk@arrowB\@empty
Dot
\else
pop pop
\fi }
{ N 2 mul { pop } repeat }
ifelse
grestore}}
\def\pscustom{\pst@object{pscustom}}
\long\def\pscustom@i#1{%
\begin@SpecialObj
\solid@star
\let\pst@ifcustom\iftrue
\let\begin@ClosedObj\begin@CustomObj
\let\end@ClosedObj\endgroup
\def\begin@OpenObj{\begin@CustomObj\pst@addarrowdef}%
\let\end@OpenObj\endgroup
\let\begin@AltOpenObj\begin@CustomObj
\def\begin@SpecialObj{%
\begingroup
\pst@misplaced{special graphics object}%
\def\addto@pscode####1{}
\let\end@SpecialObj\endgroup}%
\def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
\def\psclip##1{\pst@misplaced\psclip}%
\def\pst@repeatarrowsflag{\z@}%
\let\pst@setrepeatarrowsflag\relax
\showpointsfalse
\let\showpointstrue\relax
\def\pst@linetype{\pslinetype}%
\let\psset@liftpen\psset@@liftpen
\psset@liftpen{\z@}%
\def\pst@cp{/currentpoint load stopped pop }%
\def\pst@oplineto{/lineto load stopped { moveto } if }%
\def\pst@optcp##1##2{%
\ifnum##1=\z@\def##2{/currentpoint load stopped { 0 0 } if }\fi}%
\let\caddto@pscode\addto@pscode
\def\cuse@par##1{{\use@par##1}}%
\the\pst@customdefs
\setbox\pst@hbox=\hbox{#1}%
\psk@fillstyle
\pst@stroke
\end@SpecialObj}
\def\begin@CustomObj{%
\begingroup
\use@par
\addto@pscode{%
\pst@number\pslinewidth SLW
\pst@usecolor\pslinecolor}}
\def\pst@oplineto{moveto }
\def\pst@cp{}
\def\pst@optcp#1#2{}
\def\psset@liftpen#1{}
\def\psset@@liftpen#1{%
\ifcase#1\relax
\def\psk@liftpen{\z@}%
\def\pst@cp{/currentpoint load stopped pop }%
\def\pst@oplineto{/lineto load stopped { moveto } if }%
\or
\def\psk@liftpen{1}%
\def\pst@cp{}%
\def\pst@oplineto{/lineto load stopped { moveto } if }%
\or
\def\psk@liftpen{2}%
\def\pst@cp{}%
\def\pst@oplineto{moveto }%
\fi}
\psset@liftpen{0}
\def\psk@liftpen{-1}
\def\psset@linetype#1{%
\pst@getint{#1}\pslinetype
\ifnum\pst@dimg<-3
\@pstrickserr{linetype must be greater than -3}\@ehpa
\def\pslinetype{0}%
\fi}
\psset@linetype{0}
\def\caddto@pscode#1{%
\@pstrickserr{Command can only be used in \string\pscustom}\@ehpa}
\let\cuse@par\caddto@pscode
\def\tx@MSave{%
/msavemtrx
[ tx@Dict /msavemtrx known { msavemtrx aload pop } if CM ]
def }
\def\tx@MRestore{%
tx@Dict /msavemtrx known { length 0 gt } { false } ifelse
{ /msavematrx [ msavematrx aload pop setmatrix ] def }
if }
\newtoks\pst@customdefs
\pst@customdefs{%
\def\newpath{\addto@pscode{newpath}}%
\def\moveto(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor moveto}}%
\def\closepath{\addto@pscode{closepath}}%
\def\gsave{\begingroup\addto@pscode{gsave}}%
\def\grestore{\endgroup\addto@pscode{grestore}}%
% DG/SR modification begin - May 12, 1997 - Patch 2
%\def\translate(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor moveto}}%
\def\translate(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor translate}}%
% DG/SR modification end
\def\rotate#1{\pst@@getangle{#1}\addto@pscode{\pst@angle rotate}}%
\def\scale#1{\pst@getscale{#1}\pst@tempg\addto@pscode{\pst@tempg}}%
\def\msave{\addto@pscode{\tx@MSave}}%
\def\mrestore{\addto@pscode{\tx@MRestore}}%
\def\swapaxes{\addto@pscode{-90 rotate -1 1 scale}}%
\def\stroke{\pst@object{stroke}}%
\def\fill{\pst@object{fill}}%
\def\openshadow{\pst@object{openshadow}}%
\def\closedshadow{\pst@object{closedshadow}}%
% DG/SR modification begin - Jan. 7, 1998 - Patch 8
%\def\movepath(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor tx@Shadow}}%
\def\movepath(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor \tx@Shadow}}%
% DG/SR modification end
\def\lineto{\pst@onecoor{lineto}}%
\def\rlineto{\pst@onecoor{rlineto}}%
\def\curveto{\pst@threecoor{curveto}}%
\def\rcurveto{\pst@threecoor{rcurveto}}%
\def\code#1{\addto@pscode{#1}}%
\def\coor(#1){\pst@@getcoor{#1}\addto@pscode\pst@coor\@ifnextchar({\coor}{}}%
\def\rcoor{\pst@getcoors{}{}}%
\def\dim#1{\pssetlength\pst@dimg{#1}\addto@pscode{\pst@number\pst@dimg}}%
\def\setcolor#1{%
\@ifundefined{color@#1}{}{\addto@pscode{\use@color{#1}}}}%
\def\arrows#1{{\psset@arrows{#1}\pst@addarrowdef}}%
\let\file\pst@rawfile
} % END \pst@customdefs
\def\closedshadow@i{\cuse@par\pst@closedshadow}
\def\openshadow@i{\cuse@par\pst@openshadow}
\def\stroke@i{\cuse@par\pst@stroke}%
\def\fill@i{\cuse@par\psk@fillstyle}%
\def\pst@onecoor#1(#2){%
\pst@@getcoor{#2}%
\addto@pscode{\pst@coor #1}}
\def\pst@threecoor#1(#2)#3(#4)#5(#6){%
\begingroup
\pst@getcoor{#2}\pst@tempa
\pst@getcoor{#4}\pst@tempb
\pst@getcoor{#6}\pst@tembc
\addto@pscode{\pst@tempa \pst@tempb \pst@tempc #1}%
\endgroup}
\def\pst@rawfile#1{%
\begingroup
\def\do##1{\catcode`##1=12\relax}"
\dospecials
\catcode`\%=14
\pst@@rawfile{#1}%
\endgroup}
\def\pst@@rawfile#1{%
\immediate\openin1 #1
\ifeof1
\@pstrickserr{File `#1' not found}\@ehpa
\else
\immediate\read1 to \pst@tempg
\loop
\ifeof1 \@pstfalse\else\@psttrue\fi
\if@pst
\addto@pscode\pst@tempg
\immediate\read1 to \pst@tempg
\repeat
\fi
\immediate\closein1\relax}
\def\tx@NArray{NArray }
\def\tx@NArray{NArray }
\def\tx@Line{Line }
\def\tx@Arcto{Arcto }
\def\tx@CheckClosed{CheckClosed }
\def\tx@Polygon{Polygon }
\def\psset@gangle#1{\pst@getangle{#1}\psk@gangle}
\psset@gangle{0}
\def\tx@Diamond{Diamond }
\def\psdiamond{\pst@object{psdiamond}}
\def\psdiamond@i(#1){%
\@ifnextchar({\psdiamond@ii(#1)}{\psdiamond@ii(0,0)(#1)}}
\def\psdiamond@ii(#1)(#2){%
\begin@ClosedObj
\pst@getcoor{#1}\pst@tempa
\pst@getcoor{#2}\pst@tempb
\addto@pscode{%
\psline@iii
pop
\psk@dimen
\pst@tempb
\psk@gangle
\pst@tempa
\tx@Diamond}%
\def\pst@linetype{4}%
\end@ClosedObj}
\def\tx@Triangle{Triangle }
\def\pstriangle{\pst@object{pstriangle}}
\def\pstriangle@i(#1){%
\@ifnextchar({\pstriangle@ii(#1)}{\pstriangle@ii(0,0)(#1)}}
\def\pstriangle@ii(#1)(#2){%
\begin@ClosedObj
\pst@getcoor{#1}\pst@tempa
\pst@getcoor{#2}\pst@tempb
\addto@pscode{%
\psline@iii
pop
\psk@dimen
\pst@tempb
\psk@gangle
\pst@tempa
\tx@Triangle}%
\def\pst@linetype{2}%
\end@ClosedObj}
\def\tx@CCA{CCA }
\def\tx@CCA{CCA }
\def\tx@CC{CC }
\def\tx@IC{IC }
\def\tx@BOC{BOC }
\def\tx@NC{NC }
\def\tx@EOC{EOC }
\def\tx@BAC{BAC }
\def\tx@NAC{NAC }
\def\tx@EAC{EAC }
\def\tx@OpenCurve{OpenCurve }
\def\tx@AltCurve{AltCurve }
\def\tx@ClosedCurve{ClosedCurve }
\def\psset@curvature#1{%
\edef\pst@tempg{#1 }%
\expandafter\psset@@curvature\pst@tempg * * * \@nil}
\def\psset@@curvature#1 #2 #3 #4\@nil{%
\pst@checknum{#1}\pst@tempg
\pst@checknum{#2}\pst@temph
\pst@checknum{#3}\pst@tempi
\edef\psk@curvature{\pst@tempg \pst@temph \pst@tempi}}
\psset@curvature{1 .1 0}
\def\pscurve{\pst@object{pscurve}}
\def\pscurve@i{%
\pst@getarrows{%
\begin@OpenObj
\pst@getcoors[\pscurve@ii}}
\def\pscurve@ii{%
\addto@pscode{%
\pst@cp
\psk@curvature\space /c ED /b ED /a ED
\ifshowpoints true \else false \fi
\tx@OpenCurve}%
\end@OpenObj}
\def\psecurve{\pst@object{psecurve}}
\def\psecurve@i{%
\pst@getarrows{%
\begin@OpenObj
\pst@getcoors[\psecurve@ii}}
\def\psecurve@ii{%
\addto@pscode{%
\psk@curvature\space /c ED /b ED /a ED
\ifshowpoints true \else false \fi
\tx@AltCurve}%
\end@OpenObj}
\def\psccurve{\pst@object{psccurve}}
\def\psccurve@i{%
\begin@ClosedObj
\pst@getcoors[\psccurve@ii}
\def\psccurve@ii{%
\addto@pscode{%
\psk@curvature\space /c ED /b ED /a ED
\ifshowpoints true \else false \fi
\tx@ClosedCurve}%
\def\pst@linetype{1}%
\end@ClosedObj}
\def\psset@dotsize#1{%
\pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
\edef\psk@@dotsize{\pst@number\pst@dimg}%
\let\psk@@@dotsize\pst@tempg
\edef\psk@dotsize{%
/DS \psk@@dotsize \psk@@@dotsize CLW mul add 2 div def }}
\psset@dotsize{2pt 2}
\def\psset@dotscale#1{%
\pst@getscale{#1}\psk@dotscale
\ifx\psk@dotscale\@empty
\def\psk@xdotscale{1 }%
\def\psk@ydotscale{1 }%
\else
\let\psk@xdotscale\pst@tempg
\let\psk@ydotscale\pst@temph
% DG/SR modification begin - Oct. 17, 1997 - Patch 5
%\fi}
\fi
\pst@getdotsize%
\psset@dotsize{\pst@dimg\space\pst@@dimtonum\pst@dimh}}
%\psset@dotscale{1}
% DG/SR modification end
\def\pst@Getangle#1#2{%
\pst@getangle{#1}\pst@tempg
\def\pst@temph{0. }%
\ifx\pst@tempg\pst@temph
\def#2{}%
\else
\edef#2{\pst@tempg\space rotate }%
\fi}
\def\psset@dotangle#1{%
\pst@getangle{#1}\psk@@dotangle
\ifdim\psk@@dotangle\p@=\z@
\let\psk@dotangle\@empty
\else
% DG/SR modification begin - Aug. 8, 1997 - Patch 4
%\edef\psk@dotangle{\psk@@dotangle rotate }
\edef\psk@dotangle{\psk@@dotangle rotate }%
% DG/SR modification end
\fi}
\psset@dotangle{0}
\def\pst@getdotsize{%
\pst@dimg=\psk@@@dotsize\pslinewidth
\advance\pst@dimg\psk@@dotsize\p@
\pst@dimh=\psk@ydotscale\pst@dimg
\pst@dimg=\psk@xdotscale\pst@dimg
\divide\pst@dimh 2
\divide\pst@dimg 2\relax}
% DG/SR modification begin - Oct. 17, 1997 - Patch 5
\psset@dotscale{1}
% DG/SR modification end
\def\psdot{\pst@object{psdot}}
\def\psdot@i{\@ifnextchar({\psdot@ii}{\psdot@ii(\z@,\z@)}}
\def\psdot@ii(#1){%
\begin@SpecialObj
\pst@@getcoor{#1}%
\addto@pscode{%
\psk@dotsize
\@nameuse{psds@\psk@dotstyle}%
\pst@coor Dot}%
\end@SpecialObj}
\def\psdots{\pst@object{psdots}}
\def\psdots@i{%
\begin@SpecialObj
\pst@getcoors[\psdots@ii}
\def\psdots@ii{%
\addto@pscode{false \tx@NArray \psdots@iii}%
\end@SpecialObj}
\def\psdots@iii{%
\psk@dotsize
\@nameuse{psds@\psk@dotstyle}
newpath
n { transform floor .5 add exch floor .5 add exch itransform Dot } repeat}
% DG: dead code (to suppress until \psset@dotstyle) ? - Aug. 4, 1997
\def\tx@SQ{SQ }
\def\tx@ST{ST }
\def\tx@SP{SP }
\def\pst@gdot#1{/Dot { gsave T \psk@dotangle \psk@dotscale #1 grestore } def }
\@namedef{psds@*}{\pst@gdot{0 0 DS \tx@SD}}
\@namedef{psds@o}{%
/r2 DS CLW sub def
\pst@gdot{0 0 DS \tx@SD \pst@usecolor\psfillcolor 0 0 r2 \tx@SD}}
\@namedef{psds@square*}{%
/r1 DS .886 mul def
\pst@gdot{r1 \tx@SQ}}
\@namedef{psds@square}{%
/r1 DS .886 mul def /r2 r1 CLW sub def
\pst@gdot{r1 \tx@SQ \pst@usecolor\psfillcolor r2 \tx@SQ}}
\@namedef{psds@triangle*}{%
/y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
\pst@gdot{x1 y1 \tx@ST}}
\@namedef{psds@triangle}{%
/y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
/y2 y1 CLW add def /x2 y2 1.732 mul neg def
\pst@gdot{x1 y1 \tx@ST \pst@usecolor\psfillcolor x2 y2 \tx@ST}}
\@namedef{psds@pentagon*}{%
/r1 DS 1.149 mul def
\pst@gdot{r1 \tx@SP}}
\@namedef{psds@pentagon}{%
DS .93 mul dup 1.236 mul /r1 ED CLW sub 1.236 mul /r2 ED
\pst@gdot{r1 \tx@SP \pst@usecolor\psfillcolor r2 \tx@SP}}
\@namedef{psds@+}{%
/DS DS 1.253 mul def
\pst@gdot{DS 0 moveto DS neg 0 L stroke 0 DS moveto 0 DS neg L stroke}}
\@namedef{psds@|}{%
\psk@tbarsize CLW mul add 2 div /DS ED
\pst@gdot{0 DS moveto 0 DS neg L stroke}}
% DG: end dead code?
\def\psset@dotstyle#1{%
\@ifundefined{psds@#1}%
{\@pstrickserr{Dot style `#1' not defined}\@eha}%
{\edef\psk@dotstyle{#1}}}
\psset@dotstyle{*}
\def\tx@FontDot{FontDot }
\def\newpsfontdot#1[#2]#3#4{%
\@namedef{psds@#1}{%
/#3 \psk@@dotangle [#2] \tx@FontDot
/Dot { moveto #4 show } bind def }}
\def\newpsfontdotH#1[#2]#3#4#5{%
\@namedef{psds@#1}{%
/#3 \psk@@dotangle [#2] \tx@FontDot
/Dot {
moveto
\iftrue
gsave \pst@usecolor\psfillcolor #5 show grestore
\fi
#4 show
} bind def }}
\pstheader{pst-dots.pro}
\newpsfontdot{*}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(b)}
\newpsfontdotH{o}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(c)}{(b)}
\newpsfontdotH{Bo}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(C)}{(b)}
\newpsfontdotH{triangle}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(t)}{(u)}
\newpsfontdotH{Btriangle}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(T)}{(u)}
\newpsfontdot{triangle*}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{square}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(s)}{(r)}
\newpsfontdotH{Bsquare}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(S)}{(r)}
\newpsfontdot{square*}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(r)}
\newpsfontdotH{pentagon}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(p)}{(q)}
\newpsfontdotH{Bpentagon}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(P)}{(q)}
\newpsfontdot{pentagon*}%
[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(q)}
% DG/SR modification begin - Mar. 18, 1997
%\newpsfontdot{diamond*}%
%[1.9 0.0 0.0 1.9 -0.4598 -0.70775]{Symbol}{<E0>}
%\newpsfontdot{diamond}%
%[2.3 0.0 0.0 2.3 -0.8533 -0.5336]{Symbol}{<A8>}
\newpsfontdot{diamond}%
[1.9 0.0 0.0 1.9 -0.4598 -0.70775]{Symbol}{<E0>}
\newpsfontdot{diamond*}%
[2.3 0.0 0.0 2.3 -0.8533 -0.5336]{Symbol}{<A8>}
% DG/SR modification end
\newpsfontdot{oplus}%
[1.44928 0.0 0.0 1.44928 -0.562319 -0.478261]{Symbol}{<C5>}
\newpsfontdot{otimes}%
[1.44928 0.0 0.0 1.44928 -0.562319 -0.475362]{Symbol}{<C4>}
\newpsfontdot{x}%
[1.8 0.0 0.0 1.8 -0.495 -0.4788]{Symbol}{<B4>}
\newpsfontdot{+}%
[2.3 0.0 0.0 2.3 -0.6486 -0.5819]{Times-Roman}{<2B>}
\newpsfontdot{asterisk}%
[2.43309 0.0 0.0 2.43309 -0.609489 -1.14477]{Times-Roman}{<2A>}
\newpsfontdot{B+}%
[2.3 0.0 0.0 2.3 -0.6555 -0.5819]{Times-Bold}{<2B>}
\newpsfontdot{Basterisk}%
[2.29358 0.0 0.0 2.29358 -0.576835 -1.08486]{Times-Bold}{<2A>}
\newpsfontdot{|}%
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.258929 -0.712302]{Helvetica}{(|)}
[1.98413 0.0 0.0 1.38 -0.258929 -0.5]{Helvetica}{(|)}
% DG/SR modification end
\newpsfontdot{B|}%
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.277778 -0.78302]{Helvetica-Bold}{(|)}
[1.98413 0.0 0.0 1.38 -0.277778 -0.5]{Helvetica-Bold}{(|)}
% DG/SR modification end
\iffalse
\newpsfontdot{*}%
[2.77778 0.0 0.0 2.77778 -0.638889 -0.813889]{Symbol}{<B7>}
\newpsfontdot{o}%
[3.33333 0.0 0.0 3.33333 -0.666667 -1.78167]{Symbol}{<B0>}
\newpsfontdot{Bo}%
[4.69484 0.0 0.0 4.69484 -0.78169 -2.97418]{Times-Bold}{<CA>}
\fi
\newdimen\pslinearc
\def\psset@linearc#1{\pssetlength\pslinearc{#1}}
\psset@linearc{0pt}
\def\psline{\pst@object{psline}}
\def\psline@i{%
\pst@getarrows{%
\begin@OpenObj
\pst@getcoors[\psline@ii}}
\def\psline@ii{%
\addto@pscode{\pst@cp \psline@iii \tx@Line}%
\end@OpenObj}
\def\psline@iii{%
\ifdim\pslinearc>\z@
/r \pst@number\pslinearc def
/Lineto { \tx@Arcto } def
\else
/Lineto /lineto load def
\fi
\ifshowpoints true \else false \fi}
\def\qline(#1)(#2){%
\def\pst@par{}%
\begin@SpecialObj
\def\pst@linetype{0}%
\pst@getcoor{#1}\pst@tempa
\pst@@getcoor{#2}%
\addto@pscode{%
\pst@tempa moveto \pst@coor L
\@nameuse{psls@\pslinestyle}}%
\end@SpecialObj}
\def\pspolygon{\pst@object{pspolygon}}
\def\pspolygon@i{%
\begin@ClosedObj
\def\pst@cp{}%
\pst@getcoors[\pspolygon@ii}
\def\pspolygon@ii{%
\addto@pscode{\psline@iii \tx@Polygon}%
\def\pst@linetype{1}%
\end@ClosedObj}
\def\psset@framearc#1{\pst@checknum{#1}\psk@framearc}
\psset@framearc{0}
\def\psset@cornersize#1{%
\pst@expandafter\psset@@cornersize{#1}\@nil}
\def\psset@@cornersize#1#2\@nil{%
\if #1a\relax
\def\psk@cornersize{\pst@number\pslinearc false }%
\else
\def\psk@cornersize{\psk@framearc true }%
\fi}
\psset@cornersize{relative}
\def\tx@Rect{Rect }
\def\tx@OvalFrame{OvalFrame }
\def\tx@Frame{Frame }
\def\psset@dimen#1{%
\pst@expandafter\psset@@dimen{#1}\@nil}
\def\psset@@dimen#1#2\@nil{%
\if #1o\relax
\def\psk@dimen{.5 }%
\else
\if #1m\relax
\def\psk@dimen{0 }%
\else
\if #1i\relax
\def\psk@dimen{-.5 }%
\fi
\fi
\fi}
\psset@dimen{outer}
\def\psframe{\pst@object{psframe}}
\def\psframe@i(#1){%
\@ifnextchar({\psframe@ii(#1)}{\psframe@ii(0,0)(#1)}}
\def\psframe@ii(#1)(#2){%
\begin@ClosedObj
\pst@getcoor{#1}\pst@tempa
\pst@@getcoor{#2}%
\addto@pscode{\psk@cornersize \pst@tempa \pst@coor \psk@dimen \tx@Frame}%
\def\pst@linetype{2}%
\showpointsfalse
\end@ClosedObj}
\def\tx@BezierNArray{BezierNArray }
\def\tx@OpenBezier{OpenBezier }
\def\tx@ClosedBezier{ClosedBezier }
\def\tx@BezierShowPoints{BezierShowPoints }
\def\psbezier{\pst@object{psbezier}}
\def\psbezier@i{%
\pst@getarrows{%
\begin@OpenObj
\pst@getcoors[\psbezier@ii}}
\def\psbezier@ii{%
\addto@pscode{%
% DG/SR modification begin - Apr. 28, 1997 - Patch 1
% \psbezier doesn't work inside \pscustom
%\pst@cp
% DG/SR modification end
\ifshowpoints true \else false \fi
\tx@OpenBezier
\ifshowpoints \tx@BezierShowPoints \fi}%
\end@OpenObj}
\def\pscbezier{\pst@object{pscbezier}}
\def\pscbezier@i{%
\begin@ClosedObj
\pst@getcoors[\pscbezier@ii}
\def\pscbezier@ii{%
\addto@pscode{%
\ifshowpoints true \else false \fi
\tx@ClosedBezier
\ifshowpoints \tx@BezierShowPoints \fi}%
\chardef\pst@linetype=1
\end@ClosedObj}
\def\tx@Parab{Parab }
\def\parabola{\pst@object{parabola}}
\def\parabola@i{\pst@getarrows\parabola@ii}
\def\parabola@ii#1(#2)#3(#4){%
\begin@OpenObj
\pst@getcoor{#2}\pst@tempa
\pst@@getcoor{#4}%
\addto@pscode{\pst@tempa \pst@coor \tx@Parab}%
\end@OpenObj}
\def\psset@gridwidth#1{\pst@getlength{#1}\psk@gridwidth}
\psset@gridwidth{.8pt}
\def\psset@griddots#1{%
\pst@cntg=#1\relax
\edef\psk@griddots{\the\pst@cntg}}
\psset@griddots{0}
\def\psset@gridcolor#1{\pst@getcolor{#1}\psgridcolor}
\psset@gridcolor{black}
\def\psset@subgridwidth#1{\pst@getlength{#1}\psk@subgridwidth}
\psset@subgridwidth{.4pt}
\def\psset@subgridcolor#1{\pst@getcolor{#1}\pssubgridcolor}
\psset@subgridcolor{gray}
\def\psset@subgriddots#1{%
\pst@cntg=#1\relax\edef\psk@subgriddots{\the\pst@cntg}}
\psset@subgriddots{0}
\def\psset@subgriddiv#1{%
\pst@cntg=#1\relax\edef\psk@subgriddiv{\the\pst@cntg}}
\psset@subgriddiv{5}
\def\psset@gridlabels#1{\pst@getlength{#1}\psk@gridlabels}
\psset@gridlabels{10pt}
\def\psset@gridlabelcolor#1{\pst@getcolor{#1}\psgridlabelcolor}
\psset@gridlabelcolor{black}
\def\tx@Grid{Grid }
\def\psgrid{\pst@object{psgrid}}
\def\psgrid@i{\@ifnextchar(%
{\psgrid@ii}{\expandafter\psgrid@iv\pic@coor}}
\def\psgrid@ii(#1){\@ifnextchar(%
{\psgrid@iii(#1)}{\psgrid@iv(0,0)(0,0)(#1)}}
\def\psgrid@iii(#1)(#2){\@ifnextchar(%
{\psgrid@iv(#1)(#2)}{\psgrid@iv(#1)(#1)(#2)}}
\def\psgrid@iv(#1)(#2)(#3){%
\begin@SpecialObj
\pst@getcoor{#1}\pst@tempa
\pst@getcoor{#2}\pst@tempb
\pst@@getcoor{#3}%
\ifnum\psk@subgriddiv>1
\addto@pscode{gsave
\psk@subgridwidth SLW \pst@usecolor\pssubgridcolor
\pst@tempb \pst@coor \pst@tempa
\pst@number\psxunit \pst@number\psyunit
\psk@subgriddiv\space \psk@subgriddots\space
{} 0 \tx@Grid grestore}%
\fi
\addto@pscode{gsave
\psk@gridwidth SLW \pst@usecolor\psgridcolor
\pst@tempb \pst@coor \pst@tempa
\pst@number\psxunit \pst@number\psyunit
1 \psk@griddots\space { \pst@usecolor\psgridlabelcolor }
\psk@gridlabels \tx@Grid grestore}%
\end@SpecialObj}
\newif\ifpsmathbox
\psmathboxtrue
\def\pst@mathflag{\z@}
\newtoks\everypsbox
\let\pst@thisbox\relax
\long\def\pst@makenotverbbox#1#2{%
\edef\pst@mathflag{%
\ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi}%
\setbox\pst@hbox=\hbox{%
\ifcase\pst@mathflag\or$\m@th\textstyle\or$\m@th\displaystyle\fi
{\pst@thisbox\the\everypsbox#2}%
\ifnum\pst@mathflag>\z@$\fi}%
#1}
\def\pst@makeverbbox#1{%
\def\pst@afterbox{#1}%
\edef\pst@mathflag{%
\ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi}%
\afterassignment\pst@beginbox
\setbox\pst@hbox\hbox}
\def\pst@beginbox{%
\ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi
\bgroup\aftergroup\pst@endbox
\pst@thisbox
\the\everypsbox}
\def\pst@endbox{%
\ifnum\pst@mathflag>\z@$\fi
\egroup
\pst@afterbox}
\def\pst@makebox{\pst@@makebox}
\def\psverbboxtrue{\def\pst@@makebox{\pst@makeverbbox}}
\def\psverbboxfalse{\def\pst@@makebox{\pst@makenotverbbox}}
\psverbboxfalse
\def\pst@longbox{%
\def\pst@makebox{%
\gdef\pst@makebox{\pst@@makebox}%
\pst@makelongbox}}
\def\pst@makelongbox#1{%
\def\pst@afterbox{#1}%
\edef\pst@mathflag{%
\ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi}%
\setbox\pst@hbox\hbox\bgroup
\aftergroup\pst@afterbox
\ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi
\begingroup
\pst@thisbox
\the\everypsbox}
\def\pst@endlongbox{%
\endgroup
\ifnum\pst@mathflag>\z@$\fi
\egroup}
\def\pslongbox#1#2{%
\@namedef{#1}{\pst@longbox#2}%
\@namedef{end#1}{\pst@endlongbox}}
\newdimen\psframesep
\def\psset@framesep#1{\pssetlength\psframesep{#1}}
\psset@framesep{3pt}
\newif\ifpsboxsep
\def\psset@boxsep#1{\@nameuse{psboxsep#1}}
\psset@boxsep{true}
\def\pst@useboxpar{%
\use@par
\if@star
\let\pslinecolor\psfillcolor
\solid@star
\let\solid@star\relax
\fi
\ifpsdoubleline \pst@setdoublesep \fi}
\def\psframebox{\pst@object{psframebox}}
\def\psframebox@i{\pst@makebox\psframebox@ii}
\def\psframebox@ii{%
\begingroup
\pst@useboxpar
\pst@dima=\pslinewidth
\advance\pst@dima by \psframesep
\pst@dimc=\wd\pst@hbox\advance\pst@dimc by \pst@dima
\pst@dimb=\dp\pst@hbox\advance\pst@dimb by \pst@dima
\pst@dimd=\ht\pst@hbox\advance\pst@dimd by \pst@dima
\setbox\pst@hbox=\hbox{%
\ifpsboxsep\kern\pst@dima\fi
\begin@ClosedObj
\addto@pscode{%
\psk@cornersize
\pst@number\pst@dima neg
\pst@number\pst@dimb neg
\pst@number\pst@dimc
\pst@number\pst@dimd
.5
\tx@Frame}%
\def\pst@linetype{2}%
\showpointsfalse
\end@ClosedObj
\box\pst@hbox
\ifpsboxsep\kern\pst@dima\fi}%
\ifpsboxsep\dp\pst@hbox=\pst@dimb\ht\pst@hbox=\pst@dimd\fi
\leavevmode\box\pst@hbox
\endgroup}
\def\psdblframebox{\pst@object{psdblframebox}}
\def\psdblframebox@i{\addto@par{doubleline=true}\psframebox@i}
\def\psclip#1{%
\leavevmode
\begingroup
\begin@psclip
\begingroup
\def\use@pscode{%
\pstVerb{%
\pst@dict
/mtrxc CM def
CP CP T
\tx@STV
\psk@origin
\psk@swapaxes
newpath
\pst@code
clip
newpath
mtrxc setmatrix
moveto
0 setgray
end}%
\gdef\pst@code{}}%
\def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
\def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
\hbox to\z@{#1}%
\endgroup
\def\endpsclip{%
\end@psclip
\endgroup}%
\ignorespaces}
\def\endpsclip{\pst@misplaced\endpsclip}
\let\begin@psclip\relax
\def\end@psclip{\pstVerb{currentpoint initclip moveto}}
\def\AltClipMode{%
\def\end@psclip{\pstVerb{\pst@grestore}}%
\def\begin@psclip{\pstVerb{gsave}}}
\def\clipbox{\@ifnextchar[{\clipbox@}{\clipbox@[\z@]}}
% DG modification begin - Apr. 3, 1997
% From paulus@immd5.informatik.uni-erlangen.de (Dietrich Paulus)
%\def\clipbox@[#1]{\pst@makebox\clipbox@@{#1}}
\def\clipbox@[#1]{\pst@makebox{\clipbox@@{#1}}}
% DG modification end
\def\clipbox@@#1{%
\pssetlength\pst@dimg{#1}%
\leavevmode\hbox{%
\begin@psclip
\pst@Verb{%
CM \tx@STV CP T newpath
/a \pst@number\pst@dimg def
/w \pst@number{\wd\pst@hbox}a add def
/d \pst@number{\dp\pst@hbox}a add neg def
/h \pst@number{\ht\pst@hbox}a add def
a neg d moveto
a neg h L
w h L
w d L
closepath
clip
newpath
0 0 moveto
setmatrix}%
\unhbox\pst@hbox
\end@psclip}}
\def\psshadowbox{\pst@object{psshadowbox}}
\def\psshadowbox@i{\pst@makebox\psshadowbox@ii}
\def\psshadowbox@ii{%
\begingroup
\pst@useboxpar
\psshadowtrue
\psboxseptrue
\def\psk@shadowangle{-45 }%
\setbox\pst@hbox=\hbox{\psframebox@ii}%
\pst@dimh=\psk@shadowsize\p@
\pst@dimh=.7071\pst@dimh
\pst@dimg=\dp\pst@hbox
\advance\pst@dimg\pst@dimh
\dp\pst@hbox=\pst@dimg
\pst@dimg=\wd\pst@hbox
\advance\pst@dimg\pst@dimh
\wd\pst@hbox=\pst@dimg
\leavevmode
\box\pst@hbox
\endgroup}
\def\pscirclebox{\pst@object{pscirclebox}}
\def\pscirclebox@i{\pst@makebox\pscirclebox@ii}
\def\pscirclebox@ii{%
\begingroup
\pst@useboxpar
\setbox\pst@hbox=\hbox{%
\pst@nodehook
\pscirclebox@iii
\box\pst@hbox}%
\ifpsboxsep \pscirclebox@sep \fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\pscirclebox@iii{%
\if@star
\pslinewidth\z@
\pstverb{\pst@dict \tx@STP \pst@usecolor\psfillcolor
newpath \pscirclebox@iv \tx@SD end}%
\else
\begin@ClosedObj
\def\pst@linetype{4}\showpointsfalse
\addto@pscode{%
\pscirclebox@iv CLW 2 div add 0 360 arc closepath}%
\end@ClosedObj
\fi}
\def\pscirclebox@iv{%
\pst@number{\wd\pst@hbox}2 div
\pst@number{\ht\pst@hbox}\pst@number{\dp\pst@hbox}add 2 div
2 copy \pst@number{\dp\pst@hbox}sub 4 2 roll
\tx@Pyth \pst@number\psframesep add }
\def\pscirclebox@sep{%
\pst@dimb=\ht\pst@hbox
\advance\pst@dimb\dp\pst@hbox
\divide\pst@dimb 2
\pst@dima=.5\wd\pst@hbox
\pst@pyth\pst@dima\pst@dimb\pst@dimc
\advance\pst@dimc\pslinewidth
\advance\pst@dimc\psframesep
\advance\pst@dimb-\pst@dimc
\setbox\pst@hbox=\hbox to2\pst@dimc{%
\hss
\vbox{\kern-\pst@dimb\box\pst@hbox}%
\hss}%
\advance\pst@dimb-\dp\pst@hbox
\dp\pst@hbox=-\pst@dimb}
\let\pst@nodehook\relax
\def\psCirclebox{\pst@object{psCirclebox}}
\def\psCirclebox@i{\pst@makebox\psCirclebox@ii}
\def\psCirclebox@ii{%
\begingroup
\pst@useboxpar
\pst@dima=\ht\pst@hbox
\advance\pst@dima\dp\pst@hbox
\divide\pst@dima\tw@
\pssetlength\pst@dimb\psk@radius
\setbox\pst@hbox=\hbox{%
\pst@nodehook
\pscircle(.5\wd\pst@hbox,\pst@dima){\pst@dimb}%
\box\pst@hbox}%
\ifpsboxsep \psCirclebox@sep \fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psCirclebox@sep{%
\pst@dimc=\pst@dimb
\advance\pst@dimb-\pst@dima
\advance\pst@dima\pst@dimc
\setbox\pst@hbox=\hbox to\tw@\pst@dimc{%
\hss
\vrule width \z@ depth \pst@dimb height \pst@dima
\box\pst@hbox
\hss}}%
\def\psovalbox{\pst@object{psovalbox}}
\def\psovalbox@i{\pst@makebox{\psovalbox@ii}}
\def\psovalbox@ii{%
\begingroup
\pst@useboxpar
\psovalbox@iii
\ifpsboxsep\psovalbox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psovalbox@iii{%
\psovalbox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
0 360
\pst@number\pst@dimc CLW 2 div sub
\pst@number\pst@dimd CLW 2 div sub
\pst@number\pst@dima
\pst@number\pst@dimb
\tx@Ellipse
closepath}%
\def\pst@linetype{2}%
\end@ClosedObj
\unhbox\pst@hbox}}
\def\psovalbox@iv{%
\pst@dimc=\pslinewidth\advance\pst@dimc\psframesep
\pst@dimd=\ht\pst@hbox\advance\pst@dimd\dp\pst@hbox
\pst@dima=.5\wd\pst@hbox
\pst@dimb=.5\pst@dimd\advance\pst@dimb-\dp\pst@hbox
\pst@dimd=.707\pst@dimd
\advance\pst@dimd\pst@dimc
\advance\pst@dimc.707\wd\pst@hbox}
\def\psovalbox@sep{%
\setbox\pst@hbox\hbox to 2\pst@dimc{\hss\unhbox\pst@hbox\hss}%
\pst@dimg=\pst@dimd
\advance\pst@dimg-\pst@dimb
\dp\pst@hbox=\pst@dimg
\advance\pst@dimd\pst@dimb
\ht\pst@hbox=\pst@dimd}
\def\psdiabox{\pst@object{psdiabox}}
\def\psdiabox@i{\pst@makebox{\psdiabox@ii}}
\def\psdiabox@ii{%
\begingroup
\pst@useboxpar
\psdiabox@iii
\ifpsboxsep\psdiabox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psdiabox@iv{%
\pst@dimg=.707\pslinewidth
\advance\pst@dimg.707\psframesep
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\pst@dimc=\pst@dima
\advance\pst@dimc\pst@dimg
\pst@dimd=\ht\pst@hbox
\advance\pst@dimd\dp\pst@hbox
\divide\pst@dimd 2
\pst@dimb=\pst@dimd
\advance\pst@dimb-\dp\pst@hbox
\advance\pst@dimd\pst@dimg}
\def\psdiabox@iii{%
\psdiabox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
\psline@iii
pop
.5
\pst@number\pst@dimc 2 mul \pst@number\pst@dimd 2 mul
0
\pst@number\pst@dima \pst@number\pst@dimb
\tx@Diamond}%
\def\pst@linetype{4}%
\end@ClosedObj
\box\pst@hbox}}
\def\psdiabox@sep{%
\setbox\pst@hbox\hbox to 4\pst@dimc{\hss\unhbox\pst@hbox\hss}%
\multiply\pst@dimd 2
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\advance\pst@dimd-2\pst@dimb
\dp\pst@hbox\pst@dimd}
\def\psset@trimode#1{\pst@expandafter\psset@@trimode{#1}\@empty\@empty\@nil}
\def\psset@@trimode#1#2#3\@nil{%
\let\pst@tempg#1\relax
\ifx\pst@tempg*%
\let\psk@@trimode\@empty
\let\pst@tempg#2\relax
\else
\let\psk@@trimode\relax
\fi
\edef\psk@trimode{%
\ifx R\pst@tempg 1 \else\ifx D\pst@tempg 2
\else\ifx L\pst@tempg 3 \else 0 \fi\fi\fi}}
\psset@trimode{U}
\def\pstribox{\pst@object{pstribox}}
\def\pstribox@i{\pst@makebox{\pstribox@ii}}
\def\pstribox@ii{%
\begingroup
\pst@useboxpar
\pstribox@iii
\ifpsboxsep\pstribox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\pstribox@iii{%
\pstribox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
\psline@iii
pop
.5
\pst@number\pst@dimc \pst@number\pst@dimd
\ifodd\psk@trimode exch \fi
\psk@trimode -90 mul
\pst@number\pst@dima \pst@number\pst@dimb
\tx@Triangle}%
\def\pst@linetype{2}%
\end@ClosedObj
\box\pst@hbox}}
\def\pstribox@iv{%
\pst@dimh=\pslinewidth
\advance\pst@dimh\psframesep
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg-\dp\pst@hbox
\divide\pst@dimg 2
\edef\pst@tempa{\number\pst@dimg sp}% For use by nodes.
\ifodd\psk@trimode
\pst@dimb\pst@dimg
\else
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\fi
\ifcase\psk@trimode
\pst@dimb=-\dp\pst@hbox
\advance\pst@dimb-\pst@dimh
\or
\pst@dima=-\pst@dimh
\or
\pst@dimb=\ht\pst@hbox
\advance\pst@dimb\pst@dimh
\or
\pst@dima=\wd\pst@hbox
\advance\pst@dima\pst@dimh
\fi
\pst@dimd=\dp\pst@hbox
\advance\pst@dimd\ht\pst@hbox
\ifx\psk@@trimode\relax
\pst@dimc=\wd\pst@hbox
\advance\pst@dimc\ifodd\psk@trimode 1.447\else 1.789\fi\pst@dimh
\multiply\pst@dimc 2
\advance\pst@dimd\ifodd\psk@trimode 1.789\else 1.447\fi\pst@dimh
\multiply\pst@dimd 2
\else
\ifodd\psk@trimode
\advance\pst@dimd 1.1547\wd\pst@hbox
\advance\pst@dimd 3.4641\pst@dimh
\pst@dimc=.866\pst@dimd
\else
\advance\pst@dimd .866\wd\pst@hbox %.866=(sqrt(3)/2)
\advance\pst@dimd 3\pst@dimh
\pst@dimc=1.1547\pst@dimd % 1.1547=(2/sqrt(3))
\fi
\fi}
\def\pstribox@sep{%
\ifodd\psk@trimode
\advance\pst@dimb.5\pst@dimd
\ht\pst@hbox=\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox=\pst@dimd
\else
\setbox\pst@hbox\hbox to \pst@dimc{\hss\unhbox\pst@hbox\hss}%
\global\pst@dimg=.5\pst@dimc
\fi
\ifcase\psk@trimode
\dp\pst@hbox-\pst@dimb
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\or
\pst@dimg=.5\wd\pst@hbox
\global\advance\pst@dimg-\pst@dima
\setbox\pst@hbox\hbox to \pst@dimc{\kern-\pst@dima\box\pst@hbox\hss}%
\or
\ht\pst@hbox\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox\pst@dimd
\or
\pst@dimg=\pst@dimc
\advance\pst@dimg-\pst@dima
\global\advance\pst@dimg.5\wd\pst@hbox
\setbox\pst@hbox\hbox to \pst@dimc{%
\hss\box\pst@hbox\kern\psframesep\kern\pslinewidth}%
\fi}
\def\psset@arcsepA#1{\pst@getlength{#1}\psk@arcsepA}
\def\psset@arcsepB#1{\pst@getlength{#1}\psk@arcsepB}
\def\psset@arcsep#1{%
\psset@arcsepA{#1}\let\psk@arcsepB\psk@arcsepA}
\psset@arcsep{0}
\def\tx@ArcArrow{ArcArrow }
\def\psarc{\pst@object{psarc}}
\def\psarc@i{%
\@ifnextchar({\psarc@iii}{\psarc@ii}}
\def\psarc@ii#1{\addto@par{arrows=#1}%
\@ifnextchar({\psarc@iii}{\psarc@iii(0,0)}}
\def\psarc@iii(#1)#2#3#4{%
\begin@OpenObj
\pst@getangle{#3}\pst@tempa
\pst@getangle{#4}\pst@tempb
\pst@@getcoor{#1}%
\pssetlength\pst@dima{#2}%
\addto@pscode{\psarc@iv \psarc@v}%
\gdef\psarc@type{0}%
\showpointsfalse
\end@OpenObj}
\def\psarc@iv{%
\pst@coor /y ED /x ED
/r \pst@number\pst@dima def
/c 57.2957 r \tx@Div def
/angleA
\pst@tempa
\psk@arcsepA c mul 2 div
\ifcase \psarc@type add \or sub \fi
def
/angleB
\pst@tempb
\psk@arcsepB c mul 2 div
\ifcase \psarc@type sub \or add \fi
def
\ifshowpoints\psarc@showpoints\fi
\ifx\psk@arrowA\@empty
\ifnum\psk@liftpen=2
r angleA \tx@PtoC
y add exch x add exch
moveto
\fi
\fi}
\def\psarc@v{%
x y r
angleA
\ifx\psk@arrowA\@empty\else
{ ArrowA CP }
{ \ifcase\psarc@type add \or sub \fi }
\tx@ArcArrow
\fi
angleB
\ifx\psk@arrowB\@empty\else
{ ArrowB }
{ \ifcase\psarc@type sub \or add \fi }
\tx@ArcArrow
\fi
\ifcase\psarc@type arc \or arcn \fi}
\def\psarc@type{0}
\def\psarc@showpoints{%
gsave
newpath
x y moveto
x y r \pst@tempa \pst@tempb
\ifcase\psarc@type arc \or arcn \fi
closepath
CLW 2 div SLW
[ \psk@dash\space ] 0 setdash stroke
grestore }
\def\psarcn{\pst@object{psarcn}}
\def\psarcn@i{\def\psarc@type{1}\psarc@i}
\def\pscircle{\pst@object{pscircle}}
\def\pscircle@i{\@ifnextchar({\pscircle@do}{\pscircle@do(0,0)}}
\def\pscircle@do(#1)#2{%
\if@star
{\use@par\qdisk(#1){#2}}%
\else
\begin@ClosedObj
\pst@@getcoor{#1}%
\pssetlength\pst@dimc{#2}%
\def\pst@linetype{4}%
\addto@pscode{%
\pst@coor
\pst@number\pst@dimc
\psk@dimen CLW mul sub
0 360 arc
closepath}%
\showpointsfalse
\end@ClosedObj
\fi
\ignorespaces}
\def\qdisk(#1)#2{%
\def\pst@par{}%
\begin@SpecialObj
\pst@@getcoor{#1}%
\pssetlength\pst@dimg{#2}%
\addto@pscode{\pst@coor \pst@number\pst@dimg \tx@SD}%
\end@SpecialObj}
\def\psset@radius#1{\pst@@getlength{#1}\psk@radius}
\psset@radius{.25cm}
\def\psCircle{\pst@object{psCircle}}
\def\psCircle@i{\@ifnextchar({\psCircle@ii}{\psCircle@ii(0,0)}}
\def\psCircle@ii(#1){\pscircle@do(#1){\psk@radius}}
\def\pswedge{\pst@object{pswedge}}
\def\pswedge@i{\@ifnextchar({\pswedge@ii}{\pswedge@ii(0,0)}}
\def\pswedge@ii(#1)#2#3#4{%
\begin@ClosedObj
\pssetlength\pst@dimc{#2}
\pst@getangle{#3}\pst@tempa
\pst@getangle{#4}\pst@tempb
\pst@@getcoor{#1}%
\def\pst@linetype{1}%
\addto@pscode{%
\pst@coor
2 copy
moveto
\pst@number\pst@dimc \psk@dimen CLW mul sub % Adjusted radius
\pst@tempa \pst@tempb
arc
closepath}%
\showpointsfalse
\end@ClosedObj}
\def\tx@Ellipse{Ellipse }
\def\psellipse{\pst@object{psellipse}}
\def\psellipse@i(#1){\@ifnextchar(%
{\psellipse@ii(#1)}{\psellipse@ii(0,0)(#1)}}
\def\psellipse@ii(#1)(#2){%
\begin@ClosedObj
\pst@getcoor{#1}\pst@tempa
\pst@@getcoor{#2}%
\addto@pscode{%
0 360
\pst@coor
\ifdim\psk@dimen\p@=\z@\else
\psk@dimen CLW mul
dup 4 -1 roll sub neg 3 1 roll sub
\fi
\pst@tempa
\tx@Ellipse
closepath}%
\def\pst@linetype{2}%
\end@ClosedObj}
\def\multips{\@ifnextchar({\def\pst@par{}\multips@ii}{\multips@i}}
\def\multips@i#1{\def\pst@par{rot=#1}\multips@ii}
\def\multips@ii(#1){\@ifnextchar({\multips@iii(#1)}{\multips@iii(\z@,\z@)(#1)}}
\long\def\multips@iii(#1)(#2)#3#4{%
\begingroup
\use@par
\pst@getcoor{#1}\pst@tempa
\pst@@getcoor{#2}%
\pst@cnta=#3\relax
\init@pscode
\addto@pscode{%
\pst@tempa T \the\pst@cnta\space \pslbrace
gsave \ifx\psk@rot\@empty\else\psk@rot rotate \fi}%
\hbox to\z@{%
\def\init@pscode{%
\addto@pscode{%
gsave
\pst@number\pslinewidth SLW
\pst@usecolor\pslinecolor}}%
\def\use@pscode{\addto@pscode{grestore}}%
\def\psclip##1{\pst@misplaced\psclip}%
\def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
#4}%
\addto@pscode{grestore \pst@coor T \psrbrace repeat}%
\leavevmode
\use@pscode
\endgroup
\ignorespaces}
\def\scalebox#1{\pst@makebox{\@scalebox{#1}}}
\def\@scalebox#1{%
\begingroup
\pst@getscale{#1}\pst@tempa
\let\pst@tempc\pst@tempg
\let\pst@tempd\pst@temph
\@@scalebox
\endgroup}
\def\@@scalebox{%
\leavevmode
\hbox{%
\ifdim\pst@tempd\p@<\z@
\pst@dimg=\pst@tempd\ht\pst@hbox
\pst@dimh=\pst@tempd\dp\pst@hbox
\dp\pst@hbox=-\pst@dimg
\ht\pst@hbox=-\pst@dimh
\else
\ht\pst@hbox=\pst@tempd\ht\pst@hbox
\dp\pst@hbox=\pst@tempd\dp\pst@hbox
\fi
\pst@dima=\pst@tempc\wd\pst@hbox
\ifdim\pst@dima<\z@\kern-\pst@dima\fi
\pst@Verb{CP CP translate \pst@tempa \tx@NET}%
\hbox to \z@{\box\pst@hbox\hss}%
\pst@Verb{%
CP CP translate
1 \pst@tempc div 1 \pst@tempd div scale
\tx@NET}%
\ifdim\pst@dima>\z@\kern\pst@dima\fi}}
\pslongbox{Scalebox}{\scalebox}
\def\scaleboxto(#1,#2){\pst@makebox{\@scaleboxto(#1,#2)}}
\def\@scaleboxto(#1,#2){%
\begingroup
\pssetlength\pst@dima{#1}%
\pssetlength\pst@dimb{#2}%
\ifdim\pst@dima=\z@\else
\pst@divide{\pst@dima}{\wd\pst@hbox}\pst@tempc
\edef\pst@tempc{\pst@tempc\space}%
\fi
\ifdim\pst@dimb=\z@
\ifdim\pst@dima=\z@
\@pstrickserr{%
\string\scaleboxto\space dimensions cannot both be zero}\@ehpa
\def\pst@tempa{}%
\def\pst@tempc{1 }%
\def\pst@tempd{1 }%
\else
\let\pst@tempd\pst@tempc
\fi
\else
\pst@dimc=\ht\pst@hbox
\advance\pst@dimc\dp\pst@hbox
\pst@divide{\pst@dimb}{\pst@dimc}\pst@tempd
\edef\pst@tempd{\pst@tempd\space}%
\ifdim\pst@dima=\z@ \let\pst@tempc\pst@tempd \fi
\fi
\edef\pst@tempa{\pst@tempc \pst@tempd scale }%
\@@scalebox
\endgroup}
\pslongbox{Scaleboxto}{\scaleboxto}
\def\tx@Rot{Rot }
\def\rotateleft{\pst@makebox{\@rotateleft\pst@hbox}}
\def\@rotateleft#1{%
\leavevmode\hbox{\hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
\pst@Verb{90 \tx@Rot}
\vbox to \z@{\vss\hbox to \z@{\box#1\hss}\vskip\z@}%
\pst@Verb{-90 \tx@Rot}}}}
\def\rotateright{\pst@makebox{\@rotateright\pst@hbox}}
\def\@rotateright#1{%
\hbox{\hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
\pst@Verb{-90 \tx@Rot}
\vbox to \z@{\hbox to \z@{\hss\box#1}\vss}%
\pst@Verb{90 \tx@Rot}}}}
\def\rotatedown{\pst@makebox{\@rotatedown\pst@hbox}}
\def\@rotatedown#1{%
\hbox{\hskip\wd#1\vbox{\vskip\ht#1\vskip\dp#1%
\pst@Verb{180 \tx@Rot}%
\vbox to \z@{\hbox to \z@{\box#1\hss}\vss}%
\pst@Verb{-180 \tx@Rot}}}}
\pslongbox{Rotateleft}{\rotateleft}
\pslongbox{Rotateright}{\rotateright}
\pslongbox{Rotatedown}{\rotatedown}
\def\pst@starbox{%
\setbox\pst@hbox\hbox{\psframebox*[boxsep=false]{\unhbox\pst@hbox}}}
\def\pst@@makesmall#1{%
\setbox#1=\hbox to\z@{\hss\vbox to \z@{\vss\box#1\vss}\hss}}
\def\pst@@@makesmall#1{%
\pst@dimh=\psk@xref\wd#1%
\ifx\psk@yref\relax
\pst@dimg=\dp#1%
\else
\pst@dimg=\psk@yref\ht#1%
\advance\pst@dimg\psk@yref\dp#1%
\fi
\setbox#1=\hbox to\z@{%
\kern-\pst@dimh\vbox to\z@{\vss\box#1\kern-\pst@dimg}\hss}}
\def\psset@ref#1{\pst@expandafter\psset@@ref{#1}\@empty,,\@nil}
\def\psset@@ref#1#2,#3,#4\@nil{%
\def\psk@xref{.5}%
\def\psk@yref{.5}%
\let\pst@makesmall\pst@@@makesmall
\ifx\@empty#3\@empty
\@nameuse{getref@#1}%
\@nameuse{getref@#2}%
\else
\pst@checknum{#1#2}\psk@xref
\pst@checknum{#3}\psk@yref
\fi}
\def\getref@c{\let\pst@makesmall\pst@@makesmall}
\def\getref@t{\def\psk@yref{1}}
\def\getref@b{\def\psk@yref{0}}
\def\getref@B{\let\psk@yref\relax}
\def\getref@l{\def\psk@xref{0}}
\def\getref@r{\def\psk@xref{1}}
\psset@ref{c}
\def\psset@rot#1{%
\pst@expandafter{\@ifnextchar*{\psset@@@rot}{\psset@@rot}}{#1}\@nil}
\def\psset@@rot#1\@nil{%
\def\next##1@#1=##2@##3\@nil{%
\ifx\relax##2%
\pst@getangle{#1}\psk@rot
\else
\def\psk@rot{##2}%
\fi}%
\expandafter\next\pst@rottable @#1=\relax @\@nil}
\def\psset@@@rot#1#2\@nil{%
\psset@@rot#2\@nil
\edef\psk@rot{\pst@rotlist \ifx\psk@rot\@empty\else\psk@rot add \fi}}
\def\pst@rotlist{mark RAngle /a ED cleartomark a neg }
\def\pst@rottable{%
@0=%
@U=%
@L=90 %
@D=180 %
@R=-90 %
@N=\pst@rotlist
@W=\pst@rotlist 90 add %
@S=\pst@rotlist 180 add %
@E=\pst@rotlist 90 sub }
\psset@rot{0}
\def\tx@RotBegin{RotBegin }
\def\tx@RotEnd{RotEnd }
\def\pst@rotate#1#2{%
\ifx#1\@empty\else
\setbox#2=\hbox{\pst@Verb{#1 \tx@RotBegin}\box#2\pst@Verb{\tx@RotEnd}}%
\fi}
\def\psput@cartesian#1{%
\hbox to \z@{\kern\pst@dimg{\vbox to \z@{\vss\box#1\vskip\pst@dimh}\hss}}}
\def\psput@special#1{%
\hbox{%
\pst@Verb{{ \pst@coor } \tx@PutCoor \tx@PutBegin}%
\box#1%
\pst@Verb{\tx@PutEnd}}}
\def\tx@PutCoor{PutCoor }
\def\tx@PutBegin{PutBegin }
\def\tx@PutEnd{PutEnd }
\def\rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\rput@i}{\rput@ii}}}
\def\rput@i[#1]{\addto@par{ref={#1}}\rput@ii}
\def\rput@ii{\@ifnextchar({\rput@iv}{\rput@iii}}
\def\rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\rput@iv}{\rput@iv(\z@,\z@)}}
\def\rput@iv(#1){\pst@killglue\pst@makebox{\rput@v{#1}}}
\def\rput@v#1{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\pst@makesmall\pst@hbox
\pst@rotate\psk@rot\pst@hbox
\psput@{#1}\pst@hbox
\endgroup
\ignorespaces}
\def\multirput{%
\def\pst@par{}%
\pst@ifstar{\@ifnextchar[{\multirput@i}{\multirput@ii}}}
\def\multirput@i[#1]{\addto@par{ref={#1}}\multirput@ii}
\def\multirput@ii{\@ifnextchar({\multirput@iv}{\multirput@iii}}
\def\multirput@iii#1{\addto@par{rot={#1}}\multirput@iv}
\def\multirput@iv(#1){%
\@ifnextchar({\multirput@v(#1)}{\multirput@v(\z@,\z@)(#1)}}
\def\multirput@v(#1,#2)(#3,#4)#5{%
\pst@makebox{\multirput@vi(#1,#2)(#3,#4){#5}}}
\def\multirput@vi(#1,#2)(#3,#4)#5{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\pst@makesmall\pst@hbox
\pst@rotate\psk@rot\pst@hbox
\pssetxlength\pst@dima{#1}%
\pssetylength\pst@dimb{#2}%
\pssetxlength\pst@dimc{#3}%
\pssetylength\pst@dimd{#4}%
\pst@cntg=#5\relax
\pst@cnth=\@ne
\leavevmode
\loop
\vbox to \z@{%
\vss
\hbox to \z@{\kern\pst@dima\copy\pst@hbox\hss}%
\vskip\pst@dimb}%
\ifnum\pst@cntg>\pst@cnth
\advance\pst@dima\pst@dimc
\advance\pst@dimb\pst@dimd
\advance\pst@cnth\@ne
\repeat
\endgroup
\ignorespaces}
\newif\if@fixedradius
\def\cput{\pst@object{cput}}
\def\cput@i{\@fixedradiusfalse\cput@ii}
\def\cput@ii{\pst@killglue\@ifnextchar({\cput@iv}{\cput@iii}}
\def\cput@iii#1{%
\addto@par{rot={#1}}%
\@ifnextchar({\cput@iv}{\cput@iv(\z@,\z@)}}
\def\cput@iv(#1){\pst@makebox{\cput@v{#1}}}
\def\cput@v#1{%
\begingroup
\use@par
\setbox\pst@hbox=\hbox{%
\psboxsepfalse
\if@fixedradius\psCirclebox@ii\else\pscirclebox@ii\fi}%
\pst@@makesmall\pst@hbox
\pst@rotate\psk@rot\pst@hbox
\psput@{#1}\pst@hbox
\endgroup
\ignorespaces}
\def\Cput{\pst@object{Cput}}
\def\Cput@i{\@fixedradiustrue\cput@ii}
\newdimen\pslabelsep
\def\psset@labelsep#1{\pssetlength\pslabelsep{#1}}
\psset@labelsep{5pt}
\def\psset@refangle#1{\pst@expandafter\psset@@refangle{#1}\@nil}
\def\psset@@refangle#1\@nil{%
\def\next##1@#1=##2"##3@##4\@nil{%
\ifx\relax##2%
\pst@getangle{#1}\psk@refangle
\def\psk@uputref{}%
\else
\def\psk@refangle{##2 }%
\def\psk@uputref{##3}%
\fi}%
\expandafter\next\pst@refangletable @#1=\relax"@\@nil}
\def\pst@refangletable{%
@r=0"20%
@u=90"02%
@l=180"10%
@d=-90"01%
@ur=45"22%
@ul=135"12%
@dr=-135"21%
@dl=-45"11}
\psset@refangle{0}
% DG/SR modification begin - Mar. 24, 1999 - Patch 10
%\def\uput{\def\pst@par{}\@ifnextchar[{\uput@ii}{\uput@i}}
\def\uput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\uput@ii}{\uput@i}}} 
% DG/SR modification end
\def\uput@i#1{\addto@par{labelsep=#1}\uput@ii}
\def\uput@ii[#1]{%
\addto@par{refangle={#1}}%
\@ifnextchar({\uput@iv}{\uput@iii}}
\def\uput@iii#1{%
\addto@par{rot={#1}}%
\@ifnextchar({\uput@iv}{\uput@iv(\z@,\z@)}}
\def\uput@iv(#1){\pst@killglue\pst@makebox{\uput@v{#1}}}
\def\uput@v#1{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\uput@vi
\psput@{#1}\pst@hbox
\endgroup
\ignorespaces}
\def\uput@vi{%
\ifx\psk@uputref\@empty
\uput@vii\tx@UUput{}%
\else
\ifx\psk@rot\@empty
\expandafter\uput@viii\psk@uputref
\else
\uput@vii\tx@UUput{}%
\fi
\fi}
\def\uput@vii#1#2{%
\edef\pst@coor{%
\pst@number\pslabelsep
#2%
\pst@number{\wd\pst@hbox}%
\pst@number{\ht\pst@hbox}%
\pst@number{\dp\pst@hbox}%
\psk@refangle\space \ifx\psk@rot\@empty\else\psk@rot\space sub \fi
\tx@Uput #1}%
\setbox\pst@hbox=\hbox to\z@{\hss\vbox to\z@{\vss\box\pst@hbox\vss}\hss}%
\setbox\pst@hbox=\psput@special\pst@hbox
\ifx\psk@rot\@empty\else\pst@rotate\psk@rot\pst@hbox\fi}
\def\uput@viii#1#2{%
\ifnum#1>\z@\ifnum#2>\z@\pslabelsep=.707\pslabelsep\fi\fi
\setbox\pst@hbox=\vbox to\z@{%
\ifnum#2=1 \vskip\pslabelsep\else\vss\fi
\hbox to\z@{%
\ifnum#1=2 \hskip\pslabelsep\else\hss\fi
\box\pst@hbox
\ifnum#1=1 \hskip\pslabelsep\else\hss\fi}%
\ifnum#2=2 \vskip\pslabelsep\else\vss\fi}}
\def\tx@Uput{Uput }
\def\tx@UUput{UUput }
\def\Rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Rput@ii}{\Rput@i}}}
\def\Rput@i#1{\addto@par{labelsep=#1}\Rput@ii}
\def\Rput@ii[#1]{\addto@par{ref={#1}}\@ifnextchar({\Rput@iv}{\Rput@iii}}
\def\Rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\Rput@iv}{\Rput@iv(\z@,\z@)}}
\def\Rput@iv(#1){\pst@killglue\pst@makebox{\Rput@v{#1}}}
\def\Rput@v#1{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\Rput@vi
\pst@makesmall\pst@hbox
\pst@rotate\psk@rot\pst@hbox
\psput@{#1}\pst@hbox
\endgroup
\ignorespaces}
\def\Rput@vi{%
\pst@dimg=\dp\pst@hbox
\advance\pst@dimg\pslabelsep
\dp\pst@hbox=\pst@dimg
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg\pslabelsep
\ht\pst@hbox=\pst@dimg
\setbox\pst@hbox\hbox{\kern\pslabelsep\box\pst@hbox\kern\pslabelsep}}%
\def\oldpsput{%
\def\pst@par{}\pst@ifstar{\@ifnextchar[{\oldpsput@i}{\oldpsput@ii}}}
\def\oldpsput@i[#1]{\addto@par{ref={#1}}\oldpsput@ii}
\def\oldpsput@ii{\@ifnextchar<{\oldpsput@iii}{\oldpsput@iv}}
\def\oldpsput@iii<#1>{\rput@iii{#1}}
\def\OldPsput{\let\psput\oldpsput}
\def\NewPsput{\let\psput\rput}
\def\pspicture{\begingroup\pst@ifstar\pst@picture}
\def\pst@picture{%
\@ifnextchar[{\pst@@picture}{\pst@@picture[0]}}
\def\pst@@picture[#1]#2(#3,#4){%
\@ifnextchar({\pst@@@picture[#1](#3,#4)}%
{\pst@@@picture[#1](0,0)(#3,#4)}}
\def\pst@@@picture[#1](#2,#3)(#4,#5){%
\pssetxlength\pst@dima{#2}%
\pssetylength\pst@dimb{#3}%
\pssetxlength\pst@dimc{#4}%
\pssetylength\pst@dimd{#5}%
\ifdim\pst@dima>\pst@dimc
\pst@dimg=\pst@dima
\pst@dima=\pst@dimc
\pst@dimc=\pst@dimg
\fi
\ifdim\pst@dimb>\pst@dimd
\pst@dimg=\pst@dimb
\pst@dimb=\pst@dimd
\pst@dimd=\pst@dimg
\fi
\def\pst@tempa{#1}%
\setbox\pst@hbox=\hbox\bgroup
\begingroup\KillGlue
\@ifundefined{@latexerr}{}{\let\unitlength\psunit}%
\edef\pic@coor{(#2,#3)(#2,#3)(#4,#5)}\ignorespaces}
\def\pic@coor{(0,0)(0,0)(10,10)}
\def\endpspicture{%
\pst@killglue
\endgroup
\egroup
\ifdim\wd\pst@hbox=\z@\else
%\@pstrickserr{Extraneous space in the pspicture environment}%
%{Type \space <return> \space to procede.}%
\fi
\ht\pst@hbox=\pst@dimd
\dp\pst@hbox=-\pst@dimb
\setbox\pst@hbox=\hbox{%
\kern-\pst@dima
\ifx\pst@tempa\@empty\else
\advance\pst@dimd-\pst@dimb
\pst@dimd=\pst@tempa\pst@dimd
\advance\pst@dimd\pst@dimb
\lower\pst@dimd
\fi
\box\pst@hbox
\kern\pst@dimc}%
\if@star\setbox\pst@hbox=\hbox{\clipbox@@\z@}\fi
\leavevmode\box\pst@hbox
\endgroup}
\@namedef{pspicture*}{\pspicture*}
\@namedef{endpspicture*}{\endpspicture}
\def\tx@BeginOL{BeginOL }
\def\tx@InitOL{InitOL }
\def\pst@initoverlay#1{\pst@Verb{\tx@InitOL /TheOL (#1) def}}
\def\AltOverlayMode{%
\def\pst@initoverlay##1{%
\pst@Verb{%
\tx@InitOL
/Visible { initclip } def
/Invisible {
CP newpath OLUnit itransform moveto clip newpath moveto
} def
/TheOL (##1) def}}}
\def\pst@overlay#1{%
\edef\curr@overlay{#1}%
\pst@Verb{(#1) BOL}%
\aftergroup\pst@endoverlay}
\def\pst@endoverlay{%
\pst@Verb{(\curr@overlay) BOL}}
\def\curr@overlay{all}
\newbox\theoverlaybox
\def\overlaybox{%
\global\setbox\theoverlaybox=\hbox\bgroup
\begingroup
\let\psoverlay\pst@overlay
\def\overlaybox{%
\@pstrickserr{Overlays cannot be nested}\@eha}%
\def\putoverlaybox{%
\@pstrickserr{You must end the overlay box
before using \string\putoverlaybox}}%
\psoverlay{main}%
\ignorespaces}
\def\endoverlaybox{\endgroup\egroup}
\def\putoverlaybox#1{%
\hbox{\pst@initoverlay{#1}\copy\theoverlaybox}}
\def\psoverlay{\@pstrickserr{\string\psoverlay\space
can only be used after \string\overlaybox}}
\ifx\pstcustomize\relax \input pstricks.con \fi
\catcode`\@=\PstAtCode\relax
%
\endinput
%%
%% END: pstricks.tex

